Towards multiple elliptic polylogarithms

We investigate the elliptic analogs of multi-indexed polylogarithms that appear in the theory of the fundamental group of the projective line minus three points as sections of a universal nilpotent bundle with regular singular connection. We use an analytic uniformisation to derive the fundamental nilpotent De Rham torsor of a single elliptic curve in terms of a double Jacobi form introduced by Kronecker. We then extend this result to any smooth family, relatively to the base, i.e., to the moduli stack $M_{1,2}$ over $M_{1,1}$. Everything relies on explicit formulas that turn out to be algebraic for rational (families of) elliptic curves, and we conclude by providing the corresponding natural $\QM$ structure.

==> Andrey-2007-02-27/1.TEX <==
\section{Universal flat connection.}
\subsection{ The basic function.}

\thesubsubsection
 The following function $F(\xi , \alpha , \tau ) $ was introduced by Leopold Kronecker
\begin{eqnarray*}
F(\xi , \alpha , \tau ) =(2\pi i)\left(
1 - \frac {1}{1-z} -\frac{1}{1-w} - \sum_{m,n=1}^{\infty}
(z^m w^n -z^{-m} w^{-n}) q^{mn}\right)\\
\Im \tau >\Im \xi >0,\Im \tau > \Im \alpha > 0;
\end{eqnarray*}
where $q=\exp (2\pi i \tau ) ,\quad
z=\exp (2\pi i \xi ),\quad w=\exp (2\pi i \alpha )$.
Then \cite{Z} $F$ can be continued to a meromorphic function
with poles at divisors $\xi =m+n\tau$ and $\alpha =m' +n'\tau$ and
\begin{equation}
F(\xi ,\alpha ;\tau )=\frac{\theta'(0;\tau ) \theta(\xi + \alpha ;\tau )}
{  \theta (\xi ;\tau ) \theta (\alpha ;\tau )}. \label{theta}
\end{equation}
The transformation  properties of $F(\xi ,\alpha ;\tau )$ are very
simple:
\begin{eqnarray}
F(\xi+1 ,\alpha ;\tau )&=&F(\xi ,\alpha ;\tau );\\
F(\xi +\tau ,\alpha ;\tau )&=
&\exp (-2 \pi i \alpha )F(\xi ,\alpha ;\tau );\\
F(\frac{\xi}{c\tau +d} ,\frac{ \alpha}{c\tau +d} ,
\frac{a\tau +b}{c\tau +d} )&=&
(c\tau +d)\exp (2\pi i\frac{c\xi \alpha }
{c\tau +d})F(\xi , \alpha ;\tau ).\label{dermod}
\end {eqnarray}
\thesubsubsection
According to Zagier, $F(\xi , \alpha ;\tau )$ can be expressed
as the exponential of the generating function of Eisenstein functions
$E_k(\xi ;\tau ) =
\displaystyle{\sum\limits_{w\in L}} {}_e \frac{1}{ (w + \xi)^k }$
and Eisenstein series
$e_k(\tau ) =
\displaystyle{\sum\limits_{w\in L}}' {}_e \frac{1}{ (w  )^k }$
($\sum {}_e$ denotes Eisenstein summation \cite{W})
:
\begin{equation}
F(\xi , \alpha ;\tau )=
\frac1{ \alpha}\exp(-\sum _{k=1}^{\infty}\frac{(-\alpha )^k}k
(E_k(\xi ;\tau )-e_k(\tau))).\label{expg}
\end{equation}
This statement is a simple corollary of Zagier's
``Logarithmic Formula'' for $F(\xi ,\alpha ;\tau )$
\cite[Section~3,Theorem(viii)]{Z} and
the power series for $E_n$ \cite[Chapter~III,formula(10)]{W}.

{\bf Remark.} In ... the factor $2\pi i$ wes missed.

From the very definition of the function $F$
it satisfies the ``mixed heat'' equation
\begin{equation}2 \pi i \frac{\partial}{\partial \tau} 
F(\xi , \alpha ;\tau ) =
\frac{\partial^2}{\partial \xi \partial \alpha} 
F(\xi , \alpha ;\tau ).\label{mhe}\end{equation}

We shall use the following identity

$$F(\xi , \alpha _1;\tau )
F'_2(\xi , \alpha_2 ;\tau )-
F(\xi , \alpha_2 ;\tau )F'_2(\xi , \alpha_1 ;\tau )
=F(\xi , \alpha_1+\alpha_2 ;\tau )(\wp(\alpha_1)-
\wp(\alpha_2)),
$$
where $F'_2(\xi , \alpha ;\tau )=\frac{\partial F(\xi , \alpha ;\tau )}{\partial \alpha}$ denotes the derivative with respect to the second argument $\alpha$ and $\wp$ denotes the Weierstra{\ss} function
$\wp =E_2-e_2$.

A proof of the last identity is rather simple.


\subsection{ The connection with
logarithmic singularity on the elliptic curve.}

Let $E_{\tau}$ be an elliptic curve defined as
$\Bbb C/\Bbb Z\tau +\Bbb Z$, $\Im (\tau)>0$.
We fix notation $\xi$ for the coordinate on $\Bbb C$.


Consider an algebra $ R=\Bbb C \ll \bfa ,B\gg$
of noncommutative formal power series in two
variables $\bfa $ and $B$. For any power series $r$
denote by the same symbol 
$r $ the endomorphism of the
left multiplication: $r (r')=rr'$. 

Define a (pro) vector bundle ${\cal P}_\tau$ on $E_\tau$
with fiber $R$ by multipliers  
$\exp (-2\pi i \bfa ) $ and $1$;
so a section of ${\cal P}_\tau$ is an $R$-valued function 
$f(\xi,\bfa , B)$ on $\Bbb C$ such that 
$f(\xi+\tau, \bfa , B)=
\exp (-2\pi i \bfa ) f(\xi, \bfa , B)$,
 $f(\xi+1, \bfa , B)=f(\xi, \bfa , B)$. Hence, an
endomorphism $L$ of the bundle  ${\cal P}_\tau$ is
an ${\rm End}(R)$-valued function $L(\xi )$ on 
$\Bbb C$ such that 
$$L(\xi+\tau )=
\exp (-2\pi i \bfa ) L(\xi )\exp (2\pi i \bfa )=
\exp (-2\pi i {\rm ad}_\bfa ) L(\xi ),$$
$$
 L(\xi+1)=L(\xi);$$ here ${\rm ad}_\bfa $ denotes
the adjoint action of $a$ on $R$: 
${\rm ad}_\bfa (p)=\bfa p-p\bfa $,
denote it by $\alpha={\rm ad}_\bfa $.

Consider an expression $ \alpha F(\xi , \alpha ;\tau )$. We treat it as a function in $\xi$
which takes values 
in formal power series in $\alpha$,
so $ \alpha F(\xi , \alpha ;\tau )B$ takes values
in formal power series in $\bfa $ and $B$ after
substitution $\alpha={\rm ad}_\bfa $, as we have denoted.


The operator $ \alpha F(\xi , \alpha ;\tau )B $
  satisfies to the quasiperiodic properties with
respect to $\xi\to\xi+\tau$ and $\xi\to \xi+1$,
so it is an endomorphism of ${\cal P}_\tau$. It is a meromorphic  function in $\xi$ with simple
pole at $0$. Hence, we prove the following result.

{\bf Proposition 1.} The differential operator  
$\nabla_{fw}=d- \alpha F(\xi , \alpha ;\tau )B d\,\xi $
defines a connection on ${\cal P}_\tau$ with logarithmic
singularity at $0$.
 
\subsection{ The connection  with
logarithmic singularity on the family of
elliptic curves.} 

We can treat the parameter $\tau$ of the elliptic
curve as a variable, so we get a family $\Bbb E$ of
elliptic curves over the upper-half-plane
$\Bbb H=\{\tau |{\Im \tau}>0\}$. Furthermore
we define a bundle with the fiber $R$ on $\Bbb E$ by
the same rule as in the case of the individual curve;
denote it  by $\cal P$. 
We shall lift
the fiberwise connection $\nabla_{fw}$ to 
a {\it flat} connection $\nabla_{\cal P}$ on $\cal R$
over {\it the surface $\Bbb E$}.

First we introduce same convenient for us notation.
Let $\bfa $ $B$ and $C$ be elements of some 
pronilpotent Lie algebra. we use notation
$\alpha$ for ${\rm ad}_\bfa $; denote by $\alpha_1^{i}
\alpha_2^{j}\odb B,C\cdb$ the element $[{\rm ad}_\bfa ^iB,
 {\rm ad}_\bfa ^jC]$. We extend such a notation 
to formal power series $f(\alpha_1, \alpha_2)$ 
in two 
{\it commutative} variables  $\alpha_1,\alpha_2$.
The Jacobi identity yields the equality
$\alpha f(\alpha_1, \alpha_2)\odb B,C\cdb=
(\alpha_1+\alpha_2) f(\alpha_1, \alpha_2)\odb B,C\cdb$.

Note, that if $C=B$, the symmetric 
($f(\alpha_1, \alpha_2)=f(\alpha_2, \alpha_1)$)
power series produces zero; in this case
it is reasonable to consider only
antisymmetric power series.

{\bf Lemma 1.} Let $D$ be a differentiation of the
Lie algebra. Then
$$D\, (f(\alpha)B)= 
\frac{f(\alpha_1+\alpha_2)-f(\alpha_2)}{\alpha_1}
\odb D\,(\bfa ),B\cdb +f(\alpha)D\,(B). $$
 
{\bf Proof.} It is sufficient to check this formula
for $f(\alpha)=\alpha^i$. For $i=0$ the statement 
is evidently true. By induction:
$$D\,(\alpha^i(B))=[D(\bfa ), \alpha^{i-1}(B)]+
\alpha d\,(\alpha^{i-1}(B))=$$
$$
\alpha_2^{i-1}(D(\bfa ),B)+(\alpha_1+\alpha_2)
\frac{(\alpha_1+\alpha_2)^{i-1}-
\alpha_2^{i-1}}{\alpha_1}
\odb D\,(\bfa ),B\cdb +\alpha(\alpha)^{i-1}D\,(B)=
$$
$$\frac{(\alpha_1+\alpha_2)^{i}-
\alpha_2^{i-1}}{\alpha_1}
\odb D\,(\bfa ),B\cdb +(\alpha)^{i}D\,(B).
$$

{\bf Lemma 2.} Let $D$ be a differentiation of the
Lie algebra. Then in the universal enveloping
the following equality holds
$$D(\exp(\bfa ))=
\exp(\bfa )\frac{\exp(-\alpha)-1}{-\alpha}D(\bfa ).
$$ 

 


 Now we are able to define the connection 
$\nabla_{\cal P}$.  Put 
$$\omega_B =-\frac12\frac{1}{2\pi i}
\frac{\alpha_1\alpha_2}{\alpha_1+\alpha_2}
\left(\left(\wp(\alpha_1)-\frac1{\alpha_1^2}\right)
-\left(\wp(\alpha_2)-\frac1{\alpha_2^2}\right)
\right)\odb B,B\cdb d\,\tau,\quad 
\omega_{\bfa} =-\frac1{2\pi i} Bd\,\tau,
$$
$$\nu=
-\left(\alpha F(\xi , \alpha ;\tau ) d\,\xi
+\frac{1}{2\pi i}\left(\alpha F'_2(\xi , \alpha ;\tau )+
\frac{1}{\alpha}\right)d\,\tau\right)B.$$
Then
$$\nabla_{\cal P}=d\,  +\nu  
+\omega_B 
\frac{\partial\,}{\partial\, B}+\omega_{\bfa}
\frac{\partial\,}{\partial\, \bfa },$$
where
$f\frac{\partial\,}{\partial\, B}$ (and 
$f\frac{\partial\,}{\partial\, \bfa }$) is the {\it 
differentiation} on $R$, so
$f\frac{\partial\, r_1r_2}{\partial\, B} =f
\frac{\partial\, r_1}{\partial\, B}  
r_2+r_1f\frac{\partial\, r_2}{\partial\, B}$
 (no term
$[\omega_B,r_1]
\frac{\partial\, r_2}{\partial\, B}$!!!). Hence the commutator 
$[f\frac{\partial\,}{\partial\, B},r ]$
 of $f\frac{\partial\,}{\partial\, B}$
and $r $ is just $f\frac{\partial\,r}{\partial\, B}  $


{\bf Proposition 2.} The operator $\nabla_{\cal P}$ 
is a connection on $\cal P$.

{\bf Proof.} We must check that $\nabla_{\cal P}$
is invariant with respect to shift $\xi\to\xi +1$
and that $\nabla_{\cal P}$ transforms in correct
way under shift $\xi \to \xi+\tau$. The first 
property
followes immediately from the invariance of $F$ with
respect to this shift. So we shall check that
$$\nabla_{\cal P}|_{\xi+\tau}=
\exp(-2\pi i \bfa )\nabla_{\cal P}|_{\xi }
\exp(2\pi i \bfa ).$$
The summand $  \nu  $
in the l.h.s. is equal to  
$$  -\left(\alpha F(\xi+\tau , \alpha ;\tau ) d\,(\xi+\tau)
+\frac{1}{2\pi i}\left(\alpha F'_2(\xi +\tau, \alpha ;\tau )+
\frac{1}{\alpha}\right)d\,\tau\right)B =
$$
$$ -\left(\exp(-2\pi i\alpha)(\alpha F(\xi  , \alpha ;\tau ) d\,\xi 
 + \alpha F(\xi  , \alpha ;\tau )d\,\tau) 
\phantom{\frac{1}{\alpha}}\right.
+$$
$$ \left.\frac{1}{2\pi i}\left(\exp(-2\pi i\alpha)(
-2\pi i\alpha F(\xi  , \alpha ;\tau )+\alpha F'_2(\xi +\tau, \alpha ;\tau ))+
\frac{1}{\alpha}\right)d\,\tau\right)B =
$$
$$ -\exp(-2\pi i\alpha)\left(\alpha F(\xi  , \alpha ;\tau ) d\,\xi 
 +  \left( \frac{1}{2\pi i}\left(
 \alpha F'_2(\xi +\tau, \alpha ;\tau )+
\frac{1}{\alpha}\right)+
\frac{\exp(2\pi i\alpha)-1}{2\pi i\alpha}\right)
d\,\tau\right)B .
$$
Other terms in the l.h.s. do not depend in $\xi$;
so they are invariant.

In the r.h.s. the term $\exp(-2\pi i \bfa )
\nu
\exp(2\pi i \bfa )$ is equal to
$$ -\exp(-2\pi i\alpha)\left(\alpha F(\xi  , \alpha ;\tau ) d\,\xi 
 +   \frac{1}{2\pi i}\left(
 \alpha F'_2(\xi +\tau, \alpha ;\tau )+
\frac{1}{\alpha}\right)  
d\,\tau\right)B .
$$

The term 
$ \exp(-2\pi i  \bfa ) \omega_B \frac{\partial\,}{\partial\, B} 
\exp(2\pi i  \bfa )$ equals $\omega_B \frac{\partial\,}{\partial\, B}$ as 
$  \frac{\partial\,\exp(2\pi i a)}{\partial\, B}=0$.

The term  $\exp(-2\pi i  \bfa ) \omega_{\bfa}  \frac{\partial\,}{\partial\,  \bfa } 
\exp(2\pi i  \bfa )$ is equal to

$$\exp(-2\pi i  \bfa ) \left(-\frac1{2\pi i}B \frac{\partial\,}{\partial\,  \bfa }\right) 
\exp(2\pi i  \bfa )
\stackrel{\mbox{Lemma 2.}}{=} \frac{\exp(-2\pi i\alpha)-1}{-2\pi i\alpha} 
(- B)-\frac1{2\pi i}B 
\frac{\partial\,}{\partial\,  \bfa }.   
$$ 
So, the l.h.s. is equal to the r.h.s.

{\bf Proposition 3.} The connection $\nabla_{\cal P}$
is flat.

{\bf Proof.}
Denote by $\omega$ the differential form
$$\nu  
+\omega_B 
\frac{\partial\,}{\partial\, B}+\omega_{\bfa}\frac{\partial\,}{\partial\, a}.$$
 
We shall prove that $d\,\omega+\omega\wedge\omega=0$.
The term $d\,\omega$ is equal to $d\,\nu $, as other terms are lifted from
one dimensional $\Bbb H$, so are closed. So,  $d\,\omega$  equals  
$$-d\, \left(\alpha F(\xi , \alpha ;\tau ) d\,\xi
+\frac{1}{2\pi i}\left(\alpha F'_2(\xi , \alpha ;\tau )+
\frac{1}{\alpha}\right)d\,\tau\right)B=$$
$$\left(
\frac{\partial}{\partial\,\tau}
(\alpha F(\xi , \alpha ;\tau )) -\frac{1}{2\pi i}\frac{\partial}{\partial\,\xi}\left(\alpha F'_2(\xi , \alpha ;\tau )+
\frac{1}{\alpha}\right)\right)d\,\xi\wedge d\,\tau
B
$$
$$\alpha\left( 
\frac{\partial}{\partial\,\tau}
F(\xi , \alpha ;\tau ) -\frac{1}{2\pi i}\frac{\partial}{\partial\,\xi}   F'_2(\xi , \alpha ;\tau )
  \right)d\,\xi\wedge d\,\tau 
B =0,
$$
as the function $F$ satisfies to the mixed heat 
equation.
The term $\omega\wedge\omega$ equals  
$$\left[\alpha F(\xi , \alpha ;\tau ) B,
\frac{1}{2\pi i}\left(\alpha F'_2(\xi , \alpha ;\tau )+
\frac{1}{\alpha}\right)B\right] d\,\xi
\wedge d\,\tau+$$
$$\left[-\frac12\frac{1}{2\pi i}
\frac{\alpha_1\alpha_2}{\alpha_1+\alpha_2}
\left(\left(\wp(\alpha_1)-\frac1{\alpha_1^2}\right)
-\left(\wp(\alpha_2)-\frac1{\alpha_2^2}\right)
\right)\odb B,B\cdb \frac{\partial}{\partial\, B},
\alpha F(\xi , \alpha ;\tau ) B
\right] d\,\xi
\wedge d\,\tau-$$
$$\left[\frac{B}{2\pi i}
\frac{\partial}{\partial\,  \bfa },
\alpha F(\xi , \alpha ;\tau ) B
\right] d\,\xi
\wedge d\,\tau. 
$$
The first summond, up to factor $\frac{d\,\xi\wedge d\,\tau}{2\pi i}$ can be written as
$$
  \alpha_1F(\xi , \alpha_1 ;\tau ) 
 \left(\alpha_2 F'_2(\xi , \alpha_2 ;\tau )+
\frac{1}{\alpha_2}\right)\odb B,B\cdb   =
$$
$$
 \frac12\left(\alpha_1F(\xi , \alpha_1 ;\tau ) 
 \left(\alpha_2 F'_2(\xi , \alpha_2 ;\tau )+
\frac{1}{\alpha_2}\right)
-\alpha_2 F(\xi , \alpha_2 ;\tau ) \left(\alpha_1
F'_2(\xi , \alpha_1 ;\tau )+
\frac{1}{\alpha_1}\right)\right)\odb B,B\cdb ;  
$$
the second one, up to the same factor, equals
$$
-\frac12(\alpha_1+\alpha_2) F(\xi , 
\alpha_1+\alpha_2 ;\tau ) \frac{\alpha_1\alpha_2}{\alpha_1+\alpha_2}
\left(\left(\wp(\alpha_1)-\frac1{\alpha_1^2}\right)
-\left(\wp(\alpha_2)-\frac1{\alpha_2^2}\right)
\right)\odb B,B\cdb ; 
 $$
the third summond can be calculated by application 
of Lemma 1, we get (up to the same factor as above)
$$ -\frac{
(\alpha_1+\alpha_2) F(\xi , \alpha_1+\alpha_2 ;\tau )
- \alpha_2 F(\xi ,  \alpha_2 ;\tau )}{\alpha_1} 
\odb B,B\cdb =
$$
 
$$-\frac12\left(\frac{
(\alpha_2^2-\alpha_1^2) 
F(\xi , \alpha_1+\alpha_2 ;\tau )+
\alpha_1^2 F(\xi ,  \alpha_1 ;\tau )-
\alpha_2^2 F(\xi ,  \alpha_2 ;\tau )}
{\alpha_1\alpha_2}\right) 
\odb B,B\cdb .
$$
Finally, we conclude that the term $\omega\wedge\omega$ is equal to 
$\frac12\frac{d\,\xi\wedge d\,\tau}{2\pi i}
\Xi(\alpha_1,\alpha_2)\odb B,B\cdb $, where
$$\Xi(\alpha_1,\alpha_2)= \alpha_1F(\xi , \alpha_1 ;\tau ) 
 \left(\alpha_2 F'_2(\xi , \alpha_2 ;\tau )+
\frac{1}{\alpha_2}\right)
-\alpha_2 F(\xi , \alpha_2 ;\tau ) \left(\alpha_1
F'_2(\xi , \alpha_1 ;\tau )+
\frac{1}{\alpha_1}\right) -$$
$$
{\alpha_1\alpha_2}   F(\xi , 
\alpha_1+\alpha_2 ;\tau )  \left(\left(\wp(\alpha_1)-\frac1{\alpha_1^2}\right)
-\left(\wp(\alpha_2)-\frac1{\alpha_2^2}\right)
\right)-$$
$$ \frac{
(\alpha_2^2-\alpha_1^2) 
F(\xi , \alpha_1+\alpha_2 ;\tau )+
\alpha_1^2 F(\xi ,  \alpha_1 ;\tau )-
\alpha_2^2 F(\xi ,  \alpha_2 ;\tau )}
{\alpha_1\alpha_2} =$$
 
$$ \alpha_1F(\xi , \alpha_1 ;\tau ) 
  \alpha_2 F'_2(\xi , \alpha_2 ;\tau ) -\alpha_2 F(\xi , \alpha_2 ;\tau )  \alpha_1
F'_2(\xi , \alpha_1 ;\tau )  -$$
$$
{\alpha_1\alpha_2}   F(\xi , 
\alpha_1+\alpha_2 ;\tau )   \left(\wp(\alpha_1) -\wp(\alpha_2)  \right)  =0.$$

So, we have proved the flatness of the connection
$\nabla_{\cal P}$.



Consider the standard action of the modular group 
$SL_2(\Bbb Z)$ on the upper-half-plane $\Bbb H$ and
the relative curve $\Bbb E$ over $\Bbb H$:
$\tau\to \tau' =\frac{a\tau +b}{c\tau +d};\quad
\xi\to \xi'=\frac{\xi}{c\tau +d}$. 
Denote by ${\cal R} $ the (pro)bundle on $\Bbb H$ with the fiber $R$.
Define an action of $SL_2(\Bbb Z)$ on $\cal R$
by the rule:
$\bfa \to \bfa'=\frac{\bfa }{c\tau +d}$,  
$B\to B'=(c\tau +d)B +2\pi i c \bfa$; and  lift this action to an action on $\cal P$ by  multiplier 
$\exp(2\pi i\frac{c \xi \bfa}{c\tau +d})$,
so the a $SL_2(\Bbb Z)$-invariant section of $\cal P$   is
an $R$-valued function $f$ in $\tau$ and $\xi$
such that 

$$f(\frac{a\tau +b}{c\tau +d}, \frac{\xi}{c\tau +d};
\frac{\bfa }{c\tau +d}, (c\tau +d)B +2\pi i c\bfa)=
\exp\left(2\pi i\frac{c \xi \bfa}{c\tau +d}\right) f(\tau, \xi;
\bfa,B).$$

This action is well defined (compatible with the group structure on $SL_2(\Bbb Z)$ and compatible
with fiberwise action of the $\Bbb Z^2$.
We leave these as an exercise to the reader. 

Hence, for an endomorphism we have the same 
condition with replacment $\bfa \to \alpha$.

{\bf Proposition 4.} The connection $\nabla_{\cal P}$
is  $SL_2(\Bbb Z)$ invariant.
 
{\bf Proof.} We shall prove that 

$$\nabla_{\cal P}  |_{\tau', \xi';
\bfa',B'}
=\exp\left(2\pi i\frac{c \xi \bfa}{c\tau +d}\right)\nabla_{\cal P} |_{\tau, \xi;
\bfa,B}\exp\left(-2\pi i\frac{c \xi \bfa}{c\tau +d}\right).$$

The term $\nu$ in the l.h.s. equals
$$
-\left(\frac{\alpha}{c\tau+d} 
F\left(\frac{\xi}{c\tau+d} , 
\frac{\alpha}{c\tau+d} ;\frac{a\tau +b}{c\tau+d} \right) 
d\,\frac{\xi}{c\tau+d}+\right.$$
$$\left.
\frac{1}{2\pi i}\left(
\frac{\alpha}{c\tau+d} 
F'_2(\frac{\xi}{c\tau+d} , 
\frac{\alpha}{c\tau+d} ;\frac{a\tau +b}{c\tau+d} 
 )+
\frac{{c\tau+d}}{ {\alpha}}\right)
d\,\frac{a\tau +b}{c\tau+d} \right)((c\tau +d)B+
2\pi i c\bfa)=
$$
 $$
-\exp\left(2\pi i\frac{c \xi \alpha}{c\tau +d}\right)\left( {\alpha} 
F( {\xi}  , 
 \alpha  ; \tau   ) 
\left(d\, {\xi}-\frac{c\xi}{c\tau+d}d\,\tau\right) -2\pi ic\bfa\left(\frac{d\, \xi}{c\tau+d}-\frac{c\xi 
d\,\tau}{(c\tau+d)^2}\right) +\right.$$
$$\left.
\frac{1}{2\pi i}\left(
 \alpha \left(2\pi i\frac{c\xi}{c\tau+d}F( {\xi}  , 
 \alpha  ; \tau   ) +  
F_2'( {\xi}  , 
 \alpha  ; \tau   ) \right)+
\exp\left(-2\pi i\frac{c \xi \alpha}{c\tau +d}\right)\frac{1}{ {\alpha}}\right)
d\,\tau \right)B
 =
$$
$$\exp\left(2\pi i\frac{c \xi \alpha}{c\tau 
+d}\right)
\nu +\frac{\exp\left(2\pi i\frac{c \xi \alpha}{c\tau +d}\right)-1}{\alpha}d\,\tau B-2\pi ic\bfa\left(\frac{d\, \xi}{c\tau+d}-\frac{c\xi
d\,\tau}{(c\tau+d)^2}\right).$$

In this calculations we use the modular property
of the function $F$ and evident equality
$f(\alpha)\bfa=f(0)\bfa$.


We have  $$\frac{\partial}{\partial B'}=
\frac1{c\tau +d} \frac{\partial}{\partial B},\quad\frac{\partial}{\partial \bfa'}=
(c\tau+d)\frac{\partial}{\partial \bfa }
-2\pi i c\frac{\partial}{\partial B}.$$ 
 As $\omega_B$ is a modular form
of the weight one:
$$\omega_B(\tau', \xi';
\bfa',B') 
=-\frac12\frac{1}{2\pi i}(c\tau +d)
\frac{\alpha_1\alpha_2}{\alpha_1+\alpha_2}
\left(\left(\wp(\alpha_1)-\frac1{\alpha_1^2}\right)
-\left(\wp(\alpha_2)-\frac1{\alpha_2^2}\right)
\right)\times$$
$$
((c\tau +d)B +2\pi i c \bfa,(c\tau +d)B +2\pi i c \bfa)\frac{d\,\tau}{(c\tau+d)^2} =(c\tau+d)
\omega_B(\tau, \xi;
\bfa,B ),$$
the term $\omega_B\frac{\partial}{\partial B}$ is $SL_2(\Bbb Z)$ invariant.

We have also:
$$\omega_{\bfa}(\tau', \xi';
\bfa',B') =-\frac1{2\pi i}((c\tau +d)B +2\pi i c \bfa)\frac{d\,\tau}{(c\tau+d)^2}=\frac1{c\tau +d}
\omega_{\bfa} -  c \bfa\frac{d\,\tau}{(c\tau+d)^2}.
$$

Note that $B'$ and $\bfa'$ depend in $\tau$ 
explicitly as function in $B$ and $\bfa$, so
$$ \left.\frac{ d}{d\,\tau}\right|_{ \bfa',B'}=  \frac{\partial }{\partial\,\tau} -\frac{cB'}{(c\tau +d)^2}
\frac{\partial }{\partial\,B}
+c\bfa'\frac{\partial }{\partial\,\bfa}
$$
Therefore
$$d|_{ \bfa',B'} +\omega_{\bfa}  
({\tau', \xi';
\bfa',B'}) 
\frac{\partial\,}{\partial\, \bfa' }= d|_{\bfa, B}+ 
d\tau\left(
  -\frac{cB'}{(c\tau +d)^2}
\frac{\partial }{\partial\,B}
+c\bfa'\frac{\partial }{\partial\,\bfa}\right)$$
$$\left(\frac1{c\tau +d}
\omega_{\bfa} -  c \bfa\frac{d\,\tau}{(c\tau+d)^2} \right)
(c\tau+d)\frac{\partial}{\partial \bfa }+$$
$$\left(-\frac1{2\pi i}B'\frac{d\,\tau}{(c\tau+d)^2}
\right)\left(-2\pi i c\frac{\partial}{\partial B}\right)=d|_{\bfa, B} +\omega_{\bfa}
\frac{\partial}{\partial \bfa }.
$$

In the r.h.s. we have:
$$\exp\left(2\pi i\frac{c \xi \bfa}{c\tau +d}\right)\left(d -\frac1{2\pi i} Bd\,\tau\frac{\partial\,}{\partial\, \bfa }
\right)\exp\left(-2\pi i\frac{c \xi \bfa}{c\tau +d}\right)=$$
$$d  -
2\pi ic\bfa\left(\frac{d\, \xi}{c\tau+d}-\frac{c\xi 
d\,\tau}{(c\tau+d)^2}\right) +\frac{\exp\left(2\pi i\frac{c \xi \alpha}{c\tau +d}\right)-1}{\alpha}d\,\tau B,
$$
the second summond comes from the differentiation 
by $\xi$ and $\tau$, the last can be calculated
with using Lemma 2.  

Evidently,
$$
\exp\left(2\pi i\frac{c \xi \bfa}{c\tau +d}\right)\nu\exp\left(-2\pi i\frac{c \xi \bfa}{c\tau +d}\right)=\exp\left(2\pi i\frac{c \xi \alpha}{c\tau 
+d}\right)
\nu;$$
and $\omega_B 
\frac{\partial\,}{\partial\, B}$ commutes with
$\exp\left(-2\pi i
\frac{c \xi \bfa}{c\tau +d}\right)$.
This finishes the proof.

Note that such a lifting of fiberwise connection to the flat connection is not unique. Indeed, one can
twist the connection $\nabla_{\cal P}$ by any $R$-valued $SL_{2}(\Bbb Z)$-invariant form  $\mu$ on $\Bbb H$
by the right multiplication on $\mu$:
$$\nabla_{\cal P}^{\mu}(G)=\nabla_{\cal P}(G)+G\mu=\nabla_{\cal P}(G)+\mu G- {\rm ad}_\mu G.$$
This connection is flat as the right and the left multiplications commute.


==> Andrey-2007-02-27/2.TEX <==

{\bf 4. Parallel transports.}

Now we pass to the parallel transports along paths.
Discuss first the general situation.
Let $\nabla$ be a holomorphic connection on a curve  
and let $\gamma$ be a path from a point $\xi_1$
to $\xi_2$. Recall that the {\it parallel transport}
${\cal J}^{\gamma}(\xi_1,\xi_2)$ from the point $\xi_1$
to the point $\xi_2$ along the path $\gamma$ is
an operator from the fiber over $\xi_1$ to the
fiber over $\xi_2$ which is the horizontal 
continuation of the identical map on the fiber
over $\xi_1$ along the path $\gamma$. In the other words,  ${\cal J}^{\gamma}(\xi_1,\xi_2)$ is the solution
of an equation $\nabla 
{\cal J}^{\gamma}(\xi_1,\xi_2)=0$, 
here $\nabla$ acts on the second argument of ${\cal J}$
with initial data ${\cal J} (\xi_1,\xi_1)=1$

In the case under consideration
the  connection $\nabla_{fw}$ acts by multiplication by some formal power series
from the left, so the parallel transport is   the multiplication from
the left by  another formal power series, this power series we
denote by the same symbol  ${\cal J}^{\gamma}(\xi_1,\xi_2)$. 
This power  series ${\cal J}^{\gamma}(\xi_1,\xi_2)$ is a
$\nabla$-horizontal continuation along the path $\gamma$ of the
formal power series equals to $1$.  

Evidently, we have
the composition formula:
${\cal J}^{\gamma\gamma'}(\xi_1,\xi_3)={\cal J}^{\gamma'}(\xi_2,\xi_3){\cal J}^{\gamma}(\xi_1,\xi_2)$.

If some of the points $\xi_i$ are the singular points
of the connection one can define a 
{\it regularized} parallel transport as followes.

The points $\xi=m\tau +n $ are singular point of the connection $\nabla_{fw}=d+\nu$
and   the connection   
has singularity of
the first order (fuchsian singularity) at $\xi$.  
  Fix  a local coordinate
$t$ near $\xi$. Let $K={\rm Res}_{\xi}(\nu)$ be the
residue of the connection at $\xi$; so, locally
$\nu=K_id\,\log t +\nu_{hol}$, $\nu_{hol}$ is holomorphic. 
Then  we can construct a local
multivalued horisontal section $S(t)$
of the type 
$G(t)\exp(-K\log t)$, $G$ are holomorphic
$G(0)=1$. Indeed,
the differential equation on $G$ is
$d\,G=-Kd\,\log t G +G Kd\,\log t
-\nu_{hol} G$; so if we put 
$$G=1+\sum_{w} wg_w(t), \mbox{ $w$'s are  words in $\bfa$ and $B$},$$ 
$g_w(0)=0$ we get a sequence of {\it holomorphic} nonhomogeneous  equations
for $g_w$, as the singularity of $[w,Kd\,log t]g_w$ vanishes either as $K$ commutes with $1$
or as $g_w$ has a zero at the origin $t=0$.
So, we  can choose the vanishing at zero solutions of these equations.
Call such a section {\it the normalized horizontal section}. Note
that if the connection has no pole at the point $\xi$, then 
the normalized horizontal section is a horizontal section whose
value at $\xi$  equals $1$.

Return to the parallel transports. Denote by $S_i$ the normalized horizontal section
near $\xi_i$.
 Fix the standard branches of $\log(t_i)$,
consider a horizontal  continuation $S_1^{\gamma}$ of $S_1$
along the path $\gamma$ from $\xi_1$ to $\xi_2$,
and compare this continuation with $S_2$:
the regularized parallel transport is defined
as the quotient 
$ {\cal J}^{\gamma}((\xi_1,t_1),(\xi_2,t_2))=
S_2^{-1}S_1^{\gamma}$. 
We also can realize
parallel transport as the product
$S_2^{-1}(\xi_2'){\cal J}^{\gamma'}(\xi_1',\xi_2') 
S_1(\xi_1')$ for $\xi_i'$ close to $\xi_i$ and
$\gamma'$ close to $\gamma$.

This regularized parallel transport depends
from the choice of the coordiantes. Indeed,
let $S'_i$ be a local solution corresponding
to another coordinate $t'_i$, it is easy to
show that
$S'_i(t'_i)=S_i(t_i) \exp 
\left(-A_i\log\left(
\frac{d\,t'_i}{d\,t_i}(0)\right)\right)$,
so 
$${\cal J}^{\gamma}((\xi_1,t'_1),(\xi_2,t'_2)
=\exp \left(A_2\log\left(
\frac{d\,t'_2}{d\,t_2}(0)\right)\right)
{\cal J}^{\gamma}((\xi_1,t_1),(\xi_2,t_2)
\exp \left(-A_1\log\left(
\frac{d\,t'_1}{d\,t_1}(0)\right)\right).$$


So, for any path on the elliptic curve $E_\tau$
we can consider the parallel transport 
with respect to the universal connection 
$\nabla_{fw}$. We can restrict ourself
by two basic transports $\Phi_A$ and $\Phi_B$,
where $A$ and $B$ are the strait paths from
$0$ to $\tau$ and from $0$ to $1$ respectively.
We use the coordinate $\xi$ for regularization
of the parallel transports. 
Note that for $\Phi_A$ we shall calculate
the parallel transport and multiply it from
the left by $\exp(2\pi i\bfa)$, as the 
bundle is not trivial. 

We want to deduce  the differential
equation on such 
transports.

Let $\xi_1(\tau)$ and $\xi_2(\tau)$ be
two local sections of $\Bbb E \to \Bbb H$;
assume that they do not intersect the singular
locus of the connection $\nabla_{\cal P}$.

Lemma. For any continuous in $\tau$ family of 
the paths $\gamma(t,\tau),\,\, 0\leq t \leq 1$ 
  from $\xi_1$ to
$\xi_2$ the parallel transport 
${\cal J}^{\gamma}(\xi_1(\tau),\xi_2(\tau))$
satisfies to
the following equation as function in $\tau$:
$$d\,{\cal J}^{\gamma}(\xi_1(\tau),\xi_2(\tau))
=$$
$$-\nu|_{\xi_2(\tau)} {\cal J}^{\gamma}(\xi_1(\tau),\xi_2(\tau))
+{\cal J}^{\gamma}(\xi_1(\tau),\xi_2(\tau))\nu|_{\xi_1(\tau)}
-\left(\omega_B\frac{\partial}{\partial\, B}
+\omega_{\bfa}\frac{\partial}{\partial\, \bfa}\right)
{\cal J}^{\gamma}(\xi_1(\tau),\xi_2(\tau)).$$

{\bf Proof.} For fixed $\tau=\tau_0$  consider a solution $f(\xi)$ of    
the equation $\nabla_{\cal P}|_{E_0}f(\xi)=0$ ($E_0=E_{\tau_0}$)
with the initial data $f(\xi_1(\tau_0))=1$. This is 
multivalued, pick its branch by continuation
along the path $\gamma_0$ ($\gamma_0(t)=
\gamma(t,\tau_0)$) 
then   
${\cal J}^{\gamma}(\xi_1(\tau_0),\xi_2(\tau_0))=
f(\xi_2(\tau_0))$  
The connection $\nabla_{\cal P}$ is
flat, so we can (locally in $\tau$) consider the solution $f(\xi,\tau)$
of the equation $\nabla_{\cal P} f(\xi, \tau)=0$
with the initial data $f(\xi_1(\tau_0),\tau_0)=1$.
Consider its continuation along $\gamma_0$.
For any $\tau$ $f(\xi,\tau)$ is the solution
of   the equation $\nabla_{\cal P}|_{E_\tau}f(\xi)=0$
with initial data $f(\xi_1(\tau_0))=f(\xi_1(\tau),\tau)$,
so $g(\xi)=f(\xi,\tau)f^{-1}(\xi_1(\tau),\tau)$ is the solution
of the same equation with the initial data $ g(\xi_1(\tau)=1$. As $\gamma_0$ is close to
$\gamma_\tau$, the branch of the solution
is the same as continuation along the path $\gamma_\tau$. Finally, we get
$$ {\cal J}^{\gamma}(\xi_1(\tau),\xi_2(\tau))=
f(\xi_2({\tau}),\tau)f^{-1}(\xi_1(\tau),\tau).$$
As $f$ is horisontal, on the section 
$\xi_i(\tau)$ we have
$$d \, f(\xi_i(\tau), \tau) =-\nu|_{\xi_i(\tau)}
f(\xi_i(\tau), \tau) -\left(\omega_B\frac{\partial}{\partial\, B}
+\omega_{\bfa}\frac{\partial}{\partial\, \bfa}\right)
f(\xi_i(\tau), \tau).$$
Substuitution of this equation to the expession for
the parallel transport finishes the proof.


So, for {\it loops} $\gamma$ from section $\xi(\tau)$
to itself
we get the following connection on the transports:

$$\nabla_{transport}=d+{\rm ad}_{\nu|_\xi}
+\omega_B\frac{\partial}{\partial\, B}
+\omega_{\bfa}\frac{\partial}{\partial\, \bfa}.$$

Discuss now the regularized transports.
Let $\xi(\tau)$ be a section of singularities
of $\nabla$ and let
$t$ be a fiberwise coordinate around it.
Then $\nu -Kd\,\log(t)$ is holomorphic ($K={\rm Res}_\xi\nu$ as above), denote by $\nu|_{(\xi,t)}$ the
restriction of this holomorhic form to $\xi$.
$\nu|_{(\xi,t)}$ depends in the choice of the coordinate $t$, indeed if $t'$ be another 
coordinate, then
$ d\,\log(t')=d\,\log(t)+d\,\log(
\partial\,t'/\partial\,t)+...$ and restriction of the
second term to $\xi(\tau)$ can not vanish.

Note that 
$$d\,K+[\nu|_{(\xi,t)},K] + \left(\omega_B\frac{\partial}{\partial\, B}
+\omega_{\bfa}\frac{\partial}{\partial\, \bfa}\right)K=0,$$
as it is the singular part of the curvature 
of $\nabla_{\cal P}$.
 
{\bf Lemma.} The  regularized transports satisfy
to the same differential equation as in the smooth case:
$$d\,{\cal J}^{\gamma}((\xi_1(\tau),t_1),(\xi_2(\tau),t_2))
=$$
$$-\nu|_{(\xi_2(\tau),t_2)} {\cal J}^{\gamma}((\xi_1(\tau),t_1),(\xi_2(\tau),t_2))
+{\cal J}^{\gamma}((\xi_1(\tau),t_1),(\xi_2(\tau),t_2))
\nu|_{(\xi_1(\tau),t_1)}
-
$$
$$\left(\omega_B\frac{\partial}{\partial\, B}
+\omega_{\bfa}\frac{\partial}{\partial\, \bfa}\right)
{\cal J}^{\gamma}((\xi_1(\tau),t_1),(\xi_2(\tau),t_2)).$$

{\bf Proof.} 
As we have the composition formula 
$${\cal J}^{\gamma}((\xi_1(\tau),t_1,(\xi_2(\tau),t_2))=S_2^{-1}(\xi_2'){\cal J}^{\gamma'}(\xi_1',\xi_2') 
S_1(\xi_1')$$ 
 and the differential equation for the transport between nonsingular points,
it is enough to deduce the differential equation
for the local solutions $S_i(t_i)$.
 
$S(t,\tau)=G(t,\tau)\exp(-\log t K)$, and
$G$ is horizontal with respect to fiberwise connection $\tilde{\nabla}_{fw} f=\nabla_{fw}f-f Kd\,\log t $, $G(0,\tau)=1$.
Note that this connection is the restriction 
on the fibers of the {\it flat} connection 
$\tilde{\nabla}f=\nabla_{\cal P}f  -f Kd\,\log t
-f\nu|_{(\xi,t)}$. Flatness of this connection
follows from: i) flatness of $\nabla_{\cal P}$;
ii) commutation between the left and the right
multiplication and iii) equation on 
$K$ and $\nu|_{(\xi,t)}$. So we can repeat the
consideration from the proof of the previous
lemma and get:

$$d_\tau \,G(t,\tau)
= -\nu|_{t} G(t,\tau)+
G(t,\tau)\nu|_{(\xi ,t)}
-\left(\omega_B\frac{\partial}{\partial\, B}
+\omega_{\bfa}\frac{\partial}{\partial\, \bfa}\right)
G(t,\tau).$$

Using the equation on $K$ and $\nu_{(\xi,t)}$,
we can deduce that for
$S(t,\tau)=G(t,\tau)\exp(-\log t K)$
the same equation fulfills. $\Box$



==> Andrey-2007-02-27/3.TEX <==
\section{Equivalence of categories.}
\subsection{Nilpotent connections.}



Recall the notion of a nilpotent connection. Let $({\cal E},\nabla=\nabla_{\cal E})$ be a (holomorphic)
bundle ${\cal E}$ of finite rank with flat connection $\nabla_{\cal E}$ on some (analytic) manifold $X$. We call
the pair $({\cal E},\nabla)$ by {\it connection}. We skip (rather evident) definitions of morphisms of
connections and sub- (quotient-) connections.

The definition of nilpotent connection
is inductive with respect to the rank of the bundle.

{\bf Definition}  The connection $({\cal O}_X, d)$ is the unique (up to isomorphisms) nilpotent connection
of rank $1$.
 A connection $({\cal E},\nabla)$ of rank bigger then one is {\it nilpotent} iff it has a subconnection
isomorphic to $({\cal O}_X, d)$ and the quotient is nilpotent.

{\bf Remark.} One can define nilpotent connections in the following way: first  determine the structure
of irreducible objects (= objects of rank one) and second  postulate that the subcategory of
the nilpotent connections is closed under extensions. 


The nilpotent connections form a  tensor subcategory ${\cal N}ilp(X)$ of the category ${\cal C}onn(X)$
 of the connections. This subcategory is closed with respect
to extensions, subqoutients and inner $Hom$'s.


Analogously, for an analytic family $\pi\colon {\cal X}\to B$ we can define relatively nilpotent connections.

{\bf Definition.} The category of relatively nilpotent connections ${\cal N}ilp({\cal X}\to B)$ is 
the closed under extensions subcategory of the category  ${\cal C}onn({\cal X})$
generated by pullbacks $\pi^*{\cal C}onn(B)$ of connections on $B$.

As in the absolute case, the category ${\cal N}ilp({\cal X}\to B)$ is a tensor category with inner $Hom$'s.


\subsection{Nilpotent connections on a punctured elliptic curve.}

Denote by $X_\tau$ the complement of the point $0$ in the elliptic curve $E_\tau$.

{\bf Theorem 1.}  The category ${\cal N}ilp(X_\tau)$ of the nilpotent connections on the punctured
elliptic curve $X_\tau$ is equivalent to the category ${\cal M}od-R$ of finite-dimensional modules
over the algebra $R= \Bbb C \ll \bfa ,B\gg$.

{\bf Proof.} Our strategy is the following. First, we define a functor 
${\cal F}= ({\cal P}_\tau,\nabla_{fw})\otimes_R *)$ from  ${\cal M}od-R$ to ${\cal N}ilp(X_\tau)$. 
Here we use that  $({\cal P}_\tau),\nabla_{fw})$ is both a nipotent connection on
$X_\tau$ and a left ${ R}$-module. Second we shall prove several results about this functor $\cal F$:

i) it is essentially surjective: any object in the target category is isomorphic
to some object in the image of $\cal F$;

ii) the functor $\cal F$ is fully faithful: the $Hom$'s betweeen targets are isomorphic to the
$Hom$' between sources.

After this we aplly standard result from the category theory: let ${\cal C}$ and ${\cal C}'$ be 
two categories and let ${\cal F}$ be a essentially surjective fully faithful
functor from ${\cal C}$ to ${\cal C}'$; then ${\cal C}$ and ${\cal C}'$ are equivalent.

We can rewrite the action of the functor  ${\cal F}=Hom_{ R}(({\cal P}_\tau,\nabla_{fw}),*)$ as followes.


Let $V$ be a finite-dimensional $R$-module, so it is a vector space with an action of two  operators
$\bfa$ and $B$. As this action continues to an action of formal power series in 
$\bfa$ and $B$, this operators are simultaneously nilpotent: any rather long word in
 $\bfa$ and $B$ acts by zero. Indeed, in opposite case there are infinitely many words 
acting by nonvanishing operators; so exists a formal power series which produces a divergent 
series of operators.


Associate to $V$ the vector bundle ${\cal V}_\tau$ on $E_\tau$
with the fiber $V$ and multipliers $\exp (-2\pi i \bfa ) $ and $1$. Define a connection
$\nabla_\tau$ on ${\cal V}_\tau$ by the same formula as $\nabla_{fw}$:
$\nabla_\tau=d- {\rm ad}_{\bfa} F(\xi , {\rm ad}_{\bfa} ;\tau )B d\,\xi $.
Then ${\cal F}(V)$ is equal to $({\cal V}_\tau, \nabla_\tau)$. Indeed, we indentify
$V$ with $R\otimes_R V$ by sending $v\in V$ to $1\otimes v$; as
 $x\otimes v=1\otimes xv$,   the left multiplication by some element $y$ of $R$ on
 the first factor is
 equivalent to the  action of this element on $v$: $(y\times 1)\otimes v=1\otimes (yv)$.  


{\bf Lemma.} The connection $({\cal V}_\tau,\nabla_\tau)$ is nilpotent.

{\bf Proof.} The intersection $K=H(V)={\rm Ker} \bfa\cap {\rm Ker}B$ of the kernels
of $\bfa$ and $B$ is not zero. In the opposite case $B(v)\neq 0;\forall v\in {\rm Ker}\bfa\setminus 0$;
as $\bfa$ is nilpotent, for some $n$ $\bfa^nB(v)\in {\rm Ker}\bfa\setminus 0$; by iterating
we get infinitely many nonzero operators which are words in $\bfa$ and $B$.

The algebra $R$ acts on $K$ trivially, so the corresponding connection is just the trival one $(K\otimes{\cal O},
d)$ and the quotient corresponds to the representation $V/K$, by induction we get nilpotency of the connection.

Note that $K(V)$ is nothing more that the zeroth cohomology group $H^0(R,V)$ of $R$ with coefficients in $V$.

{\bf Lemma A.} The map $H^0(R,V)= H^0(X_\tau,{\cal F}(H^0(R,V)))\to H^0(X_\tau,{\cal F}(V)) $ is an isomorphism.
The second map  above  is induced by embedding $H^0(R,V) \to  V$.

{\bf Proof.} Induction in the maximal length $l(V)$ of a word in $\bfa$ and $B$ which nonzero acts on $V$.
If $l(V)=0$ then  $R$ acts trivally, so  $H^0(R,V)=V$; on the other hand, ${\cal F}(V)$ is a trivial bundle $V\otimes
{\cal O}$
with the trivial connection $d$, so the space of  its horizontal sections $H^0(X_\tau,{\cal F}(V))$ equals
$V$. The length of the quotient module $V'=V/H(V)$ is one less then the length of $V$.  
Consider the module $V'$ and denote by $H'=H(V')$.   Denote by
$\tilde{H}$ the preimage of $H'$ in $V$ under the map $V\to V/H=V'$. $\tilde{H}$ is a $R$-module, as $\bfa$ and $B$ acts
on $H$ by zero, we have a map $H'\otimes <\bfa,B>_{\Bbb C}\to H$. The partially dual map 
$H'\to H\otimes <\bfa,B>^{\vee}_{\Bbb C}$ is injective as the simultaneous kernel of $\bfa$ and $B$ on $\tilde{H}$
is $H$. Choose some spliting $i\colon H'\to \tilde{H}$ of the sequence 
$0\to H\to \tilde{H}\to H'\to 0$ of vector spaces.

By induction assumptions, the  horizontal sections of ${\cal F}(V')$
are constant sections of ${\cal F}(H')$, so we can identify them with vectors in $H'$.
Let $s$ be some horizontal section of ${\cal F}(V)$, denote by $v'\in H'$ the corresponding
horizontal section of ${\cal F}(V')$, put $v\in \tilde{H}\in V$ the vector $i(v')$. $s(v)=v+E_1(\xi)\bfa (v)$ is a
section of the bundle  ${\cal F}(V)$ (it has required quasiperiodicity), the difference $s-s(v)$ is a 
section of ${\cal F}(H)$, so it is $H$-valued elliptic function $f=f(\xi)$. We have $s=s(v)+f$.
As it is horizontal, $\nabla(s(v)+f)=-B(v)d\,\xi +d\,E_1(\xi)\bfa (v)+d\,f$ is equal to zero.
But space spanned by constants and $d\,E_1$ dos not contain differential of elliptic functions,  so
$B(v)$ and $a(v)$ are zero, hence $v=0$ and section $s$ belongs to the trivial subbundle
${\cal F}(H)$. The horizontal section of it are equal to vectors in $H$. This ends the proof of
the lemma.

{\bf Remark.} The consideration above can be reinterpret in more homological way. Namly, one can prove
by induction that $H^0(X_\tau,{\cal F}(V))=H(V)$ and $H^1(X_\tau,{\cal F}(V))=V/(RV)\otimes <\bfa,B>^{\vee}_{\Bbb C}$.
The main consideration  of the inductive step is that 
for long exact sequence induced by
$$0\to {\cal F}(H)\to {\cal F}(V)\to {\cal F}(V')\to 0$$
the connecting homomorphism 
$H^0(X_\tau,{\cal F}(V'))\to H^1(X_\tau,{\cal F}(H))$ is injective.

We shall use this lemma for the proof of the second  property of the functor $\cal F$ -- that it is
fully faithful. An additional argument in this proof is the comparison of inner $Hom$'s. In general, for
modulas over noncomutaive rings the inner $Hom$ does not exist. We define the structure of $R$-module
on the vector space $Hom_{\Bbb C}(V_1,V_2)$ for modules $(V_1,\rho_1)$ and $(V_2,rho_2)$ by the following rule 
$\rho_{Hom}(x)(L)=\rho_2(x)\circ  L-L\circ\rho_1(x)$ for generators $\bfa$ and $B$ and continue $\rho_{Hom}$
to $R$ by multiplicativity. In other words, this is inner $Hom$ in the category of 
representation of free {\bf Lie algebra} generated by $\bfa$ and $B$. Note that $H^0(R, {cal H}om (V_1,V_2))=
Hom_R(V_1,V_2)$, Indeed a $\Bbb C$-linear map $L$ from $V_1$ to $V_2$ is $R$-linear iff
$\rho_2(x)\circ  L=L\circ\rho_1(x)$, $x=\bfa,B$.

{\bf Lemma B.} The functor $\cal F$ is compatible with inner $Hom$'s:
${\cal F}({\cal H}om(V_1,V_2))={\cal H}om({\cal F}(V_1),{\cal F}(V_2))$; in the lhs ${\cal H}om$ denotes
the inner $Hom$ in the category of $R$-modules, in the r.h.s -- in the category of nilpotent connections
on $X_\tau$.

{\bf Proof.} This fact becames evident if we take in account that formulas defining this functor contains
only $\bfa$, $B$ and their commutators, so they lie in the free Lie algebra generated by $\bfa$ and $B$.


As maps of nilpotent connections coincide with the sections of inner $Hom$, by application of Lemma A we
get the following result.

{\bf Proposition.} The functor $\cal F$ is fully faithfull. 






\section{The equivalence for families.}

In this section we present a description of the relatively nilpotent connections on the universal 
punctured elliptic curve $\pi \colon {\Bbb X}\to {\Bbb H}$ in the same spirit as in the case
of an induvidual curve.

\subsection{Sheaves of free algebras} 

Consider    a trivial (pro)boundle  ${\cal R}$ on $\Bbb H$ with fiber $R$ and equpped with the action of $SL_2(\Bbb Z)$
  by formulas: $\bfa \to \bfa'=\frac{\bfa }{c\tau +d}$, 
$B\to B'=(c\tau +d)B +2\pi i c \bfa$. Equip  this bundle by $SL_2(\Bbb Z)$-invariant connection 

$$\nabla_{\frak R}=d\,    
+\omega_B 
\frac{\partial\,}{\partial\, B}+\omega_{\bfa}
\frac{\partial\,}{\partial\, \bfa },$$

$$\omega_B =-\frac12\frac{1}{2\pi i}
\frac{\alpha_1\alpha_2}{\alpha_1+\alpha_2}
\left(\left(\wp(\alpha_1)-\frac1{\alpha_1^2}\right)
-\left(\wp(\alpha_2)-\frac1{\alpha_2^2}\right)
\right)(B,B)d\,\tau,\quad 
\omega_{\bfa} =-\frac1{2\pi i} Bd\,\tau,
$$

We denote  this (pro)connection $({\cal R},\nabla_{\frak R})$ by ${\frak R}$

{\bf Remark.} Note that the term  $\omega_{\bfa}
\frac{\partial\,}{\partial\, \bfa }$ corresponds to the connection on the
tensor algebra of the first homology group eqipped by Gau\ss-Manin connection.

One can also consider the (sub)bundle $\cal L$ of free Lie algebras generated by $\bfa$ and $B$;
$SL_2(\Bbb Z)$ acts on it.  
Moreover, $\cal L$ is invariant under the connection $\nabla_{\frak R}$

For any ${\cal R}$-valued  one-form  $\mu$ on an open subset $U$ of $\Bbb H$ one can twist the connection
$\nabla_{\frak R}$ by $\mu$: $\nabla^\mu_{\frak R}=\nabla_{\frak R}-{\rm ad}_\mu$, im $\mu$ takes values
in subbundle of Lie algebras $\frak L$, $\nabla^\mu_{\frak R}$ preserves this subbundle. The connection
$({\cal R},\nabla^\mu_{\frak R})$ over $U$ we denote by ${\frak R}^\mu$. If $U=\Bbb H$ and the form
 $\mu$ is $SL_2(\Bbb Z)$-invariant,
then  ${\frak R}^\mu$ is $SL_2(\Bbb Z)$-invariant; if $\mu$ is invariant under some subgroup $\Gamma$
of $SL_2(\Bbb Z)$,  ${\frak R}^\mu$ is $\Gamma$-invariant.

\subsection{${\frak R}$-modules and relatively nilpotent connections.}

In this susection we generalize the functor $\cal F$ for the relative case. 

Let ${\Bbb V}$ be a  connection over an open subset $U$ of $\Bbb H$ which is a (right) module over (restriction of)
$\frak R$. Put  $${\cal F}(\Bbb V)= ({\cal P}, \nabla_{\cal P})\otimes_{\pi^*{\frak R}}\pi^*\Bbb V;$$
where we use an evident structure of the left  $\pi^*{\frak R}$-module on $\cal P$. ${\cal F}(\Bbb V)$ is
a connection on $\pi^{-1}(U)$. If $U=\Bbb H$ and the connection $\Bbb V$ is $\Gamma$-invariant,
then  ${\cal F}(\Bbb V)$ is $\Gamma$-invariant, $\Gamma$ be a subgroup of the $SL_2(\Bbb Z)$.

More explicitly, $\Bbb V$ goes under functor $\cal F$ to the connection $({\cal V}, \nabla_{\cal V})$ where
$\cal V$ be a bundle on $\Bbb E$  which is just a pull-back of $\Bbb V$ on $\Bbb H\times \Bbb C$ glued
by multipliers $\exp(-2\pi i \bfa)$ and $1$ under the shifts by $\tau$ and $1$ respectively. 
The connection $\nabla_{\cal V}$ is defined as followes: 

$$\nabla_{\cal V}=\nabla_{\Bbb V}+\nu;\quad
\nu=-\left(\alpha F(\xi , \alpha ;\tau ) d\,\xi
+\frac{1}{2\pi i}\left(\alpha F'_2(\xi , \alpha ;\tau )+
\frac{1}{\alpha}\right)d\,\tau\right)B;$$
where $\nabla_{\Bbb V}$ denotes the connection on the pull-back $\pi^*\Bbb V$.


Evidently, we can generalize this functor to the case of ${\frak R}^\mu$-modules with replacing
$({\cal P}, \nabla_{\cal P})$ by $({\cal P}, \nabla_{\cal P}^\mu)$.

{\bf Lemma.} Let $\xi(\tau):U\to \pi^{-1}U$ be a section of $\pi:\pi^{-1}U\to U$. Put $\mu =\nu|_{\xi}$.
Then the restriction ${\frak R}^\mu(\Bbb V)|_\xi$ of the connection ${\frak R}^\mu(\Bbb V)$ to $\xi$
coincides with $\Bbb V$.

{\bf Proof.} The connection $\nabla_{\cal V}^\mu$ associated to ${\frak R}^\mu(\Bbb V)$ expresses as 
$\nabla_{\Bbb V}+\nu -\mu,$, so its restriction is $\nabla_{\Bbb V}+\nu|_{\xi} -\mu=\nabla_{\Bbb V}$.

Now we shall prove that locally in base this functor presents an equivalence of categories.
The proof of fully faithfulness is analogous to the proof in the case of induvidual curve, and
we leave it as exercise for the reader. The Essentual surjectivity followes from the following consideration.  

Let $({\cal V}, \nabla)$ be a relative nilpotent connection on $P\colon U\to \Bbb H$ with finite order pole at zero
section. we shall prove that it has the required form.

Its restriction to any 
fiber of $p$ is a nilpotent connection, so according to Theorem  A we can associate to this restriction
a vector space $V$ with action of two operators $\bfa$ and $B$. As this restriction forms a family
of connection, we have a family of operators $\bfa(\tau)$, $B(\tau)$ acting on $V$.
So, the connection $\nabla$ can be written as $d-\nu(\bfa,B) -\Phi(\xi, \tau)d\,\tau$ by formal subtraction and addition of 
the expression $\nu$.

As $\nabla$ is flat, $\Phi$ must be holomorphic, this statement can be obtained by calculation of the singular part
of curvature near zero section.

From the quasiperiodicity  with respect to $\xi\to \xi+\tau$, $\xi\to \xi+1$ we get
$$\Phi(\xi+\tau, \tau)-\exp(-2\pi i\alpha)\Phi(\xi, \tau)=-\frac{\exp(-2\pi i\alpha)-1}{-\alpha}\left(\frac d{d\,\tau}\bfa 
+\frac B{2\pi i}\right),$$
$$
\Phi(\xi+1, \tau)=\Phi(\xi, \tau).$$

{\bf Lemma.} $\Phi(\xi, \tau)$ does not depends in $\xi$.

{\bf Proof.} Denote by $K$  the expression $\left(\frac d{d\,\tau}\bfa 
+\frac B{2\pi i}\right)$. The function $-(F(\xi, \alpha)-\frac 1\alpha)K$ satisfies the required quasiperiodicity, so
$\Phi(\xi,\tau)+(F(\xi, \alpha)-\frac 1\alpha)K$ satisfies the homogenious equations, so equals to $\alpha F(\xi, \alpha)C$
for some $C(\tau)$. As $\Phi(\xi, \tau)=\alpha F(\xi, \alpha)C(\tau)-(F(\xi, \alpha)-\frac 1\alpha)K$ is holomorphic, 
the singilar part
$(\alpha C(\tau)-K)frac 1\xi$ at $\xi=0$ vanishes, so $K=\alpha C(\tau)$ and $\Phi(\xi, \tau)=C(\tau)$

So we get 
$$\frac{\exp(-2\pi i\alpha)-1}{-\alpha}\left(-\alpha \Phi(\tau)\right)=\frac{\exp(-2\pi i\alpha)-1}{-\alpha}\left(\frac d{d\,\tau}\bfa 
+\frac B{2\pi i}\right).$$
as $\bfa$ is nilpotent, the operator $\frac{\exp(-2\pi i\alpha)-1}{-\alpha}$ is invertible, so we get
 $ \frac d{d\,\tau}\bfa 
 -[\Phi, \bfa]=-\frac B{2\pi i}$.
 
 Now we calculate the curvature of $\nabla$. The calculation is parallel to the calculation of the curvature
 of the connection on $\cal P$.
 We get $d\,(\Phi(\tau)d\,\tau) =0$ and
 $$d\, \nu = -\left(\frac{\partial \bfa}{\partial \tau}\frac{\partial }{\partial \bfa} 
 +\frac{\partial B}{\partial \tau}\frac{\partial }{\partial B}\right)\nu \wedge d\,\tau=$$
 $$
  \left(\left(-\frac{B}{2\pi i} +[\Phi, \bfa]\right) 
\frac{\partial}{\partial\,  \bfa }+\frac{\partial B}{\partial \tau}\frac{\partial }{\partial B}\right)
\alpha F(\xi , \alpha ;\tau ) B
  d\,\xi
\wedge d\,\tau= 
  $$
 
 $$ \frac{
(\alpha_1+\alpha_2) F(\xi , \alpha_1+\alpha_2 ;\tau )
- \alpha_2 F(\xi ,  \alpha_2 ;\tau )}{\alpha_1} 
\left(\left(-\frac{B}{2\pi i} +[\Phi, \bfa]\right),B\right)d\,\xi
\wedge d\,\tau
$$
$$+ \alpha F(\xi , \alpha ;\tau )\frac{\partial B}{\partial \tau}d\,\xi
\wedge d\,\tau$$

The term $\nu\wedge\nu$ equals, up to factor $\frac12\frac{d\,\xi\wedge d\,\tau}{2\pi i}$,
$$\left({\alpha_1\alpha_2}   F(\xi , 
\alpha_1+\alpha_2 ;\tau )  \left(\wp(\alpha_1) 
-\wp(\alpha_2) \right) +\frac{\alpha_1F(\xi , 
\alpha_1  ;\tau )}{\alpha_2}-\frac{\alpha_2F(\xi , 
\alpha_2  ;\tau )}{\alpha_1}
\right)(B,B) .$$

The term $\nu\wedge (\Phi(\tau)d\,\tau)+ (\Phi(\tau)d\,\tau)\wedge \nu$ is equal to
$$[\alpha F(\xi , \alpha ;\tau )B,\Phi(\tau)]d\,\xi
\wedge d\,\tau=\alpha _1F(\xi , \alpha _1;\tau )(B,\Phi(\tau))d\,\xi
\wedge d\,\tau.
$$

Finally, the curvature  equals, up to factor $\frac12\frac{d\,\xi\wedge d\,\tau}{2\pi i}$,
$$  \alpha F(\xi , \alpha ;\tau )\left(
\frac{\alpha_1\alpha_2}{\alpha_1+\alpha_2}
\left(\left(\wp(\alpha_1)-\frac1{\alpha_1^2}\right)
-\left(\wp(\alpha_2)-\frac1{\alpha_2^2}\right)
\right)(B,B) +4\pi i \left(\frac{\partial B}{\partial \tau}-[\Phi(\tau),B]
\right)\right).$$

As the operator $\alpha F(\xi , \alpha ;\tau )$ is invertable, the flatness of connection is equivalent to the
condition  
$$\frac{\partial B}{\partial \tau}-[\Phi(\tau),B]=-\frac12\frac{d\,\xi\wedge d\,\tau}{2\pi i}
\frac{\alpha_1\alpha_2}{\alpha_1+\alpha_2}
\left(\left(\wp(\alpha_1)-\frac1{\alpha_1^2}\right)
-\left(\wp(\alpha_2)-\frac1{\alpha_2^2}\right)\right).$$


==> Andrey-2007-02-27/4.TEX <==
\subsection{ The universal connection on the elliptic curves with several punctures.}

 
Let $\eta_0=0,\eta_1, \cdots,\eta_n$ are mutually different  points on the elliptic curve $X_\tau$, we will often
identify the with their preimages in $\Bbb C$.

Associate to each $\eta_i$ a new formal variable $K_i$. Put $R^{(n)}=\Bbb C\ll \bfa ,B, K_i\gg $.
As above, define a (pro) vector bundle ${\cal P}^{(n)}_\tau$ on $E_\tau$
with fiber $R^{(n)}$ by multipliers  
$\exp (-2\pi i \bfa ) $ and $1$.

{\bf Proposition 1.} The differential operator  
$$\nabla_{fw}=d- \alpha F(\xi , \alpha ;\tau )B d\,\xi -\sum_{i+1}^n (F(\xi -\eta_i,\alpha ;\tau )-F(\xi,\alpha ;\tau ) )
K_i d\,\xi $$
is a connection on ${\cal R}^{(n)}_\tau$ with log singularities at $0$ and $\eta_i$'s.

The proof is parallel to the case $n=0$.

As in the case $n=0$ we can try to lift this connection on the family, in which $\tau$ and $\eta_i$'s play the
role of coordinates on the base of the family.

The   shift $\eta_i \to \eta_i +\tau$ acts on $R^{(n)}$ by $K_i\to \exp(-2\pi i\alpha)K_i$, 
$B \to B +\frac{\exp(-2\pi i \alpha)-1}{\alpha}K_i$
 

 
\subsection{ The universal connection on the square of an elliptic curve.}

We discribe an universal flat connection on the square of the elliptic curve $X=X_\tau$ with logarithmic
singularities at $0\times X$ $X\times 0$ and diagonal $\Delta_X$. 

Put $U^{(2)}=U^{(2)}_\tau=X\times X\setminus
\{0\times X\cup X\times 0\cup \Delta_X\}$. Then $U^{(2)}_\tau$ can be treated as a fiber of the forgetful
map of modular spaces ${\cal M}_{1,3}\to {\cal M}_{1,1}$. The action of the symmetric group ${\frak S}_3$
can be described as permutation of $(\xi_0=0,\xi_1,\xi_2)$ and shifting the first point to zero:
$\sigma:( \xi_0,\xi_1,\xi_2)\to ( \xi_{\sigma(0)},\xi_{\sigma(1)},\xi_{\sigma(2)})
\to ( 0,\xi_{\sigma(1)}-\xi_{\sigma(0)},\xi_{\sigma(2)}-\xi_{\sigma(0)})$.

Consider a noncomutative associative ring $R^{(2)}$ generated by $\bfa^{(i)},B^{(i)}$, $i=1,2$ with relations
$$[\bfa^{(1)},\bfa^{(2)}]=0,\quad [\bfa^{(1)},B^{(2)}]=[\bfa^{(2)},B^{(1)}],\quad [B^{(1)},B^{(2)}]=0;$$
$$[\bfa^{(1)},[\bfa^{(2)},B^{(1)}+B^{(2)}]]=0,\quad [B^{(1)},[B^{(2)},\bfa^{(1)}+\bfa^{(2)}]]=0.$$
Define an action of the symmetric group ${\frak S}_3$ on it as permutation of 
$(\bfa^{(0)}= -\bfa^{(1)}-\bfa^{(2)},\bfa^{(1)},\bfa^{(2)})$ and $(B^{(0)}=-B^{(1)}-B^{(2)},B^{(1)},B^{(2)})$.
It is easy to check that this action preserves the relations. Denote by $\alpha^{(i)}$ the adjoint action
of $\bfa^{(i)}$

Consider a bundle ${\cal P}^{(2)}_\tau$ on $X\times X$ with fiber $R^{(2)}$ defined by multipliers 
$\exp(-2 \pi i\bfa^{(j)})$ with respect to shift $\xi_j\to \xi_j+\tau$ and multipliers $1$  
shift of $\xi$'s by one. It is easy to check that this bundle is ${\frak S}_3$ invariant.

Define a $R^{(2)}$-valued differential form $\nu^{(2)}$ on $\Bbb C^2$ with logarithmic singularities by formula
$$\nu^{(2)}(\xi_1,\xi_2,)=
(\alpha^{(1)}+\alpha^{(2)})F(\xi_1,\alpha^{(1)}+\alpha^{(2)})
(\alpha^{(2)})F(\xi_2-\xi_1, \alpha^{(2)})B^{(1)}d\,\xi_1+$$
$$
(\alpha^{(1)}+\alpha^{(2)})F(\xi_2,\alpha^{(1)}+\alpha^{(2)})
(\alpha^{(1)})F(\xi_1-\xi_2, \alpha^{(1)})B^{(2)}d\,\xi_2$$
 
 
 {\bf Lemma.} The form $\nu^{(2)}$ satisfies to the several properties: 
 
 i) this  form is pull back of a form on the square of the elliptic curve with values in bundle 
 ${\cal P}^{(2)}_\tau$;
 
 ii) this form is ${\frak S}_3$-invariant;
 
 iii) this form is closed: $d\,\nu^{(2)}=0$;
 
 iv) the wedge-square of this form vanishes: $\nu^{(2)}\wedge \nu^{(2)}=0$.
 
 {\bf Proof.} The statement i) followes immediatly from the quasiperiodicity of $F$.
 
 ii) This followes from the following identity (the Fay identity):
 $$ 
 F(\xi_1,\alpha^{(1)} )
 F(\xi_2 , \alpha^{(2)}) =
 F(\xi_1,\alpha^{(1)}+\alpha^{(2)})
 F(\xi_2-\xi_1, \alpha^{(2)}) +
 F(\xi_2,\alpha^{(1)}+\alpha^{(2)})
 F(\xi_1-\xi_2, \alpha^{(1)}).  $$
 
 
 iii) and iv) can be proved by the following consideration. As in the case of the bundle
 ${\cal P}$ over the curve $X$, it is easy to check that the only regular section of ${\cal P}^{(2)}_\tau$
 is zero section. So, it is sufficient to check that  $d\,\nu^{(2)} $ and
 $\nu^{(2)}\wedge \nu^{(2)} $ has no poles. From the ${\frak S}_2$-invariancy it is enough to consider 
 the locus $\xi_1=0$. The singular part of $d\,\nu^{(2)} $ near this locus is equal to
 $$-\frac{\partial F(\xi_2-\xi_1, \alpha^{(2)})}{\partial \xi_2}(\alpha^{(1)}+\alpha^{(2)})\alpha^{(2)}B^{(1)}
 \frac{d\,\xi_1}{\xi_1}\wedge d\,\xi_2=0,$$
 as $(\alpha^{(1)}+\alpha^{(2)})\alpha^{(2)}B^{(1)}$ according to relations in $R^{(2)}$ and 
 $\frac{\partial F(\xi_2-\xi_1, \alpha^{(2)})}{\partial \xi_2}$ is a  Taylor power series in $\alpha^{(2)}$.
 
 The singular part of $\nu^{(2)}\wedge \nu^{(2)} $ near $\xi_1=0$ equals
 
 $$[(\alpha^{(1)}+\alpha^{(2)}) B^{(1)} ,
B^{(2)}+
(\alpha^{(1)}+\alpha^{(2)})F(\xi_2,\alpha^{(1)}+\alpha^{(2)})-1+$$
$$
\alpha^{(1)}F( -\xi_2, \alpha^{(1)})-1)B^{(2)}
]
\frac{d\,\xi_1}{\xi_1}\wedge d\,\xi_2,$$
here we use the relations $(\alpha^{(1)}+\alpha^{(2)})(\alpha^{(2)})^kB^{(1)}=0$, $k>0$,
$(\alpha^{(1)}+\alpha^{(2)})^l(\alpha^{(1)})^kB^{(2)}=0$, $k,l>0$ which hold in $R^{(2)}$. The term
$[(\alpha^{(1)}+\alpha^{(2)}) 
 B^{(1)},
B^{(2)}]$ vanishes, so this singular part equals
$$ [(\alpha^{(1)}+\alpha^{(2)}) B^{(1)} ,
(\alpha^{(1)}+\alpha^{(2)})F(\xi_2,\alpha^{(1)}+\alpha^{(2)})+ 
(-\alpha^{(1)})F( \xi_2, -\alpha^{(1)})-2)B^{(2)}
]
\frac{d\,\xi_1}{\xi_1}\wedge d\,\xi_2.$$
 Hence, it is enough to prove that for $k>0$, $[(\alpha^{(1)}+\alpha^{(2)}) B^{(1)} ,((\alpha^{(1)}+\alpha^{(2)})^k+(-\alpha^{(1)})^k)
 B^{(2)}]=0$, 
 in $R^{(2)}$. An elementary calculation showes that $(x+y)^k+(-x)^k =\phi_k(x,y)x(x+y) +y^k$ for some polinomials
 $\phi_k(x,y)$. We have 
 $$ ((\alpha^{(1)}+\alpha^{(2)})^k+(-\alpha^{(1)})^k)
 B^{(2)}=(\phi_k(\alpha^{(1)},\alpha^{(2)})\alpha^{(1)}(\alpha^{(1)}+\alpha^{(2)})+(\alpha^{(2)})^k)B^{(2)}=
 (\alpha^{(2)})^kB^{(2)},$$
 as $\alpha^{(1)}(\alpha^{(1)}+\alpha^{(2)}) B^{(2)}=0.$ By induction in $k$ we prove that 
 $[(\alpha^{(1)}+\alpha^{(2)}) B^{(1)},(\alpha^{(2)})^kB^{(2)}]=0$. For $k=0$ this is just the relation in 
 $R^{(2)}$. The step of the induction:
 $$[(\alpha^{(1)}+\alpha^{(2)}) B^{(1)},(\alpha^{(2)})^{k+1}B^{(2)}]=
 \alpha^{(2)}[(\alpha^{(1)}+\alpha^{(2)}) B^{(1)},(\alpha^{(2)})^kB^{(2)}]-$$
 $$
 [\alpha^{(2)}(\alpha^{(1)}+\alpha^{(2)}) B^{(1)},(\alpha^{(2)})^kB^{(2)}]=0,$$
 as $\alpha^{(2)}(\alpha^{(1)}+\alpha^{(2)}) B^{(1)}=0$. $\Box$
 
 The previous lemma implies that the differential operator $d\, - \nu^{(2)}$ defines a ${\frak S}_3$-invariant
 flat connection $\nabla^{(2)}_\tau$ on 
 the restriction of 
 ${\cal P}^{(2)}_\tau$ to $U^{(2)}$ with logarithic singularities.
 
 {\bf Remark.} By using the pair $({\cal P}^{(2)}_\tau,\nabla^{(2)}_\tau$  one can describe the category of
 nilpotent connections on $U^{(2)}$ in the same manner as in section ... the category of
 nilpotent connections on $U$ was described by ${\cal P},\nabla_\tau$.
 
 
 \subsection{Elliptic hexagon equation.}
  
In the subsection we derive an equation on the parellel transports on the elliptic curve $X_\tau$. Our strategy is
like in the original Drinfelds paper .... We consider a {\it contractible} loop $\gamma^{(2)}$ on $U^{(2)}$,
the parallel transport along it with respect to $\nabla^{(2)}_\tau$ is $1$ as the loop is contractible and
the connection is flat. On the other hand, we express this transport as product of six parallel transports 
along the paths on the singular locus of the connection  $\nabla^{(2)}_\tau$. This get us an equation.


We start by some generalities about the description of horizontal sections near singularities of connection which
generalize our  consideration for defenition of the regularized parallel transport.

Recall (see the discussion about differential equations for parallel transport)
that if $D$ be a smooth divisors defined by equation $t=0$ and if $\nabla=d+\nu$ by a flat connection with
logarithmic singularity  at $D$ then we can define a "restriction" $\nu|_{(D,t)}$ of the form $\nu$ to divisor
as $(\nu-K(\nu) d\,\log t)|_D$, $K={\rm Res}_D$. Denote by $\nabla|_{(D,t)}=d+\nu|_{(D,t)}$ the "restriction" of the connection
to the divisor. Morover, the residue $K(\nu)$ is horizontal with respect to the adjoint action of this connection.
On the other hand, the local equation $t=0$ defines a contraction $p_t$ of some 
neighborhood of $D$ to $D$

{\bf Lemma.} Let the residue $K$ be nilpotent. Let $J$ be a horizontal section of  $\nabla|_{(D,t)}=d+\nu|_{(D,t)}$ on the 
divisor $D$. Then one can "continue" this section to a horizontal section section $S_J$ of $\nabla$ in some 
neighborhood of $D$ of the form $S_J=G\exp(-K\log t)p_t^*J$, $G$ is holomorphic and $G|_D=1$
 
A proof is parallel to the  case $D$ is a point.

Let the singular locus of a logarithmic flat connection $\nabla=d +\nu$ is a normal crossing divisor and let 
locally the equations of two components $D_1$ and $D_2$ of this singular locus are $t_1=0$ and $t_2=0$. 
Then the restrictions of  the residues $K_i={\rm Res}_{D_i}(\nu)|_{D_1\cap D_2}$ commute, as this commutator 
is coefficient of the singular part of the curvature. Let $K_i$ are simultaneuosly nilpotent.

{\bf Lemma.} Let $K_i$ are simultaneuosly nilpotent. Then there exists a $\nabla$-horizontal section $S^{(2)}$ of the
the shape $S^{(2)}=G\exp(-K_1\log t_1 -K_2\log t_2)$, $G$ is holomorphic and $G|_{D_1\cap D_2}=1$.

We leave a proof as an exercise for the reader.

We use such horizontal sections for comparison  of the parallel transports on $U^{(2)}$ with parallel transports
on the components of the singular locus of the connection $\nabla^{(2)}$. Note that this locus is not a divisor 
with normal crossing on $X\times X$, so for application of the lemmas we shall blow up the point $(\xi_1=0, \xi_2=0)$,
denote the result of this blow up by $X^{(2)}$. So, the singular locus of   $\nabla^{(2)}$ on 
$X^{(2)}$ is union of the exceptional divisor $X_{012}$ 
and three elliptic curves $X_{ij}$, $i< j=0,1,2$; the exceptional divisor is a rational curve, the elliptic curves
$X_{ij}$ are proper preimages of the curves $\xi_i=\xi_j$ ($\xi_0=0$). We introduce a coordinate $x=\xi_1/\xi_2$ 
on the rational curve $X_{012}$, in this coordinate the intersections with $X_{01}$, $X_{12}$ and $X_{02}$
are the points $0$, $1$ and $\infty$ correspondently. On $X_{ij}$ the intersection with $X_{012}$ is
the point $\ne$.

Denote by $\Delta^2$  a triangle $0\le t_1\le t_2 \le 1$; consider the blow up   of 
the affine plane $\Bbb R^2$ at the vertices
$(0,0)$, $(0,1)$ $(1,1)$ of the triagle
$\Delta^2$. Take the (topological) closure $\Delta^{(2)}$  in this blow up of the open triangle
$0< t_1< t_2 < 1$.  This closure $\Delta^{(2)}$ is a hexagon, three sides of this hexagon are the sides 
$\Sigma_{01}= \{t_1=0\}$, $\Sigma_{12}=\{t_1=t_2\}$ and $\Sigma_{02}=\{t_2=1\}$ of triangle $\Delta^2$, extra three 
sides $\Sigma_{012}^{\lambda\mu}$, $\lambda<\mu=0,1,\infty$  lie on the exceptional divisors 
(preimages of the vertices of the triangle, $\Sigma_{012}^{01}$ over $(0,0)$,
$\Sigma_{012}^{0\infty}$ over $(0,1)$ and $\Sigma_{012}^{1\infty}$ over $(1,1)$). The labeling of the sides
will be motivated bellow. 

Consider the following piecewise-smooth  contractible loop $\sigma$  in the interior of the hexagon $\Delta^{(2)}$;
this loop   is the union of six smooth paths $\sigma_*^*$
which connect points   near the vertices of the hexagon, any path $\sigma_*^*$ is close to the corresponding side
$\Sigma_*^*$ of the hexagon.

 Associate to a smooth loop $\gamma:[0,1]\to X, \gamma(0)=\gamma(1)=\ne$ without self-intersections
 its ``iteration'' $\gamma^2:
\Delta^2\to X\times X, (t_1,t_2)\to (\gamma(t_1),\gamma(t_2))$. The  map $\gamma^2$   determines a map of the 
open triangle  into $U^{(2)}$, so this map induces a map $\gamma^{(2)}$ of the closure $\Delta^{(2)}$ of the triangle
to the  $X^{(2)}$. The boundary of the hexagon $\Delta^{(2)}$ maps to the singular locus of the connection
$\nabla^{(2)}$; $\Sigma_{ij}$ maps to the path $\gamma$ on $X_{ij}$,  $\Sigma_{012}^{\lambda\mu}$ maps to the segment
in $X_{012}$ connecting the points $\lambda$ and $\mu$. This motivate notation for the sides of the hexagon.

As  the loop $\sigma$ in the hexagon $\Delta^{(2)}$ is contractible, the loop $\gamma^{(2)}\circ \sigma$ 
in $U^{(2)}$ is  
contractible; therefore the parallel transport
along it equals to $1$. On the other hand, the loop $\sigma$ is closed to the boundary of the hexagon $\Delta^{(2)}$
and this boundary maps to the singular locus of connection; so, we can apply assimptotic formulas for the
horizontal sections near singularities. 

We shall equipp a component of the singular locus with equation of this component. Globally this is impossible,
as the normal bundle is nontrivial. For elliptic curves $X_{ij}$ we choose such an equation on the universal 
covering of $X^{(2)}$. For the rational curve $X_{012}$ we have three paths along which we calculate parallel 
transport. Each path connect two of marked points $0,1,\infty$.


For sach a path we use a local equation of the component, this equation is valid outside the third marked point.
 


 


==> Andrey-2007-03-03/1.TEX <==
\section{Universal flat connection.}
\subsection{ The basic function.}

\thesubsubsection
 The following function $F(\xi , \alpha , \tau ) $ was introduced by Leopold Kronecker
\begin{eqnarray*}
F(\xi , \alpha , \tau ) =(2\pi i)\left(
1 - \frac {1}{1-z} -\frac{1}{1-w} - \sum_{m,n=1}^{\infty}
(z^m w^n -z^{-m} w^{-n}) q^{mn}\right)\\
\Im \tau >\Im \xi >0,\Im \tau > \Im \alpha > 0;
\end{eqnarray*}
where $q=\exp (2\pi i \tau ) ,\quad
z=\exp (2\pi i \xi ),\quad w=\exp (2\pi i \alpha )$.
Then \cite{Z} $F$ can be continued to a meromorphic function
with poles at divisors $\xi =m+n\tau$ and $\alpha =m' +n'\tau$ and
\begin{equation}
F(\xi ,\alpha ;\tau )=\frac{\theta'(0;\tau ) \theta(\xi + \alpha ;\tau )}
{  \theta (\xi ;\tau ) \theta (\alpha ;\tau )}. \label{theta}
\end{equation}
The transformation  properties of $F(\xi ,\alpha ;\tau )$ are very
simple:
\begin{eqnarray}
F(\xi+1 ,\alpha ;\tau )&=&F(\xi ,\alpha ;\tau );\\
F(\xi +\tau ,\alpha ;\tau )&=
&\exp (-2 \pi i \alpha )F(\xi ,\alpha ;\tau );\\
F(\frac{\xi}{c\tau +d} ,\frac{ \alpha}{c\tau +d} ,
\frac{a\tau +b}{c\tau +d} )&=&
(c\tau +d)\exp (2\pi i\frac{c\xi \alpha }
{c\tau +d})F(\xi , \alpha ;\tau ).\label{dermod}
\end {eqnarray}
\thesubsubsection
According to Zagier, $F(\xi , \alpha ;\tau )$ can be expressed
as the exponential of the generating function of Eisenstein functions
$E_k(\xi ;\tau ) =
\displaystyle{\sum\limits_{w\in L}} {}_e \frac{1}{ (w + \xi)^k }$
and Eisenstein series
$e_k(\tau ) =
\displaystyle{\sum\limits_{w\in L}}' {}_e \frac{1}{ (w  )^k }$
($\sum {}_e$ denotes Eisenstein summation \cite{W})
:
\begin{equation}
F(\xi , \alpha ;\tau )=
\frac1{ \alpha}\exp(-\sum _{k=1}^{\infty}\frac{(-\alpha )^k}k
(E_k(\xi ;\tau )-e_k(\tau))).\label{expg}
\end{equation}
This statement is a simple corollary of Zagier's
``Logarithmic Formula'' for $F(\xi ,\alpha ;\tau )$
\cite[Section~3,Theorem(viii)]{Z} and
the power series for $E_n$ \cite[Chapter~III,formula(10)]{W}.

{\bf Remark.} In ... the factor $2\pi i$ wes missed.

From the very definition of the function $F$
it satisfies the ``mixed heat'' equation
\begin{equation}2 \pi i \frac{\partial}{\partial \tau} 
F(\xi , \alpha ;\tau ) =
\frac{\partial^2}{\partial \xi \partial \alpha} 
F(\xi , \alpha ;\tau ).\label{mhe}\end{equation}

We shall use the following identity

$$F(\xi , \alpha _1;\tau )
F'_2(\xi , \alpha_2 ;\tau )-
F(\xi , \alpha_2 ;\tau )F'_2(\xi , \alpha_1 ;\tau )
=F(\xi , \alpha_1+\alpha_2 ;\tau )(\wp(\alpha_1)-
\wp(\alpha_2)),
$$
where $F'_2(\xi , \alpha ;\tau )=\frac{\partial F(\xi , \alpha ;\tau )}{\partial \alpha}$ denotes the derivative with respect to the second argument $\alpha$ and $\wp$ denotes the Weierstra{\ss} function
$\wp =E_2-e_2$.

A proof of the last identity is rather simple.


\subsection{ The connection with
logarithmic singularity on the elliptic curve.}

Let $E_{\tau}$ be an elliptic curve defined as
$\Bbb C/\Bbb Z\tau +\Bbb Z$, $\Im (\tau)>0$.
We fix notation $\xi$ for the coordinate on $\Bbb C$.


Consider an algebra $ R=\Bbb C \ll \bfa ,B\gg$
of noncommutative formal power series in two
variables $\bfa $ and $B$. For any power series $r$
denote by the same symbol 
$r $ the endomorphism of the
left multiplication: $r (r')=rr'$. 

Define a (pro) vector bundle ${\cal P}_\tau$ on $E_\tau$
with fiber $R$ by multipliers  
$\exp (-2\pi i \bfa ) $ and $1$;
so a section of ${\cal P}_\tau$ is an $R$-valued function 
$f(\xi,\bfa , B)$ on $\Bbb C$ such that 
$f(\xi+\tau, \bfa , B)=
\exp (-2\pi i \bfa ) f(\xi, \bfa , B)$,
 $f(\xi+1, \bfa , B)=f(\xi, \bfa , B)$. Hence, an
endomorphism $L$ of the bundle  ${\cal P}_\tau$ is
an ${\rm End}(R)$-valued function $L(\xi )$ on 
$\Bbb C$ such that 
$$L(\xi+\tau )=
\exp (-2\pi i \bfa ) L(\xi )\exp (2\pi i \bfa )=
\exp (-2\pi i {\rm ad}_\bfa ) L(\xi ),$$
$$
 L(\xi+1)=L(\xi);$$ here ${\rm ad}_\bfa $ denotes
the adjoint action of $a$ on $R$: 
${\rm ad}_\bfa (p)=\bfa p-p\bfa $,
denote it by $\alpha={\rm ad}_\bfa $.

Consider an expression $ \alpha F(\xi , \alpha ;\tau )$. We treat it as a function in $\xi$
which takes values 
in formal power series in $\alpha$,
so $ \alpha F(\xi , \alpha ;\tau )B$ takes values
in formal power series in $\bfa $ and $B$ after
substitution $\alpha={\rm ad}_\bfa $, as we have denoted.


The operator $ \alpha F(\xi , \alpha ;\tau )B $
  satisfies to the quasiperiodic properties with
respect to $\xi\to\xi+\tau$ and $\xi\to \xi+1$,
so it is an endomorphism of ${\cal P}_\tau$. It is a meromorphic  function in $\xi$ with simple
pole at $0$. Hence, we prove the following result.

{\bf Proposition 1.} The differential operator  
$\nabla_{fw}=d- \alpha F(\xi , \alpha ;\tau )B d\,\xi $
defines a connection on ${\cal P}_\tau$ with logarithmic
singularity at $0$.
 
\subsection{ The connection  with
logarithmic singularity on the family of
elliptic curves.} 

We can treat the parameter $\tau$ of the elliptic
curve as a variable, so we get a family $\Bbb E$ of
elliptic curves over the upper-half-plane
$\Bbb H=\{\tau |{\Im \tau}>0\}$. Furthermore
we define a bundle with the fiber $R$ on $\Bbb E$ by
the same rule as in the case of the individual curve;
denote it  by $\cal P$. 
We shall lift
the fiberwise connection $\nabla_{fw}$ to 
a {\it flat} connection $\nabla_{\cal P}$ on $\cal R$
over {\it the surface $\Bbb E$}.

First we introduce same convenient for us notation.
Let $\bfa $ $B$ and $C$ be elements of some 
pronilpotent Lie algebra. we use notation
$\alpha$ for ${\rm ad}_\bfa $; denote by $\alpha_1^{i}
\alpha_2^{j}\odb B,C\cdb$ the element $[{\rm ad}_\bfa ^iB,
 {\rm ad}_\bfa ^jC]$. We extend such a notation 
to formal power series $f(\alpha_1, \alpha_2)$ 
in two 
{\it commutative} variables  $\alpha_1,\alpha_2$.
The Jacobi identity yields the equality
$\alpha f(\alpha_1, \alpha_2)\odb B,C\cdb=
(\alpha_1+\alpha_2) f(\alpha_1, \alpha_2)\odb B,C\cdb$.

Note, that if $C=B$, the symmetric 
($f(\alpha_1, \alpha_2)=f(\alpha_2, \alpha_1)$)
power series produces zero; in this case
it is reasonable to consider only
antisymmetric power series.

{\bf Lemma 1.} Let $D$ be a differentiation of the
Lie algebra. Then
$$D\, (f(\alpha)B)= 
\frac{f(\alpha_1+\alpha_2)-f(\alpha_2)}{\alpha_1}
\odb D\,(\bfa ),B\cdb +f(\alpha)D\,(B). $$
 
{\bf Proof.} It is sufficient to check this formula
for $f(\alpha)=\alpha^i$. For $i=0$ the statement 
is evidently true. By induction:
$$D\,(\alpha^i(B))=[D(\bfa ), \alpha^{i-1}(B)]+
\alpha d\,(\alpha^{i-1}(B))=$$
$$
\alpha_2^{i-1}(D(\bfa ),B)+(\alpha_1+\alpha_2)
\frac{(\alpha_1+\alpha_2)^{i-1}-
\alpha_2^{i-1}}{\alpha_1}
\odb D\,(\bfa ),B\cdb +\alpha(\alpha)^{i-1}D\,(B)=
$$
$$\frac{(\alpha_1+\alpha_2)^{i}-
\alpha_2^{i-1}}{\alpha_1}
\odb D\,(\bfa ),B\cdb +(\alpha)^{i}D\,(B).
$$

{\bf Lemma 2.} Let $D$ be a differentiation of the
Lie algebra. Then in the universal enveloping
the following equality holds
$$D(\exp(\bfa ))=
\exp(\bfa )\frac{\exp(-\alpha)-1}{-\alpha}D(\bfa ).
$$ 

 


 Now we are able to define the connection 
$\nabla_{\cal P}$.  Put 
$$\omega_B =-\frac12\frac{1}{2\pi i}
\frac{\alpha_1\alpha_2}{\alpha_1+\alpha_2}
\left(\left(\wp(\alpha_1)-\frac1{\alpha_1^2}\right)
-\left(\wp(\alpha_2)-\frac1{\alpha_2^2}\right)
\right)\odb B,B\cdb d\,\tau,\quad 
\omega_{\bfa} =-\frac1{2\pi i} Bd\,\tau,
$$
$$\nu=
-\left(\alpha F(\xi , \alpha ;\tau ) d\,\xi
+\frac{1}{2\pi i}\left(\alpha F'_2(\xi , \alpha ;\tau )+
\frac{1}{\alpha}\right)d\,\tau\right)B.$$
Then
$$\nabla_{\cal P}=d\,  +\nu  
+\omega_B 
\frac{\partial\,}{\partial\, B}+\omega_{\bfa}
\frac{\partial\,}{\partial\, \bfa },$$
where
$f\frac{\partial\,}{\partial\, B}$ (and 
$f\frac{\partial\,}{\partial\, \bfa }$) is the {\it 
differentiation} on $R$, so
$f\frac{\partial\, r_1r_2}{\partial\, B} =f
\frac{\partial\, r_1}{\partial\, B}  
r_2+r_1f\frac{\partial\, r_2}{\partial\, B}$
 (no term
$[\omega_B,r_1]
\frac{\partial\, r_2}{\partial\, B}$!!!). Hence the commutator 
$[f\frac{\partial\,}{\partial\, B},r ]$
 of $f\frac{\partial\,}{\partial\, B}$
and $r $ is just $f\frac{\partial\,r}{\partial\, B}  $


{\bf Proposition 2.} The operator $\nabla_{\cal P}$ 
is a connection on $\cal P$.

{\bf Proof.} We must check that $\nabla_{\cal P}$
is invariant with respect to shift $\xi\to\xi +1$
and that $\nabla_{\cal P}$ transforms in correct
way under shift $\xi \to \xi+\tau$. The first 
property
followes immediately from the invariance of $F$ with
respect to this shift. So we shall check that
$$\nabla_{\cal P}|_{\xi+\tau}=
\exp(-2\pi i \bfa )\nabla_{\cal P}|_{\xi }
\exp(2\pi i \bfa ).$$
The summand $  \nu  $
in the l.h.s. is equal to  
$$  -\left(\alpha F(\xi+\tau , \alpha ;\tau ) d\,(\xi+\tau)
+\frac{1}{2\pi i}\left(\alpha F'_2(\xi +\tau, \alpha ;\tau )+
\frac{1}{\alpha}\right)d\,\tau\right)B =
$$
$$ -\left(\exp(-2\pi i\alpha)(\alpha F(\xi  , \alpha ;\tau ) d\,\xi 
 + \alpha F(\xi  , \alpha ;\tau )d\,\tau) 
\phantom{\frac{1}{\alpha}}\right.
+$$
$$ \left.\frac{1}{2\pi i}\left(\exp(-2\pi i\alpha)(
-2\pi i\alpha F(\xi  , \alpha ;\tau )+\alpha F'_2(\xi +\tau, \alpha ;\tau ))+
\frac{1}{\alpha}\right)d\,\tau\right)B =
$$
$$ -\exp(-2\pi i\alpha)\left(\alpha F(\xi  , \alpha ;\tau ) d\,\xi 
 +  \left( \frac{1}{2\pi i}\left(
 \alpha F'_2(\xi +\tau, \alpha ;\tau )+
\frac{1}{\alpha}\right)+
\frac{\exp(2\pi i\alpha)-1}{2\pi i\alpha}\right)
d\,\tau\right)B .
$$
Other terms in the l.h.s. do not depend in $\xi$;
so they are invariant.

In the r.h.s. the term $\exp(-2\pi i \bfa )
\nu
\exp(2\pi i \bfa )$ is equal to
$$ -\exp(-2\pi i\alpha)\left(\alpha F(\xi  , \alpha ;\tau ) d\,\xi 
 +   \frac{1}{2\pi i}\left(
 \alpha F'_2(\xi +\tau, \alpha ;\tau )+
\frac{1}{\alpha}\right)  
d\,\tau\right)B .
$$

The term 
$ \exp(-2\pi i  \bfa ) \omega_B \frac{\partial\,}{\partial\, B} 
\exp(2\pi i  \bfa )$ equals $\omega_B \frac{\partial\,}{\partial\, B}$ as 
$  \frac{\partial\,\exp(2\pi i a)}{\partial\, B}=0$.

The term  $\exp(-2\pi i  \bfa ) \omega_{\bfa}  \frac{\partial\,}{\partial\,  \bfa } 
\exp(2\pi i  \bfa )$ is equal to

$$\exp(-2\pi i  \bfa ) \left(-\frac1{2\pi i}B \frac{\partial\,}{\partial\,  \bfa }\right) 
\exp(2\pi i  \bfa )
\stackrel{\mbox{Lemma 2.}}{=} \frac{\exp(-2\pi i\alpha)-1}{-2\pi i\alpha} 
(- B)-\frac1{2\pi i}B 
\frac{\partial\,}{\partial\,  \bfa }.   
$$ 
So, the l.h.s. is equal to the r.h.s.

{\bf Proposition 3.} The connection $\nabla_{\cal P}$
is flat.

{\bf Proof.}
Denote by $\omega$ the differential form
$$\nu  
+\omega_B 
\frac{\partial\,}{\partial\, B}+\omega_{\bfa}\frac{\partial\,}{\partial\, a}.$$
 
We shall prove that $d\,\omega+\omega\wedge\omega=0$.
The term $d\,\omega$ is equal to $d\,\nu $, as other terms are lifted from
one dimensional $\Bbb H$, so are closed. So,  $d\,\omega$  equals  
$$-d\, \left(\alpha F(\xi , \alpha ;\tau ) d\,\xi
+\frac{1}{2\pi i}\left(\alpha F'_2(\xi , \alpha ;\tau )+
\frac{1}{\alpha}\right)d\,\tau\right)B=$$
$$\left(
\frac{\partial}{\partial\,\tau}
(\alpha F(\xi , \alpha ;\tau )) -\frac{1}{2\pi i}\frac{\partial}{\partial\,\xi}\left(\alpha F'_2(\xi , \alpha ;\tau )+
\frac{1}{\alpha}\right)\right)d\,\xi\wedge d\,\tau
B
$$
$$\alpha\left( 
\frac{\partial}{\partial\,\tau}
F(\xi , \alpha ;\tau ) -\frac{1}{2\pi i}\frac{\partial}{\partial\,\xi}   F'_2(\xi , \alpha ;\tau )
  \right)d\,\xi\wedge d\,\tau 
B =0,
$$
as the function $F$ satisfies to the mixed heat 
equation.
The term $\omega\wedge\omega$ equals  
$$\left[\alpha F(\xi , \alpha ;\tau ) B,
\frac{1}{2\pi i}\left(\alpha F'_2(\xi , \alpha ;\tau )+
\frac{1}{\alpha}\right)B\right] d\,\xi
\wedge d\,\tau+$$
$$\left[-\frac12\frac{1}{2\pi i}
\frac{\alpha_1\alpha_2}{\alpha_1+\alpha_2}
\left(\left(\wp(\alpha_1)-\frac1{\alpha_1^2}\right)
-\left(\wp(\alpha_2)-\frac1{\alpha_2^2}\right)
\right)\odb B,B\cdb \frac{\partial}{\partial\, B},
\alpha F(\xi , \alpha ;\tau ) B
\right] d\,\xi
\wedge d\,\tau-$$
$$\left[\frac{B}{2\pi i}
\frac{\partial}{\partial\,  \bfa },
\alpha F(\xi , \alpha ;\tau ) B
\right] d\,\xi
\wedge d\,\tau. 
$$
The first summond, up to factor $\frac{d\,\xi\wedge d\,\tau}{2\pi i}$ can be written as
$$
  \alpha_1F(\xi , \alpha_1 ;\tau ) 
 \left(\alpha_2 F'_2(\xi , \alpha_2 ;\tau )+
\frac{1}{\alpha_2}\right)\odb B,B\cdb   =
$$
$$
 \frac12\left(\alpha_1F(\xi , \alpha_1 ;\tau ) 
 \left(\alpha_2 F'_2(\xi , \alpha_2 ;\tau )+
\frac{1}{\alpha_2}\right)
-\alpha_2 F(\xi , \alpha_2 ;\tau ) \left(\alpha_1
F'_2(\xi , \alpha_1 ;\tau )+
\frac{1}{\alpha_1}\right)\right)\odb B,B\cdb ;  
$$
the second one, up to the same factor, equals
$$
-\frac12(\alpha_1+\alpha_2) F(\xi , 
\alpha_1+\alpha_2 ;\tau ) \frac{\alpha_1\alpha_2}{\alpha_1+\alpha_2}
\left(\left(\wp(\alpha_1)-\frac1{\alpha_1^2}\right)
-\left(\wp(\alpha_2)-\frac1{\alpha_2^2}\right)
\right)\odb B,B\cdb ; 
 $$
the third summond can be calculated by application 
of Lemma 1, we get (up to the same factor as above)
$$ -\frac{
(\alpha_1+\alpha_2) F(\xi , \alpha_1+\alpha_2 ;\tau )
- \alpha_2 F(\xi ,  \alpha_2 ;\tau )}{\alpha_1} 
\odb B,B\cdb =
$$
 
$$-\frac12\left(\frac{
(\alpha_2^2-\alpha_1^2) 
F(\xi , \alpha_1+\alpha_2 ;\tau )+
\alpha_1^2 F(\xi ,  \alpha_1 ;\tau )-
\alpha_2^2 F(\xi ,  \alpha_2 ;\tau )}
{\alpha_1\alpha_2}\right) 
\odb B,B\cdb .
$$
Finally, we conclude that the term $\omega\wedge\omega$ is equal to 
$\frac12\frac{d\,\xi\wedge d\,\tau}{2\pi i}
\Xi(\alpha_1,\alpha_2)\odb B,B\cdb $, where
$$\Xi(\alpha_1,\alpha_2)= \alpha_1F(\xi , \alpha_1 ;\tau ) 
 \left(\alpha_2 F'_2(\xi , \alpha_2 ;\tau )+
\frac{1}{\alpha_2}\right)
-\alpha_2 F(\xi , \alpha_2 ;\tau ) \left(\alpha_1
F'_2(\xi , \alpha_1 ;\tau )+
\frac{1}{\alpha_1}\right) -$$
$$
{\alpha_1\alpha_2}   F(\xi , 
\alpha_1+\alpha_2 ;\tau )  \left(\left(\wp(\alpha_1)-\frac1{\alpha_1^2}\right)
-\left(\wp(\alpha_2)-\frac1{\alpha_2^2}\right)
\right)-$$
$$ \frac{
(\alpha_2^2-\alpha_1^2) 
F(\xi , \alpha_1+\alpha_2 ;\tau )+
\alpha_1^2 F(\xi ,  \alpha_1 ;\tau )-
\alpha_2^2 F(\xi ,  \alpha_2 ;\tau )}
{\alpha_1\alpha_2} =$$
 
$$ \alpha_1F(\xi , \alpha_1 ;\tau ) 
  \alpha_2 F'_2(\xi , \alpha_2 ;\tau ) -\alpha_2 F(\xi , \alpha_2 ;\tau )  \alpha_1
F'_2(\xi , \alpha_1 ;\tau )  -$$
$$
{\alpha_1\alpha_2}   F(\xi , 
\alpha_1+\alpha_2 ;\tau )   \left(\wp(\alpha_1) -\wp(\alpha_2)  \right)  =0.$$

So, we have proved the flatness of the connection
$\nabla_{\cal P}$.



Consider the standard action of the modular group 
$SL_2(\Bbb Z)$ on the upper-half-plane $\Bbb H$ and
the relative curve $\Bbb E$ over $\Bbb H$:
$\tau\to \tau' =\frac{a\tau +b}{c\tau +d};\quad
\xi\to \xi'=\frac{\xi}{c\tau +d}$. 
Denote by ${\cal R} $ the (pro)bundle on $\Bbb H$ with the fiber $R$.
Define an action of $SL_2(\Bbb Z)$ on $\cal R$
by the rule:
$\bfa \to \bfa'=\frac{\bfa }{c\tau +d}$,  
$B\to B'=(c\tau +d)B +2\pi i c \bfa$; and  lift this action to an action on $\cal P$ by  multiplier 
$\exp(2\pi i\frac{c \xi \bfa}{c\tau +d})$,
so the a $SL_2(\Bbb Z)$-invariant section of $\cal P$   is
an $R$-valued function $f$ in $\tau$ and $\xi$
such that 

$$f(\frac{a\tau +b}{c\tau +d}, \frac{\xi}{c\tau +d};
\frac{\bfa }{c\tau +d}, (c\tau +d)B +2\pi i c\bfa)=
\exp\left(2\pi i\frac{c \xi \bfa}{c\tau +d}\right) f(\tau, \xi;
\bfa,B).$$

This action is well defined (compatible with the group structure on $SL_2(\Bbb Z)$ and compatible
with fiberwise action of the $\Bbb Z^2$.
We leave these as an exercise to the reader. 

Hence, for an endomorphism we have the same 
condition with replacment $\bfa \to \alpha$.

{\bf Proposition 4.} The connection $\nabla_{\cal P}$
is  $SL_2(\Bbb Z)$ invariant.
 
{\bf Proof.} We shall prove that 

$$\nabla_{\cal P}  |_{\tau', \xi';
\bfa',B'}
=\exp\left(2\pi i\frac{c \xi \bfa}{c\tau +d}\right)\nabla_{\cal P} |_{\tau, \xi;
\bfa,B}\exp\left(-2\pi i\frac{c \xi \bfa}{c\tau +d}\right).$$

The term $\nu$ in the l.h.s. equals
$$
-\left(\frac{\alpha}{c\tau+d} 
F\left(\frac{\xi}{c\tau+d} , 
\frac{\alpha}{c\tau+d} ;\frac{a\tau +b}{c\tau+d} \right) 
d\,\frac{\xi}{c\tau+d}+\right.$$
$$\left.
\frac{1}{2\pi i}\left(
\frac{\alpha}{c\tau+d} 
F'_2(\frac{\xi}{c\tau+d} , 
\frac{\alpha}{c\tau+d} ;\frac{a\tau +b}{c\tau+d} 
 )+
\frac{{c\tau+d}}{ {\alpha}}\right)
d\,\frac{a\tau +b}{c\tau+d} \right)((c\tau +d)B+
2\pi i c\bfa)=
$$
 $$
-\exp\left(2\pi i\frac{c \xi \alpha}{c\tau +d}\right)\left( {\alpha} 
F( {\xi}  , 
 \alpha  ; \tau   ) 
\left(d\, {\xi}-\frac{c\xi}{c\tau+d}d\,\tau\right) -2\pi ic\bfa\left(\frac{d\, \xi}{c\tau+d}-\frac{c\xi 
d\,\tau}{(c\tau+d)^2}\right) +\right.$$
$$\left.
\frac{1}{2\pi i}\left(
 \alpha \left(2\pi i\frac{c\xi}{c\tau+d}F( {\xi}  , 
 \alpha  ; \tau   ) +  
F_2'( {\xi}  , 
 \alpha  ; \tau   ) \right)+
\exp\left(-2\pi i\frac{c \xi \alpha}{c\tau +d}\right)\frac{1}{ {\alpha}}\right)
d\,\tau \right)B
 =
$$
$$\exp\left(2\pi i\frac{c \xi \alpha}{c\tau 
+d}\right)
\nu +\frac{\exp\left(2\pi i\frac{c \xi \alpha}{c\tau +d}\right)-1}{\alpha}d\,\tau B-2\pi ic\bfa\left(\frac{d\, \xi}{c\tau+d}-\frac{c\xi
d\,\tau}{(c\tau+d)^2}\right).$$

In this calculations we use the modular property
of the function $F$ and evident equality
$f(\alpha)\bfa=f(0)\bfa$.


We have  $$\frac{\partial}{\partial B'}=
\frac1{c\tau +d} \frac{\partial}{\partial B},\quad\frac{\partial}{\partial \bfa'}=
(c\tau+d)\frac{\partial}{\partial \bfa }
-2\pi i c\frac{\partial}{\partial B}.$$ 
 As $\omega_B$ is a modular form
of the weight one:
$$\omega_B(\tau', \xi';
\bfa',B') 
=-\frac12\frac{1}{2\pi i}(c\tau +d)
\frac{\alpha_1\alpha_2}{\alpha_1+\alpha_2}
\left(\left(\wp(\alpha_1)-\frac1{\alpha_1^2}\right)
-\left(\wp(\alpha_2)-\frac1{\alpha_2^2}\right)
\right)\times$$
$$
((c\tau +d)B +2\pi i c \bfa,(c\tau +d)B +2\pi i c \bfa)\frac{d\,\tau}{(c\tau+d)^2} =(c\tau+d)
\omega_B(\tau, \xi;
\bfa,B ),$$
the term $\omega_B\frac{\partial}{\partial B}$ is $SL_2(\Bbb Z)$ invariant.

We have also:
$$\omega_{\bfa}(\tau', \xi';
\bfa',B') =-\frac1{2\pi i}((c\tau +d)B +2\pi i c \bfa)\frac{d\,\tau}{(c\tau+d)^2}=\frac1{c\tau +d}
\omega_{\bfa} -  c \bfa\frac{d\,\tau}{(c\tau+d)^2}.
$$

Note that $B'$ and $\bfa'$ depend in $\tau$ 
explicitly as function in $B$ and $\bfa$, so
$$ \left.\frac{ d}{d\,\tau}\right|_{ \bfa',B'}=  \frac{\partial }{\partial\,\tau} -\frac{cB'}{(c\tau +d)^2}
\frac{\partial }{\partial\,B}
+c\bfa'\frac{\partial }{\partial\,\bfa}
$$
Therefore
$$d|_{ \bfa',B'} +\omega_{\bfa}  
({\tau', \xi';
\bfa',B'}) 
\frac{\partial\,}{\partial\, \bfa' }= d|_{\bfa, B}+ 
d\tau\left(
  -\frac{cB'}{(c\tau +d)^2}
\frac{\partial }{\partial\,B}
+c\bfa'\frac{\partial }{\partial\,\bfa}\right)$$
$$\left(\frac1{c\tau +d}
\omega_{\bfa} -  c \bfa\frac{d\,\tau}{(c\tau+d)^2} \right)
(c\tau+d)\frac{\partial}{\partial \bfa }+$$
$$\left(-\frac1{2\pi i}B'\frac{d\,\tau}{(c\tau+d)^2}
\right)\left(-2\pi i c\frac{\partial}{\partial B}\right)=d|_{\bfa, B} +\omega_{\bfa}
\frac{\partial}{\partial \bfa }.
$$

In the r.h.s. we have:
$$\exp\left(2\pi i\frac{c \xi \bfa}{c\tau +d}\right)\left(d -\frac1{2\pi i} Bd\,\tau\frac{\partial\,}{\partial\, \bfa }
\right)\exp\left(-2\pi i\frac{c \xi \bfa}{c\tau +d}\right)=$$
$$d  -
2\pi ic\bfa\left(\frac{d\, \xi}{c\tau+d}-\frac{c\xi 
d\,\tau}{(c\tau+d)^2}\right) +\frac{\exp\left(2\pi i\frac{c \xi \alpha}{c\tau +d}\right)-1}{\alpha}d\,\tau B,
$$
the second summond comes from the differentiation 
by $\xi$ and $\tau$, the last can be calculated
with using Lemma 2.  

Evidently,
$$
\exp\left(2\pi i\frac{c \xi \bfa}{c\tau +d}\right)\nu\exp\left(-2\pi i\frac{c \xi \bfa}{c\tau +d}\right)=\exp\left(2\pi i\frac{c \xi \alpha}{c\tau 
+d}\right)
\nu;$$
and $\omega_B 
\frac{\partial\,}{\partial\, B}$ commutes with
$\exp\left(-2\pi i
\frac{c \xi \bfa}{c\tau +d}\right)$.
This finishes the proof.

Note that such a lifting of fiberwise connection to the flat connection is not unique. Indeed, one can
twist the connection $\nabla_{\cal P}$ by any $R$-valued $SL_{2}(\Bbb Z)$-invariant form  $\mu$ on $\Bbb H$
by the right multiplication on $\mu$:
$$\nabla_{\cal P}^{\mu}(G)=\nabla_{\cal P}(G)+G\mu=\nabla_{\cal P}(G)+\mu G- {\rm ad}_\mu G.$$
This connection is flat as the right and the left multiplications commute.


==> Andrey-2007-03-03/2.TEX <==

{\bf 4. Parallel transports.}

Now we pass to the parallel transports along paths.
Discuss first the general situation.
Let $\nabla$ be a holomorphic connection on a curve  
and let $\gamma$ be a path from a point $\xi_1$
to $\xi_2$. Recall that the {\it parallel transport}
${\cal J}^{\gamma}(\xi_1,\xi_2)$ from the point $\xi_1$
to the point $\xi_2$ along the path $\gamma$ is
an operator from the fiber over $\xi_1$ to the
fiber over $\xi_2$ which is the horizontal 
continuation of the identical map on the fiber
over $\xi_1$ along the path $\gamma$. In the other words,  ${\cal J}^{\gamma}(\xi_1,\xi_2)$ is the solution
of an equation $\nabla 
{\cal J}^{\gamma}(\xi_1,\xi_2)=0$, 
here $\nabla$ acts on the second argument of ${\cal J}$
with initial data ${\cal J} (\xi_1,\xi_1)=1$

In the case under consideration
the  connection $\nabla_{fw}$ acts by multiplication by some formal power series
from the left, so the parallel transport is   the multiplication from
the left by  another formal power series, this power series we
denote by the same symbol  ${\cal J}^{\gamma}(\xi_1,\xi_2)$. 
This power  series ${\cal J}^{\gamma}(\xi_1,\xi_2)$ is a
$\nabla$-horizontal continuation along the path $\gamma$ of the
formal power series equals to $1$.  

Evidently, we have
the composition formula:
${\cal J}^{\gamma\gamma'}(\xi_1,\xi_3)={\cal J}^{\gamma'}(\xi_2,\xi_3){\cal J}^{\gamma}(\xi_1,\xi_2)$.

If some of the points $\xi_i$ are the singular points
of the connection one can define a 
{\it regularized} parallel transport as followes.

The points $\xi=m\tau +n $ are singular point of the connection $\nabla_{fw}=d+\nu$
and   the connection   
has singularity of
the first order (fuchsian singularity) at $\xi$.  
  Fix  a local coordinate
$t$ near $\xi$. Let $K={\rm Res}_{\xi}(\nu)$ be the
residue of the connection at $\xi$; so, locally
$\nu=K_id\,\log t +\nu_{hol}$, $\nu_{hol}$ is holomorphic. 
Then  we can construct a local
multivalued horisontal section $S(t)$
of the type 
$G(t)\exp(-K\log t)$, $G$ are holomorphic
$G(0)=1$. Indeed,
the differential equation on $G$ is
$d\,G=-Kd\,\log t G +G Kd\,\log t
-\nu_{hol} G$; so if we put 
$$G=1+\sum_{w} wg_w(t), \mbox{ $w$'s are  words in $\bfa$ and $B$},$$ 
$g_w(0)=0$ we get a sequence of {\it holomorphic} nonhomogeneous  equations
for $g_w$, as the singularity of $[w,Kd\,log t]g_w$ vanishes either as $K$ commutes with $1$
or as $g_w$ has a zero at the origin $t=0$.
So, we  can choose the vanishing at zero solutions of these equations.
Call such a section {\it the normalized horizontal section}. Note
that if the connection has no pole at the point $\xi$, then 
the normalized horizontal section is a horizontal section whose
value at $\xi$  equals $1$.

Return to the parallel transports. Denote by $S_i$ the normalized horizontal section
near $\xi_i$.
 Fix the standard branches of $\log(t_i)$,
consider a horizontal  continuation $S_1^{\gamma}$ of $S_1$
along the path $\gamma$ from $\xi_1$ to $\xi_2$,
and compare this continuation with $S_2$:
the regularized parallel transport is defined
as the quotient 
$ {\cal J}^{\gamma}((\xi_1,t_1),(\xi_2,t_2))=
S_2^{-1}S_1^{\gamma}$. 
We also can realize
parallel transport as the product
$S_2^{-1}(\xi_2'){\cal J}^{\gamma'}(\xi_1',\xi_2') 
S_1(\xi_1')$ for $\xi_i'$ close to $\xi_i$ and
$\gamma'$ close to $\gamma$.

This regularized parallel transport depends
from the choice of the coordiantes. Indeed,
let $S'_i$ be a local solution corresponding
to another coordinate $t'_i$, it is easy to
show that
$S'_i(t'_i)=S_i(t_i) \exp 
\left(-A_i\log\left(
\frac{d\,t'_i}{d\,t_i}(0)\right)\right)$,
so 
$${\cal J}^{\gamma}((\xi_1,t'_1),(\xi_2,t'_2)
=\exp \left(A_2\log\left(
\frac{d\,t'_2}{d\,t_2}(0)\right)\right)
{\cal J}^{\gamma}((\xi_1,t_1),(\xi_2,t_2)
\exp \left(-A_1\log\left(
\frac{d\,t'_1}{d\,t_1}(0)\right)\right).$$


So, for any path on the elliptic curve $E_\tau$
we can consider the parallel transport 
with respect to the universal connection 
$\nabla_{fw}$. We can restrict ourself
by two basic transports $\Phi_A$ and $\Phi_B$,
where $A$ and $B$ are the strait paths from
$0$ to $\tau$ and from $0$ to $1$ respectively.
We use the coordinate $\xi$ for regularization
of the parallel transports. 
Note that for $\Phi_A$ we shall calculate
the parallel transport and multiply it from
the left by $\exp(2\pi i\bfa)$, as the 
bundle is not trivial. 

We want to deduce  the differential
equation on such 
transports.

Let $\xi_1(\tau)$ and $\xi_2(\tau)$ be
two local sections of $\Bbb E \to \Bbb H$;
assume that they do not intersect the singular
locus of the connection $\nabla_{\cal P}$.

Lemma. For any continuous in $\tau$ family of 
the paths $\gamma(t,\tau),\,\, 0\leq t \leq 1$ 
  from $\xi_1$ to
$\xi_2$ the parallel transport 
${\cal J}^{\gamma}(\xi_1(\tau),\xi_2(\tau))$
satisfies to
the following equation as function in $\tau$:
$$d\,{\cal J}^{\gamma}(\xi_1(\tau),\xi_2(\tau))
=$$
$$-\nu|_{\xi_2(\tau)} {\cal J}^{\gamma}(\xi_1(\tau),\xi_2(\tau))
+{\cal J}^{\gamma}(\xi_1(\tau),\xi_2(\tau))\nu|_{\xi_1(\tau)}
-\left(\omega_B\frac{\partial}{\partial\, B}
+\omega_{\bfa}\frac{\partial}{\partial\, \bfa}\right)
{\cal J}^{\gamma}(\xi_1(\tau),\xi_2(\tau)).$$

{\bf Proof.} For fixed $\tau=\tau_0$  consider a solution $f(\xi)$ of    
the equation $\nabla_{\cal P}|_{E_0}f(\xi)=0$ ($E_0=E_{\tau_0}$)
with the initial data $f(\xi_1(\tau_0))=1$. This is 
multivalued, pick its branch by continuation
along the path $\gamma_0$ ($\gamma_0(t)=
\gamma(t,\tau_0)$) 
then   
${\cal J}^{\gamma}(\xi_1(\tau_0),\xi_2(\tau_0))=
f(\xi_2(\tau_0))$  
The connection $\nabla_{\cal P}$ is
flat, so we can (locally in $\tau$) consider the solution $f(\xi,\tau)$
of the equation $\nabla_{\cal P} f(\xi, \tau)=0$
with the initial data $f(\xi_1(\tau_0),\tau_0)=1$.
Consider its continuation along $\gamma_0$.
For any $\tau$ $f(\xi,\tau)$ is the solution
of   the equation $\nabla_{\cal P}|_{E_\tau}f(\xi)=0$
with initial data $f(\xi_1(\tau_0))=f(\xi_1(\tau),\tau)$,
so $g(\xi)=f(\xi,\tau)f^{-1}(\xi_1(\tau),\tau)$ is the solution
of the same equation with the initial data $ g(\xi_1(\tau)=1$. As $\gamma_0$ is close to
$\gamma_\tau$, the branch of the solution
is the same as continuation along the path $\gamma_\tau$. Finally, we get
$$ {\cal J}^{\gamma}(\xi_1(\tau),\xi_2(\tau))=
f(\xi_2({\tau}),\tau)f^{-1}(\xi_1(\tau),\tau).$$
As $f$ is horisontal, on the section 
$\xi_i(\tau)$ we have
$$d \, f(\xi_i(\tau), \tau) =-\nu|_{\xi_i(\tau)}
f(\xi_i(\tau), \tau) -\left(\omega_B\frac{\partial}{\partial\, B}
+\omega_{\bfa}\frac{\partial}{\partial\, \bfa}\right)
f(\xi_i(\tau), \tau).$$
Substuitution of this equation to the expession for
the parallel transport finishes the proof.


So, for {\it loops} $\gamma$ from section $\xi(\tau)$
to itself
we get the following connection on the transports:

$$\nabla_{transport}=d+{\rm ad}_{\nu|_\xi}
+\omega_B\frac{\partial}{\partial\, B}
+\omega_{\bfa}\frac{\partial}{\partial\, \bfa}.$$

Discuss now the regularized transports.
Let $\xi(\tau)$ be a section of singularities
of $\nabla$ and let
$t$ be a fiberwise coordinate around it.
Then $\nu -Kd\,\log(t)$ is holomorphic ($K={\rm Res}_\xi\nu$ as above), denote by $\nu|_{(\xi,t)}$ the
restriction of this holomorhic form to $\xi$.
$\nu|_{(\xi,t)}$ depends in the choice of the coordinate $t$, indeed if $t'$ be another 
coordinate, then
$ d\,\log(t')=d\,\log(t)+d\,\log(
\partial\,t'/\partial\,t)+...$ and restriction of the
second term to $\xi(\tau)$ can not vanish.

Note that 
$$d\,K+[\nu|_{(\xi,t)},K] + \left(\omega_B\frac{\partial}{\partial\, B}
+\omega_{\bfa}\frac{\partial}{\partial\, \bfa}\right)K=0,$$
as it is the singular part of the curvature 
of $\nabla_{\cal P}$.
 
{\bf Lemma.} The  regularized transports satisfy
to the same differential equation as in the smooth case:
$$d\,{\cal J}^{\gamma}((\xi_1(\tau),t_1),(\xi_2(\tau),t_2))
=$$
$$-\nu|_{(\xi_2(\tau),t_2)} {\cal J}^{\gamma}((\xi_1(\tau),t_1),(\xi_2(\tau),t_2))
+{\cal J}^{\gamma}((\xi_1(\tau),t_1),(\xi_2(\tau),t_2))
\nu|_{(\xi_1(\tau),t_1)}
-
$$
$$\left(\omega_B\frac{\partial}{\partial\, B}
+\omega_{\bfa}\frac{\partial}{\partial\, \bfa}\right)
{\cal J}^{\gamma}((\xi_1(\tau),t_1),(\xi_2(\tau),t_2)).$$

{\bf Proof.} 
As we have the composition formula 
$${\cal J}^{\gamma}((\xi_1(\tau),t_1,(\xi_2(\tau),t_2))=S_2^{-1}(\xi_2'){\cal J}^{\gamma'}(\xi_1',\xi_2') 
S_1(\xi_1')$$ 
 and the differential equation for the transport between nonsingular points,
it is enough to deduce the differential equation
for the local solutions $S_i(t_i)$.
 
$S(t,\tau)=G(t,\tau)\exp(-\log t K)$, and
$G$ is horizontal with respect to fiberwise connection $\tilde{\nabla}_{fw} f=\nabla_{fw}f-f Kd\,\log t $, $G(0,\tau)=1$.
Note that this connection is the restriction 
on the fibers of the {\it flat} connection 
$\tilde{\nabla}f=\nabla_{\cal P}f  -f Kd\,\log t
-f\nu|_{(\xi,t)}$. Flatness of this connection
follows from: i) flatness of $\nabla_{\cal P}$;
ii) commutation between the left and the right
multiplication and iii) equation on 
$K$ and $\nu|_{(\xi,t)}$. So we can repeat the
consideration from the proof of the previous
lemma and get:

$$d_\tau \,G(t,\tau)
= -\nu|_{t} G(t,\tau)+
G(t,\tau)\nu|_{(\xi ,t)}
-\left(\omega_B\frac{\partial}{\partial\, B}
+\omega_{\bfa}\frac{\partial}{\partial\, \bfa}\right)
G(t,\tau).$$

Using the equation on $K$ and $\nu_{(\xi,t)}$,
we can deduce that for
$S(t,\tau)=G(t,\tau)\exp(-\log t K)$
the same equation fulfills. $\Box$



==> Andrey-2007-03-03/3.TEX <==
\section{Equivalence of categories.}
\subsection{Nilpotent connections.}



Recall the notion of a nilpotent connection. Let $({\cal E},\nabla=\nabla_{\cal E})$ be a (holomorphic)
bundle ${\cal E}$ of finite rank with flat connection $\nabla_{\cal E}$ on some (analytic) manifold $X$. We call
the pair $({\cal E},\nabla)$ by {\it connection}. We skip (rather evident) definitions of morphisms of
connections and sub- (quotient-) connections.

The definition of nilpotent connection
is inductive with respect to the rank of the bundle.

{\bf Definition}  The connection $({\cal O}_X, d)$ is the unique (up to isomorphisms) nilpotent connection
of rank $1$.
 A connection $({\cal E},\nabla)$ of rank bigger then one is {\it nilpotent} iff it has a subconnection
isomorphic to $({\cal O}_X, d)$ and the quotient is nilpotent.

{\bf Remark.} One can define nilpotent connections in the following way: first  determine the structure
of irreducible objects (= objects of rank one) and second  postulate that the subcategory of
the nilpotent connections is closed under extensions. 


The nilpotent connections form a  tensor subcategory ${\cal N}ilp(X)$ of the category ${\cal C}onn(X)$
 of the connections. This subcategory is closed with respect
to extensions, subqoutients and inner $Hom$'s.


Analogously, for an analytic family $\pi\colon {\cal X}\to B$ we can define relatively nilpotent connections.

{\bf Definition.} The category of relatively nilpotent connections ${\cal N}ilp({\cal X}\to B)$ is 
the closed under extensions subcategory of the category  ${\cal C}onn({\cal X})$
generated by pullbacks $\pi^*{\cal C}onn(B)$ of connections on $B$.

As in the absolute case, the category ${\cal N}ilp({\cal X}\to B)$ is a tensor category with inner $Hom$'s.


\subsection{Nilpotent connections on a punctured elliptic curve.}

Denote by $X_\tau$ the complement of the point $0$ in the elliptic curve $E_\tau$.

{\bf Theorem 1.}  The category ${\cal N}ilp(X_\tau)$ of the nilpotent connections on the punctured
elliptic curve $X_\tau$ is equivalent to the category ${\cal M}od-R$ of finite-dimensional modules
over the algebra $R= \Bbb C \ll \bfa ,B\gg$.

{\bf Proof.} Our strategy is the following. First, we define a functor 
${\cal F}= ({\cal P}_\tau,\nabla_{fw})\otimes_R *)$ from  ${\cal M}od-R$ to ${\cal N}ilp(X_\tau)$. 
Here we use that  $({\cal P}_\tau),\nabla_{fw})$ is both a nipotent connection on
$X_\tau$ and a left ${ R}$-module. Second we shall prove several results about this functor $\cal F$:

i) it is essentially surjective: any object in the target category is isomorphic
to some object in the image of $\cal F$;

ii) the functor $\cal F$ is fully faithful: the $Hom$'s betweeen targets are isomorphic to the
$Hom$' between sources.

After this we aplly standard result from the category theory: let ${\cal C}$ and ${\cal C}'$ be 
two categories and let ${\cal F}$ be a essentially surjective fully faithful
functor from ${\cal C}$ to ${\cal C}'$; then ${\cal C}$ and ${\cal C}'$ are equivalent.

We can rewrite the action of the functor  ${\cal F}=Hom_{ R}(({\cal P}_\tau,\nabla_{fw}),*)$ as followes.


Let $V$ be a finite-dimensional $R$-module, so it is a vector space with an action of two  operators
$\bfa$ and $B$. As this action continues to an action of formal power series in 
$\bfa$ and $B$, this operators are simultaneously nilpotent: any rather long word in
 $\bfa$ and $B$ acts by zero. Indeed, in opposite case there are infinitely many words 
acting by nonvanishing operators; so exists a formal power series which produces a divergent 
series of operators.


Associate to $V$ the vector bundle ${\cal V}_\tau$ on $E_\tau$
with the fiber $V$ and multipliers $\exp (-2\pi i \bfa ) $ and $1$. Define a connection
$\nabla_\tau$ on ${\cal V}_\tau$ by the same formula as $\nabla_{fw}$:
$\nabla_\tau=d- {\rm ad}_{\bfa} F(\xi , {\rm ad}_{\bfa} ;\tau )B d\,\xi $.
Then ${\cal F}(V)$ is equal to $({\cal V}_\tau, \nabla_\tau)$. Indeed, we indentify
$V$ with $R\otimes_R V$ by sending $v\in V$ to $1\otimes v$; as
 $x\otimes v=1\otimes xv$,   the left multiplication by some element $y$ of $R$ on
 the first factor is
 equivalent to the  action of this element on $v$: $(y\times 1)\otimes v=1\otimes (yv)$.  


{\bf Lemma.} The connection $({\cal V}_\tau,\nabla_\tau)$ is nilpotent.

{\bf Proof.} The intersection $K=H(V)={\rm Ker} \bfa\cap {\rm Ker}B$ of the kernels
of $\bfa$ and $B$ is not zero. In the opposite case $B(v)\neq 0;\forall v\in {\rm Ker}\bfa\setminus 0$;
as $\bfa$ is nilpotent, for some $n$ $\bfa^nB(v)\in {\rm Ker}\bfa\setminus 0$; by iterating
we get infinitely many nonzero operators which are words in $\bfa$ and $B$.

The algebra $R$ acts on $K$ trivially, so the corresponding connection is just the trival one $(K\otimes{\cal O},
d)$ and the quotient corresponds to the representation $V/K$, by induction we get nilpotency of the connection.

Note that $K(V)$ is nothing more that the zeroth cohomology group $H^0(R,V)$ of $R$ with coefficients in $V$.

{\bf Lemma A.} The map $H^0(R,V)= H^0(X_\tau,{\cal F}(H^0(R,V)))\to H^0(X_\tau,{\cal F}(V)) $ is an isomorphism.
The second map  above  is induced by embedding $H^0(R,V) \to  V$.

{\bf Proof.} Induction in the maximal length $l(V)$ of a word in $\bfa$ and $B$ which nonzero acts on $V$.
If $l(V)=0$ then  $R$ acts trivally, so  $H^0(R,V)=V$; on the other hand, ${\cal F}(V)$ is a trivial bundle $V\otimes
{\cal O}$
with the trivial connection $d$, so the space of  its horizontal sections $H^0(X_\tau,{\cal F}(V))$ equals
$V$. The length of the quotient module $V'=V/H(V)$ is one less then the length of $V$.  
Consider the module $V'$ and denote by $H'=H(V')$.   Denote by
$\tilde{H}$ the preimage of $H'$ in $V$ under the map $V\to V/H=V'$. $\tilde{H}$ is a $R$-module, as $\bfa$ and $B$ acts
on $H$ by zero, we have a map $H'\otimes <\bfa,B>_{\Bbb C}\to H$. The partially dual map 
$H'\to H\otimes <\bfa,B>^{\vee}_{\Bbb C}$ is injective as the simultaneous kernel of $\bfa$ and $B$ on $\tilde{H}$
is $H$. Choose some spliting $i\colon H'\to \tilde{H}$ of the sequence 
$0\to H\to \tilde{H}\to H'\to 0$ of vector spaces.

By induction assumptions, the  horizontal sections of ${\cal F}(V')$
are constant sections of ${\cal F}(H')$, so we can identify them with vectors in $H'$.
Let $s$ be some horizontal section of ${\cal F}(V)$, denote by $v'\in H'$ the corresponding
horizontal section of ${\cal F}(V')$, put $v\in \tilde{H}\in V$ the vector $i(v')$. $s(v)=v+E_1(\xi)\bfa (v)$ is a
section of the bundle  ${\cal F}(V)$ (it has required quasiperiodicity), the difference $s-s(v)$ is a 
section of ${\cal F}(H)$, so it is $H$-valued elliptic function $f=f(\xi)$. We have $s=s(v)+f$.
As it is horizontal, $\nabla(s(v)+f)=-B(v)d\,\xi +d\,E_1(\xi)\bfa (v)+d\,f$ is equal to zero.
But space spanned by constants and $d\,E_1$ dos not contain differential of elliptic functions,  so
$B(v)$ and $a(v)$ are zero, hence $v=0$ and section $s$ belongs to the trivial subbundle
${\cal F}(H)$. The horizontal section of it are equal to vectors in $H$. This ends the proof of
the lemma.

{\bf Remark.} The consideration above can be reinterpret in more homological way. Namly, one can prove
by induction that $H^0(X_\tau,{\cal F}(V))=H(V)$ and $H^1(X_\tau,{\cal F}(V))=V/(RV)\otimes <\bfa,B>^{\vee}_{\Bbb C}$.
The main consideration  of the inductive step is that 
for long exact sequence induced by
$$0\to {\cal F}(H)\to {\cal F}(V)\to {\cal F}(V')\to 0$$
the connecting homomorphism 
$H^0(X_\tau,{\cal F}(V'))\to H^1(X_\tau,{\cal F}(H))$ is injective.

We shall use this lemma for the proof of the second  property of the functor $\cal F$ -- that it is
fully faithful. An additional argument in this proof is the comparison of inner $Hom$'s. In general, for
modulas over noncomutaive rings the inner $Hom$ does not exist. We define the structure of $R$-module
on the vector space $Hom_{\Bbb C}(V_1,V_2)$ for modules $(V_1,\rho_1)$ and $(V_2,rho_2)$ by the following rule 
$\rho_{Hom}(x)(L)=\rho_2(x)\circ  L-L\circ\rho_1(x)$ for generators $\bfa$ and $B$ and continue $\rho_{Hom}$
to $R$ by multiplicativity. In other words, this is inner $Hom$ in the category of 
representation of free {\bf Lie algebra} generated by $\bfa$ and $B$. Note that $H^0(R, {cal H}om (V_1,V_2))=
Hom_R(V_1,V_2)$, Indeed a $\Bbb C$-linear map $L$ from $V_1$ to $V_2$ is $R$-linear iff
$\rho_2(x)\circ  L=L\circ\rho_1(x)$, $x=\bfa,B$.

{\bf Lemma B.} The functor $\cal F$ is compatible with inner $Hom$'s:
${\cal F}({\cal H}om(V_1,V_2))={\cal H}om({\cal F}(V_1),{\cal F}(V_2))$; in the lhs ${\cal H}om$ denotes
the inner $Hom$ in the category of $R$-modules, in the r.h.s -- in the category of nilpotent connections
on $X_\tau$.

{\bf Proof.} This fact becames evident if we take in account that formulas defining this functor contains
only $\bfa$, $B$ and their commutators, so they lie in the free Lie algebra generated by $\bfa$ and $B$.


As maps of nilpotent connections coincide with the sections of inner $Hom$, by application of Lemma A we
get the following result.

{\bf Proposition.} The functor $\cal F$ is fully faithfull. 






\section{The equivalence for families.}

In this section we present a description of the relatively nilpotent connections on the universal 
punctured elliptic curve $\pi \colon {\Bbb X}\to {\Bbb H}$ in the same spirit as in the case
of an induvidual curve.

\subsection{Sheaves of free algebras} 

Consider    a trivial (pro)boundle  ${\cal R}$ on $\Bbb H$ with fiber $R$ and equpped with the action of $SL_2(\Bbb Z)$
  by formulas: $\bfa \to \bfa'=\frac{\bfa }{c\tau +d}$, 
$B\to B'=(c\tau +d)B +2\pi i c \bfa$. Equip  this bundle by $SL_2(\Bbb Z)$-invariant connection 

$$\nabla_{\frak R}=d\,    
+\omega_B 
\frac{\partial\,}{\partial\, B}+\omega_{\bfa}
\frac{\partial\,}{\partial\, \bfa },$$

$$\omega_B =-\frac12\frac{1}{2\pi i}
\frac{\alpha_1\alpha_2}{\alpha_1+\alpha_2}
\left(\left(\wp(\alpha_1)-\frac1{\alpha_1^2}\right)
-\left(\wp(\alpha_2)-\frac1{\alpha_2^2}\right)
\right)(B,B)d\,\tau,\quad 
\omega_{\bfa} =-\frac1{2\pi i} Bd\,\tau,
$$

We denote  this (pro)connection $({\cal R},\nabla_{\frak R})$ by ${\frak R}$

{\bf Remark.} Note that the term  $\omega_{\bfa}
\frac{\partial\,}{\partial\, \bfa }$ corresponds to the connection on the
tensor algebra of the first homology group eqipped by Gau\ss-Manin connection.

One can also consider the (sub)bundle $\cal L$ of free Lie algebras generated by $\bfa$ and $B$;
$SL_2(\Bbb Z)$ acts on it.  
Moreover, $\cal L$ is invariant under the connection $\nabla_{\frak R}$

For any ${\cal R}$-valued  one-form  $\mu$ on an open subset $U$ of $\Bbb H$ one can twist the connection
$\nabla_{\frak R}$ by $\mu$: $\nabla^\mu_{\frak R}=\nabla_{\frak R}-{\rm ad}_\mu$, im $\mu$ takes values
in subbundle of Lie algebras $\frak L$, $\nabla^\mu_{\frak R}$ preserves this subbundle. The connection
$({\cal R},\nabla^\mu_{\frak R})$ over $U$ we denote by ${\frak R}^\mu$. If $U=\Bbb H$ and the form
 $\mu$ is $SL_2(\Bbb Z)$-invariant,
then  ${\frak R}^\mu$ is $SL_2(\Bbb Z)$-invariant; if $\mu$ is invariant under some subgroup $\Gamma$
of $SL_2(\Bbb Z)$,  ${\frak R}^\mu$ is $\Gamma$-invariant.

\subsection{${\frak R}$-modules and relatively nilpotent connections.}

In this susection we generalize the functor $\cal F$ for the relative case. 

Let ${\Bbb V}$ be a  connection over an open subset $U$ of $\Bbb H$ which is a (right) module over (restriction of)
$\frak R$. Put  $${\cal F}(\Bbb V)= ({\cal P}, \nabla_{\cal P})\otimes_{\pi^*{\frak R}}\pi^*\Bbb V;$$
where we use an evident structure of the left  $\pi^*{\frak R}$-module on $\cal P$. ${\cal F}(\Bbb V)$ is
a connection on $\pi^{-1}(U)$. If $U=\Bbb H$ and the connection $\Bbb V$ is $\Gamma$-invariant,
then  ${\cal F}(\Bbb V)$ is $\Gamma$-invariant, $\Gamma$ be a subgroup of the $SL_2(\Bbb Z)$.

More explicitly, $\Bbb V$ goes under functor $\cal F$ to the connection $({\cal V}, \nabla_{\cal V})$ where
$\cal V$ be a bundle on $\Bbb E$  which is just a pull-back of $\Bbb V$ on $\Bbb H\times \Bbb C$ glued
by multipliers $\exp(-2\pi i \bfa)$ and $1$ under the shifts by $\tau$ and $1$ respectively. 
The connection $\nabla_{\cal V}$ is defined as followes: 

$$\nabla_{\cal V}=\nabla_{\Bbb V}+\nu;\quad
\nu=-\left(\alpha F(\xi , \alpha ;\tau ) d\,\xi
+\frac{1}{2\pi i}\left(\alpha F'_2(\xi , \alpha ;\tau )+
\frac{1}{\alpha}\right)d\,\tau\right)B;$$
where $\nabla_{\Bbb V}$ denotes the connection on the pull-back $\pi^*\Bbb V$.


Evidently, we can generalize this functor to the case of ${\frak R}^\mu$-modules with replacing
$({\cal P}, \nabla_{\cal P})$ by $({\cal P}, \nabla_{\cal P}^\mu)$.

{\bf Lemma.} Let $\xi(\tau):U\to \pi^{-1}U$ be a section of $\pi:\pi^{-1}U\to U$. Put $\mu =\nu|_{\xi}$.
Then the restriction ${\frak R}^\mu(\Bbb V)|_\xi$ of the connection ${\frak R}^\mu(\Bbb V)$ to $\xi$
coincides with $\Bbb V$.

{\bf Proof.} The connection $\nabla_{\cal V}^\mu$ associated to ${\frak R}^\mu(\Bbb V)$ expresses as 
$\nabla_{\Bbb V}+\nu -\mu,$, so its restriction is $\nabla_{\Bbb V}+\nu|_{\xi} -\mu=\nabla_{\Bbb V}$.

Now we shall prove that locally in base this functor presents an equivalence of categories.
The proof of fully faithfulness is analogous to the proof in the case of induvidual curve, and
we leave it as exercise for the reader. The Essentual surjectivity followes from the following consideration.  

Let $({\cal V}, \nabla)$ be a relative nilpotent connection on $P\colon U\to \Bbb H$ with finite order pole at zero
section. we shall prove that it has the required form.

Its restriction to any 
fiber of $p$ is a nilpotent connection, so according to Theorem  A we can associate to this restriction
a vector space $V$ with action of two operators $\bfa$ and $B$. As this restriction forms a family
of connection, we have a family of operators $\bfa(\tau)$, $B(\tau)$ acting on $V$.
So, the connection $\nabla$ can be written as $d-\nu(\bfa,B) -\Phi(\xi, \tau)d\,\tau$ by formal subtraction and addition of 
the expression $\nu$.

As $\nabla$ is flat, $\Phi$ must be holomorphic, this statement can be obtained by calculation of the singular part
of curvature near zero section.

From the quasiperiodicity  with respect to $\xi\to \xi+\tau$, $\xi\to \xi+1$ we get
$$\Phi(\xi+\tau, \tau)-\exp(-2\pi i\alpha)\Phi(\xi, \tau)=-\frac{\exp(-2\pi i\alpha)-1}{-\alpha}\left(\frac d{d\,\tau}\bfa 
+\frac B{2\pi i}\right),$$
$$
\Phi(\xi+1, \tau)=\Phi(\xi, \tau).$$

{\bf Lemma.} $\Phi(\xi, \tau)$ does not depends in $\xi$.

{\bf Proof.} Denote by $K$  the expression $\left(\frac d{d\,\tau}\bfa 
+\frac B{2\pi i}\right)$. The function $-(F(\xi, \alpha)-\frac 1\alpha)K$ satisfies the required quasiperiodicity, so
$\Phi(\xi,\tau)+(F(\xi, \alpha)-\frac 1\alpha)K$ satisfies the homogenious equations, so equals to $\alpha F(\xi, \alpha)C$
for some $C(\tau)$. As $\Phi(\xi, \tau)=\alpha F(\xi, \alpha)C(\tau)-(F(\xi, \alpha)-\frac 1\alpha)K$ is holomorphic, 
the singilar part
$(\alpha C(\tau)-K)frac 1\xi$ at $\xi=0$ vanishes, so $K=\alpha C(\tau)$ and $\Phi(\xi, \tau)=C(\tau)$

So we get 
$$\frac{\exp(-2\pi i\alpha)-1}{-\alpha}\left(-\alpha \Phi(\tau)\right)=\frac{\exp(-2\pi i\alpha)-1}{-\alpha}\left(\frac d{d\,\tau}\bfa 
+\frac B{2\pi i}\right).$$
as $\bfa$ is nilpotent, the operator $\frac{\exp(-2\pi i\alpha)-1}{-\alpha}$ is invertible, so we get
 $ \frac d{d\,\tau}\bfa 
 -[\Phi, \bfa]=-\frac B{2\pi i}$.
 
 Now we calculate the curvature of $\nabla$. The calculation is parallel to the calculation of the curvature
 of the connection on $\cal P$.
 We get $d\,(\Phi(\tau)d\,\tau) =0$ and
 $$d\, \nu = -\left(\frac{\partial \bfa}{\partial \tau}\frac{\partial }{\partial \bfa} 
 +\frac{\partial B}{\partial \tau}\frac{\partial }{\partial B}\right)\nu \wedge d\,\tau=$$
 $$
  \left(\left(-\frac{B}{2\pi i} +[\Phi, \bfa]\right) 
\frac{\partial}{\partial\,  \bfa }+\frac{\partial B}{\partial \tau}\frac{\partial }{\partial B}\right)
\alpha F(\xi , \alpha ;\tau ) B
  d\,\xi
\wedge d\,\tau= 
  $$
 
 $$ \frac{
(\alpha_1+\alpha_2) F(\xi , \alpha_1+\alpha_2 ;\tau )
- \alpha_2 F(\xi ,  \alpha_2 ;\tau )}{\alpha_1} 
\left(\left(-\frac{B}{2\pi i} +[\Phi, \bfa]\right),B\right)d\,\xi
\wedge d\,\tau
$$
$$+ \alpha F(\xi , \alpha ;\tau )\frac{\partial B}{\partial \tau}d\,\xi
\wedge d\,\tau$$

The term $\nu\wedge\nu$ equals, up to factor $\frac12\frac{d\,\xi\wedge d\,\tau}{2\pi i}$,
$$\left({\alpha_1\alpha_2}   F(\xi , 
\alpha_1+\alpha_2 ;\tau )  \left(\wp(\alpha_1) 
-\wp(\alpha_2) \right) +\frac{\alpha_1F(\xi , 
\alpha_1  ;\tau )}{\alpha_2}-\frac{\alpha_2F(\xi , 
\alpha_2  ;\tau )}{\alpha_1}
\right)(B,B) .$$

The term $\nu\wedge (\Phi(\tau)d\,\tau)+ (\Phi(\tau)d\,\tau)\wedge \nu$ is equal to
$$[\alpha F(\xi , \alpha ;\tau )B,\Phi(\tau)]d\,\xi
\wedge d\,\tau=\alpha _1F(\xi , \alpha _1;\tau )(B,\Phi(\tau))d\,\xi
\wedge d\,\tau.
$$

Finally, the curvature  equals, up to factor $\frac12\frac{d\,\xi\wedge d\,\tau}{2\pi i}$,
$$  \alpha F(\xi , \alpha ;\tau )\left(
\frac{\alpha_1\alpha_2}{\alpha_1+\alpha_2}
\left(\left(\wp(\alpha_1)-\frac1{\alpha_1^2}\right)
-\left(\wp(\alpha_2)-\frac1{\alpha_2^2}\right)
\right)(B,B) +4\pi i \left(\frac{\partial B}{\partial \tau}-[\Phi(\tau),B]
\right)\right).$$

As the operator $\alpha F(\xi , \alpha ;\tau )$ is invertable, the flatness of connection is equivalent to the
condition  
$$\frac{\partial B}{\partial \tau}-[\Phi(\tau),B]=-\frac12\frac{d\,\xi\wedge d\,\tau}{2\pi i}
\frac{\alpha_1\alpha_2}{\alpha_1+\alpha_2}
\left(\left(\wp(\alpha_1)-\frac1{\alpha_1^2}\right)
-\left(\wp(\alpha_2)-\frac1{\alpha_2^2}\right)\right).$$


==> Andrey-2007-03-03/4.TEX <==
\subsection{ The universal connection on the elliptic curves with several punctures.}

 
Let $\eta_0=0,\eta_1, \cdots,\eta_n$ are mutually different  points on the elliptic curve $X_\tau$, we will often
identify the with their preimages in $\Bbb C$.

Associate to each $\eta_i$ a new formal variable $K_i$. Put $R^{(n)}=\Bbb C\ll \bfa ,B, K_i\gg $.
As above, define a (pro) vector bundle ${\cal P}^{(n)}_\tau$ on $E_\tau$
with fiber $R^{(n)}$ by multipliers  
$\exp (-2\pi i \bfa ) $ and $1$.

{\bf Proposition 1.} The differential operator  
$$\nabla_{fw}=d- \alpha F(\xi , \alpha ;\tau )B d\,\xi -\sum_{i+1}^n (F(\xi -\eta_i,\alpha ;\tau )-F(\xi,\alpha ;\tau ) )
K_i d\,\xi $$
is a connection on ${\cal R}^{(n)}_\tau$ with log singularities at $0$ and $\eta_i$'s.

The proof is parallel to the case $n=0$.

As in the case $n=0$ we can try to lift this connection on the family, in which $\tau$ and $\eta_i$'s play the
role of coordinates on the base of the family.

The   shift $\eta_i \to \eta_i +\tau$ acts on $R^{(n)}$ by $K_i\to \exp(-2\pi i\alpha)K_i$, 
$B \to B +\frac{\exp(-2\pi i \alpha)-1}{\alpha}K_i$
 

 
\subsection{ The universal connection on the square of an elliptic curve.}

We discribe an universal flat connection on the square of the elliptic curve $X=X_\tau$ with logarithmic
singularities at $0\times X$ $X\times 0$ and diagonal $\Delta_X$. 

Put $U^{(2)}=U^{(2)}_\tau=X\times X\setminus
\{0\times X\cup X\times 0\cup \Delta_X\}$. Then $U^{(2)}_\tau$ can be treated as a fiber of the forgetful
map of modular spaces ${\cal M}_{1,3}\to {\cal M}_{1,1}$. The action of the symmetric group ${\frak S}_3$
can be described as permutation of $(\xi_0=0,\xi_1,\xi_2)$ and shifting the first point to zero:
$\sigma:( \xi_0,\xi_1,\xi_2)\to ( \xi_{\sigma(0)},\xi_{\sigma(1)},\xi_{\sigma(2)})
\to ( 0,\xi_{\sigma(1)}-\xi_{\sigma(0)},\xi_{\sigma(2)}-\xi_{\sigma(0)})$.

Consider a noncomutative associative ring $R^{(2)}$ generated by $\bfa^{(i)},B^{(i)}$, $i=1,2$ with relations
$$[\bfa^{(1)},\bfa^{(2)}]=0,\quad [\bfa^{(1)},B^{(2)}]=[\bfa^{(2)},B^{(1)}],\quad [B^{(1)},B^{(2)}]=0;$$
$$[\bfa^{(1)},[\bfa^{(2)},B^{(1)}+B^{(2)}]]=0,\quad [B^{(1)},[B^{(2)},\bfa^{(1)}+\bfa^{(2)}]]=0.$$
Define an action of the symmetric group ${\frak S}_3$ on it as permutation of 
$(\bfa^{(0)}= -\bfa^{(1)}-\bfa^{(2)},\bfa^{(1)},\bfa^{(2)})$ and $(B^{(0)}=-B^{(1)}-B^{(2)},B^{(1)},B^{(2)})$.
It is easy to check that this action preserves the relations. Denote by $\alpha^{(i)}$ the adjoint action
of $\bfa^{(i)}$

Consider a bundle ${\cal P}^{(2)}_\tau$ on $X\times X$ with fiber $R^{(2)}$ defined by multipliers 
$\exp(-2 \pi i\bfa^{(j)})$ with respect to shift $\xi_j\to \xi_j+\tau$ and multipliers $1$  
shift of $\xi$'s by one. It is easy to check that this bundle is ${\frak S}_3$ invariant.

Define a $R^{(2)}$-valued differential form $\nu^{(2)}$ on $\Bbb C^2$ with logarithmic singularities by formula
$$\nu^{(2)}(\xi_1,\xi_2,)=
(\alpha^{(1)}+\alpha^{(2)})F(\xi_1,\alpha^{(1)}+\alpha^{(2)})
(\alpha^{(2)})F(\xi_2-\xi_1, \alpha^{(2)})B^{(1)}d\,\xi_1+$$
$$
(\alpha^{(1)}+\alpha^{(2)})F(\xi_2,\alpha^{(1)}+\alpha^{(2)})
(\alpha^{(1)})F(\xi_1-\xi_2, \alpha^{(1)})B^{(2)}d\,\xi_2$$
 
 
 {\bf Lemma.} The form $\nu^{(2)}$ satisfies to the several properties: 
 
 i) this  form is pull back of a form on the square of the elliptic curve with values in bundle 
 ${\cal P}^{(2)}_\tau$;
 
 ii) this form is ${\frak S}_3$-invariant;
 
 iii) this form is closed: $d\,\nu^{(2)}=0$;
 
 iv) the wedge-square of this form vanishes: $\nu^{(2)}\wedge \nu^{(2)}=0$.
 
 {\bf Proof.} The statement i) followes immediatly from the quasiperiodicity of $F$.
 
 ii) This followes from the following identity (the Fay identity):
 $$ 
 F(\xi_1,\alpha^{(1)} )
 F(\xi_2 , \alpha^{(2)}) =
 F(\xi_1,\alpha^{(1)}+\alpha^{(2)})
 F(\xi_2-\xi_1, \alpha^{(2)}) +
 F(\xi_2,\alpha^{(1)}+\alpha^{(2)})
 F(\xi_1-\xi_2, \alpha^{(1)}).  $$
 
 
 iii) and iv) can be proved by the following consideration. As in the case of the bundle
 ${\cal P}$ over the curve $X$, it is easy to check that the only regular section of ${\cal P}^{(2)}_\tau$
 is zero section. So, it is sufficient to check that  $d\,\nu^{(2)} $ and
 $\nu^{(2)}\wedge \nu^{(2)} $ has no poles. From the ${\frak S}_2$-invariancy it is enough to consider 
 the locus $\xi_1=0$. The singular part of $d\,\nu^{(2)} $ near this locus is equal to
 $$-\frac{\partial F(\xi_2-\xi_1, \alpha^{(2)})}{\partial \xi_2}(\alpha^{(1)}+\alpha^{(2)})\alpha^{(2)}B^{(1)}
 \frac{d\,\xi_1}{\xi_1}\wedge d\,\xi_2=0,$$
 as $(\alpha^{(1)}+\alpha^{(2)})\alpha^{(2)}B^{(1)}$ according to relations in $R^{(2)}$ and 
 $\frac{\partial F(\xi_2-\xi_1, \alpha^{(2)})}{\partial \xi_2}$ is a  Taylor power series in $\alpha^{(2)}$.
 
 The singular part of $\nu^{(2)}\wedge \nu^{(2)} $ near $\xi_1=0$ equals
 
 $$[(\alpha^{(1)}+\alpha^{(2)}) B^{(1)} ,
B^{(2)}+
(\alpha^{(1)}+\alpha^{(2)})F(\xi_2,\alpha^{(1)}+\alpha^{(2)})-1+$$
$$
\alpha^{(1)}F( -\xi_2, \alpha^{(1)})-1)B^{(2)}
]
\frac{d\,\xi_1}{\xi_1}\wedge d\,\xi_2,$$
here we use the relations $(\alpha^{(1)}+\alpha^{(2)})(\alpha^{(2)})^kB^{(1)}=0$, $k>0$,
$(\alpha^{(1)}+\alpha^{(2)})^l(\alpha^{(1)})^kB^{(2)}=0$, $k,l>0$ which hold in $R^{(2)}$. The term
$[(\alpha^{(1)}+\alpha^{(2)}) 
 B^{(1)},
B^{(2)}]$ vanishes, so this singular part equals
$$ [(\alpha^{(1)}+\alpha^{(2)}) B^{(1)} ,
(\alpha^{(1)}+\alpha^{(2)})F(\xi_2,\alpha^{(1)}+\alpha^{(2)})+ 
(-\alpha^{(1)})F( \xi_2, -\alpha^{(1)})-2)B^{(2)}
]
\frac{d\,\xi_1}{\xi_1}\wedge d\,\xi_2.$$
 Hence, it is enough to prove that for $k>0$, $[(\alpha^{(1)}+\alpha^{(2)}) B^{(1)} ,((\alpha^{(1)}+\alpha^{(2)})^k+(-\alpha^{(1)})^k)
 B^{(2)}]=0$, 
 in $R^{(2)}$. An elementary calculation showes that $(x+y)^k+(-x)^k =\phi_k(x,y)x(x+y) +y^k$ for some polinomials
 $\phi_k(x,y)$. We have 
 $$ ((\alpha^{(1)}+\alpha^{(2)})^k+(-\alpha^{(1)})^k)
 B^{(2)}=(\phi_k(\alpha^{(1)},\alpha^{(2)})\alpha^{(1)}(\alpha^{(1)}+\alpha^{(2)})+(\alpha^{(2)})^k)B^{(2)}=
 (\alpha^{(2)})^kB^{(2)},$$
 as $\alpha^{(1)}(\alpha^{(1)}+\alpha^{(2)}) B^{(2)}=0.$ By induction in $k$ we prove that 
 $[(\alpha^{(1)}+\alpha^{(2)}) B^{(1)},(\alpha^{(2)})^kB^{(2)}]=0$. For $k=0$ this is just the relation in 
 $R^{(2)}$. The step of the induction:
 $$[(\alpha^{(1)}+\alpha^{(2)}) B^{(1)},(\alpha^{(2)})^{k+1}B^{(2)}]=
 \alpha^{(2)}[(\alpha^{(1)}+\alpha^{(2)}) B^{(1)},(\alpha^{(2)})^kB^{(2)}]-$$
 $$
 [\alpha^{(2)}(\alpha^{(1)}+\alpha^{(2)}) B^{(1)},(\alpha^{(2)})^kB^{(2)}]=0,$$
 as $\alpha^{(2)}(\alpha^{(1)}+\alpha^{(2)}) B^{(1)}=0$. $\Box$
 
 The previous lemma implies that the differential operator $d\, - \nu^{(2)}$ defines a ${\frak S}_3$-invariant
 flat connection $\nabla^{(2)}_\tau$ on 
 the restriction of 
 ${\cal P}^{(2)}_\tau$ to $U^{(2)}$ with logarithic singularities.
 
 {\bf Remark.} By using the pair $({\cal P}^{(2)}_\tau,\nabla^{(2)}_\tau$  one can describe the category of
 nilpotent connections on $U^{(2)}$ in the same manner as in section ... the category of
 nilpotent connections on $U$ was described by ${\cal P},\nabla_\tau$.
 
 
 \subsection{Elliptic hexagon equation.}
  
In the subsection we derive an equation on the parellel transports on the elliptic curve $X_\tau$. Our strategy is
like in the original Drinfelds paper .... We consider a {\it contractible} loop $\gamma^{(2)}$ on $U^{(2)}$,
the parallel transport along it with respect to $\nabla^{(2)}_\tau$ is $1$ as the loop is contractible and
the connection is flat. On the other hand, we express this transport as product of six parallel transports 
along the paths on the singular locus of the connection  $\nabla^{(2)}_\tau$. This get us an equation.


We start by some generalities about the description of horizontal sections near singularities of connection which
generalize our  consideration for defenition of the regularized parallel transport.

Recall (see the discussion about differential equations for parallel transport)
that if $D$ be a smooth divisors defined by equation $t=0$ and if $\nabla=d+\nu$ by a flat connection with
logarithmic singularity  at $D$ then we can define a "restriction" $\nu|_{(D,t)}$ of the form $\nu$ to divisor
as $(\nu-K(\nu) d\,\log t)|_D$, $K={\rm Res}_D$. Denote by $\nabla|_{(D,t)}=d+\nu|_{(D,t)}$ the "restriction" of the connection
to the divisor. Morover, the residue $K(\nu)$ is horizontal with respect to the adjoint action of this connection.
On the other hand, the local equation $t=0$ defines a contraction $p_t$ of some 
neighborhood of $D$ to $D$

{\bf Lemma.} Let the residue $K$ be nilpotent. Let $J$ be a horizontal section of  $\nabla|_{(D,t)}=d+\nu|_{(D,t)}$ on the 
divisor $D$. Then one can "continue" this section to a horizontal section section $S_J$ of $\nabla$ in some 
neighborhood of $D$ of the form $S_J=G\exp(-K\log t)p_t^*J$, $G$ is holomorphic and $G|_D=1$
 
A proof is parallel to the  case $D$ is a point.

Let the singular locus of a logarithmic flat connection $\nabla=d +\nu$ is a normal crossing divisor and let 
locally the equations of two components $D_1$ and $D_2$ of this singular locus are $t_1=0$ and $t_2=0$. 
Then the restrictions of  the residues $K_i={\rm Res}_{D_i}(\nu)|_{D_1\cap D_2}$ commute, as this commutator 
is coefficient of the singular part of the curvature. Let $K_i$ are simultaneuosly nilpotent.

{\bf Lemma.} Let $K_i$ are simultaneuosly nilpotent. Then there exists a $\nabla$-horizontal section $S^{(2)}$ of the
the shape $S^{(2)}=G\exp(-K_1\log t_1 -K_2\log t_2)$, $G$ is holomorphic and $G|_{D_1\cap D_2}=1$.

We leave a proof as an exercise for the reader.

We use such horizontal sections for comparison  of the parallel transports on $U^{(2)}$ with parallel transports
on the components of the singular locus of the connection $\nabla^{(2)}$. Note that this locus is not a divisor 
with normal crossing on $X\times X$, so for application of the lemmas we shall blow up the point $(\xi_1=0, \xi_2=0)$,
denote the result of this blow up by $X^{(2)}$. So, the singular locus of   $\nabla^{(2)}$ on 
$X^{(2)}$ is union of the exceptional divisor $X_{012}$ 
and three elliptic curves $X_{ij}$, $i< j=0,1,2$; the exceptional divisor is a rational curve, the elliptic curves
$X_{ij}$ are proper preimages of the curves $\xi_i=\xi_j$ ($\xi_0=0$). We introduce a coordinate $x=\xi_1/\xi_2$ 
on the rational curve $X_{012}$, in this coordinate the intersections with $X_{01}$, $X_{12}$ and $X_{02}$
are the points $0$, $1$ and $\infty$ correspondently. On $X_{ij}$ the intersection with $X_{012}$ is
the point $\ne$.

Denote by $\Delta^2$  a triangle $0\le t_1\le t_2 \le 1$; consider the blow up   of 
the affine plane $\Bbb R^2$ at the vertices
$(0,0)$, $(0,1)$ $(1,1)$ of the triagle
$\Delta^2$. Take the (topological) closure $\Delta^{(2)}$  in this blow up of the open triangle
$0< t_1< t_2 < 1$.  This closure $\Delta^{(2)}$ is a hexagon, three sides of this hexagon are the sides 
$\Sigma_{01}= \{t_1=0\}$, $\Sigma_{12}=\{t_1=t_2\}$ and $\Sigma_{02}=\{t_2=1\}$ of triangle $\Delta^2$, extra three 
sides $\Sigma_{012}^{\lambda\mu}$, $\lambda<\mu=0,1,\infty$  lie on the exceptional divisors 
(preimages of the vertices of the triangle, $\Sigma_{012}^{01}$ over $(0,0)$,
$\Sigma_{012}^{0\infty}$ over $(0,1)$ and $\Sigma_{012}^{1\infty}$ over $(1,1)$). The labeling of the sides
will be motivated bellow. 

Consider the following piecewise-smooth  contractible loop $\sigma$  in the interior of the hexagon $\Delta^{(2)}$;
this loop   is the union of six smooth paths $\sigma_*^*$
which connect points   near the vertices of the hexagon, any path $\sigma_*^*$ is close to the corresponding side
$\Sigma_*^*$ of the hexagon.

 Associate to a smooth loop $\gamma:[0,1]\to X, \gamma(0)=\gamma(1)=\ne$ without self-intersections
 its ``iteration'' $\gamma^2:
\Delta^2\to X\times X, (t_1,t_2)\to (\gamma(t_1),\gamma(t_2))$. The  map $\gamma^2$   determines a map of the 
open triangle  into $U^{(2)}$, so this map induces a map $\gamma^{(2)}$ of the closure $\Delta^{(2)}$ of the triangle
to the  $X^{(2)}$. The boundary of the hexagon $\Delta^{(2)}$ maps to the singular locus of the connection
$\nabla^{(2)}$; $\Sigma_{ij}$ maps to the path $\gamma$ on $X_{ij}$,  $\Sigma_{012}^{\lambda\mu}$ maps to the segment
in $X_{012}$ connecting the points $\lambda$ and $\mu$. This motivate notation for the sides of the hexagon.

As  the loop $\sigma$ in the hexagon $\Delta^{(2)}$ is contractible, the loop $\gamma^{(2)}\circ \sigma$ 
in $U^{(2)}$ is  
contractible; therefore the parallel transport
along it equals to $1$. On the other hand, the loop $\sigma$ is closed to the boundary of the hexagon $\Delta^{(2)}$
and this boundary maps to the singular locus of connection; so, we can apply assimptotic formulas for the
horizontal sections near singularities. 

We shall equipp a component of the singular locus with equation of this component. Globally this is impossible,
as the normal bundle is nontrivial. For elliptic curves $X_{ij}$ we choose such an equation on the universal 
covering of $X^{(2)}$. For the rational curve $X_{012}$ we have three paths along which we calculate parallel 
transport. Each path connect two of marked points $0,1,\infty$.


For sach a path we use a local equation of the component, this equation is valid outside the third marked point.
 


 


==> Andrey-2007-03-03/alg.tex <==
\section{Algebraic structure.} In this section we describe the algebraic $\Bbb Q$
structure on $\cal P$ and $R$ for an elliptic curve defined over
$\Bbb Q$.

We start from reminding of some standard  facts about algebraic
elliptic curves. Let $(X,O)$ be an elliptic curve defined over
some field $k$ of characteristic zero.
 Then  it can be represented as a plane cubic $y^2=4x^3-g_2 x -g_3$,
 $g_2, g_3\in k$  and the
 marked point $O$ lies at infinity. This form is unique up to
 dilatations $g_2\to\lambda^4g_2,\quad g_3\to\lambda^6g_3,\quad
 x\to\lambda^2x,\quad y\to\lambda^3y$, $\lambda\in k$.

  If $k$ is a subfield of $\Bbb C$, e.g.
$k=\Bbb Q$, one can represent the analytic curve $X(\Bbb C)$ as the
quotient of $\Bbb C$ by some lattice $L$. The
map  from $X(\Bbb C)$ to $\Bbb C/L$ is defined by integration
of the form
$\omega =d\,x/y$ from the marked point to the variable one
$p\to\int_O^p\omega$. The ambiguity in choosing of the path of integration
belongs to the topological first homology group $H_1(X(\Bbb C),\Bbb Z)$
which corresponds to the lattice $L$.
 Choose some basis $(u, v)$ in
such a way that $\Im (v/u)>0$, put $\tau=v/u$. Then
$g_2=60u^{-4}e_4(\tau),\quad g_3=140u^{-4}e_6(\tau)$, moreover
the map
$\xi\to (x(\xi)=u^{-2}(E_2(\xi,\tau)-e_2(\tau)),\quad y(\xi)=-2u^{-3}E_3(\xi,\tau))$
produces an analytic isomorphism between $X_{\tau}=\Bbb C/(\Bbb Z\tau +\Bbb Z)$
and  $X(\Bbb C)$ and $\omega=d\,x/y=ud\,\xi$. So, $u$ can be calulated as the
period (elliptic integral) of the algebraic form $\omega$ against a
topological
chain. If we choose another equation of $X$, twisted say, by $\lambda$,
then $\omega$ becomes $\lambda^{-1}\omega$ and $(u,v)\to (\lambda^{-1}u,
\lambda^{-1}v)$.


Some analytic preparations. Note that over the complement
$U_\tau$ to the marked point in $X_\tau$ the bundle $\cal P$
defined by multiplier $\exp(-2\pi i\t)$ is trivial and can be
trivialized by the left multiplication by
$g(\xi)=\exp(-E_1(\xi,\tau)\t)$, indeed,  sections of $\cal P$
are the quasiperiodic functions $f$ on $\Bbb C$:
$f(\xi+1)=f(\xi);\quad f(\xi+\tau)=\exp(-2\pi i\t)f(\xi)$; hence
$g(\xi)f$ are periodic, as $E_1(\xi+1,\tau)=E_1(\xi,\tau), \quad
E_1(\xi+\tau,\tau)= E_1(\xi,\tau)-2\pi i$.

The connection $\nabla=d-\ad_\t F(\xi,\ad_\t)Ad\,\xi$
transforms under the gauge transformation $s\to g(\xi)s$ to the operator
$$g(\xi)\nabla g^{-1}(\xi)=d-d\,g(\xi)g^{-1}(\xi)-
g(\xi)\ad_\t F(\xi,\ad_\t)Ag^{-1}d\,\xi$$
$$=d-E_2(\xi,\tau)\t d\,\xi -\exp(-E_1(\xi,\tau)\ad_\t )
 \exp\left(-\sum _{k=1}^{\infty}\frac{(-\ad_\t  )^k}k
(E_k(\xi,\tau  )-e_k(\tau))\right)Ad\,\xi$$
$$=
d-\left((E_2(\xi,\tau)-e_2(\tau))\t    +
 \exp\left(-\sum _{k=2}^{\infty}\frac{(-\ad_\t  )^k}k
(E_k(\xi,\tau  )-e_k(\tau))\right)(A+e_2(\tau)\t\right)d\,\xi.
$$

Consider new generators $\talg=u\t$ and ${\salg}=u^{-1}(A+e_2(\tau)\t)$ of the 
ring $R$. In terms of this generators
the transformed connection has the form:
$$d-\left(u^{-1}(E_2(\xi,\tau)-e_2(\tau))\talg    +
 \exp\left(-\sum _{k=2}^{\infty}\frac{(-\ad_{\talg } )^k}k
u^{-k}(E_k(\xi,\tau  )-e_k(\tau))\right){\salg}\right)ud\,\xi.
$$


As $e_{2k}(\tau)$, $k\ge 4$ are polynomial in $e_4(\tau)$ and
$e_6(\tau)$ with rational coefficients ,
$u^{-2k}e_{2k}(\tau)$  are polynomial in $60u^{-4}e_4(\tau)=g_2$ and
$140u^{-6}e_6(\tau)=g_3$ with rational coefficients.

As $E_k(\xi,\tau)$ are polynomial in $(E_2(\xi,\tau)-e_2(\tau)$,
$E_3(\xi,\tau)$, $e_4(\tau)$ and $e_6(\tau)$ with rational coefficients,
$u^{-k}E_k(\xi,\tau)$ are polynomial in $u^{-2}(E_2(\xi,\tau)-e_2(\tau)=x$,
$-2u^{-3}E_3(\xi,\tau)=y$, $g_2$ and $g_3$ with rational coefficients.

So, we see that for generators $\talg$ and ${\salg}$
the transformed connection $\nabla_{alg}$ is algebraic over $\Bbb
Q$; hence the ring $R_{alg}=\Bbb Q\ll \talg, {\salg}\gg$
is the algebraic $\Bbb Q$-structure on $R$.  Note that this
rational structure does not depends in the choice of the equation
of the elliptic curve, as a change of the equation multiplies $u$
by some {\it rational} number $\lambda^{-1}$.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%Relative case%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We shall realize analytic stacks $\Bbb H/SL_2(\Bbb Z)$ and $\Bbb X/SL_2(\Bbb Z)$
as stacks of $\Bbb C$-points of some algebraic stacks. All  mentioned bellow results are very classical and belongs to the 19{th}
century mathematics.

Consider the product $\Bbb H\times \Bbb C^*$, denote the coordinate on $\Bbb C^*$
by $u$. Define the action of $SL_2(\Bbb Z)$ by the following formula:
$$\left(\begin{array}{cc}
a&b\\
c&d
\end{array}\right):(\tau,u)\to\left(\frac{a\tau+b}{c\tau+b},
(c\tau+d)u\right).$$ In the coordinates $(v=u\tau,u)$ this action
is linear action on the column of $v$ and $u$. Then the map
$(\tau,u)\to (g_2=60u^{-4}e_4(\tau),\quad g_3=140u^{-4}e_6(\tau))$
is $SL_2(\Bbb Z)$-invariant and provides an isomorphism of the
quotient and  the complement ${\cal B}_{\Bbb C}$ of the curve
$\Delta:=g_2^3-27g_3^2=0$ in $\Bbb C^2$. As $ \Bbb H/SL_2(\Bbb Z)$
is the quotient of $ (\Bbb H\times\Bbb C^*)/SL_2(\Bbb Z)$ by $\Bbb
C^*$ acting on the second factor, this quotient stack  is equal to
$\Bbb C$-points of the quotient stack of ${\cal B}=\Bbb
A^2\setminus \{\Delta =0\}$ by the following action om $\Bbb G_m$:
$(g_2, g_3)\to(\lambda^{-4}g_2, \lambda^{-6}g_3)$. Evidently, this
algebraic stack is defined over $\Bbb Q$.

In the same way, we can consider the quotient $(\Bbb X\times\Bbb C^*)/SL_2(\Bbb Z)$ with
the same action of the group $SL_2(\Bbb Z)$ on the second factor.
Furthermore, the map $(\tau,\xi,u)\to  (g_2=60u^{-4}e_4(\tau),\quad g_3=140u^{-4}e_6(\tau)
x =u^{-2}(E_2(\xi,\tau)-e_2(\tau)),y=-2u^{-3}E_3(\xi,\tau),z=1)$ is an
isomorphism of this quotient with a complex projective cubic ${\cal Q}_{\Bbb C}
=\{y^2z=4x^3-g_2xz^2-g_3z^3\}$
over ${\cal B}_\Bbb C$. We get that $\Bbb X/SL_2(\Bbb Z)$ equals a stack of
$\Bbb
C$-points of the quotient of the cubic ${\cal Q}=\{y^2z=4x^3-g_2xz^2-g_3z^3\}$
over $\cal B$ by the action of $\Bbb G_m$ defined as the following:
$(g_2,g_3,x,y)\to (\lambda^{-4}g_2, \lambda^{-6}g_3 ,\lambda^{-2}x,
\lambda^{-3}y)$. The variety $\cal Q$ and action on it is defined over
$\Bbb Q$. The complement of the neutral section corresponds to the
affine curve ${\cal Q}^{aff}=\{y^2=4x^3-g_2x-g_3\}$.



Some analytic preparation.

As in the case of individual curve we apply the gauge
transformation of the left multiplication by $g(\xi,
\tau)=\exp(-E_1(\xi, \tau)\t)$. This transform the connection
$\nabla$ on $\frak P$ to
$$d-d\,g(\xi,\tau)g^{-1}(\xi,\tau)+g(\xi,\tau)\nu(\xi,\tau)g^{-1}(\xi,\tau)
-g(\xi,\tau)\psi_\t\partial_\t g^{-1}(\xi,\tau)-
g(\xi,\tau)\psi_A\partial_Ag^{-1}(\xi,\tau)$$
$$=d-(E_2 d\,\xi -\frac1{2\pi i}(E_3-E_1E_2)d\,\tau)\t
-\left(\exp\left(-\sum _{k=2}^{\infty}\frac{(-\ad_\t )^k}k
(E_k -e_k )\right) d\,\xi\right.
$$
$$
+\left(\left(-\frac{1}{\ad_\t}
+\sum _{k=1}^{\infty}
(-\ad_\t )^{k-1}
(E_k -e_k )
\right)
\exp\left(-\sum _{k=2}^{\infty}
\frac{(-\ad_\t )^k}k
(E_k -e_k )\right)\right.$$
$$\left.\left.+
\frac{\exp(-E_1\ad_\t)}{\ad_\t}\right)\frac{d\,\tau}{2\pi i}\right) A
+\left(\psi_\t\partial_\t -\frac1{2\pi
i}\frac{\exp(-E_1\ad_\t)-1}{-\ad_{\t}}
Ad\,\tau\right)+\psi_A\partial_A$$
$$=d-\left(E_2 \t
+\exp\left(-\sum _{k=2}^{\infty}\frac{(-\ad_\t )^k}k
(E_k -e_k )\right)A \right)(d\,\xi +\frac1{2\pi i}E_1d\,\tau)
+ E_3 \frac{\t d\,\tau}{2\pi i}
$$
$$
-\left(\left(-\frac{1}{\ad_\t}
+\sum _{k=2}^{\infty}
(-\ad_\t )^{k-1}
(E_k -e_k )
\right)
\exp\left(-\sum _{k=2}^{\infty}
\frac{(-\ad_\bfa )^k}k
(E_k -e_k )\right)+
\frac{1}{\ad_\t}\right)\frac{Ad\,\tau}{2\pi i} $$
$$
+\psi_\t\partial_\t  +\psi_A\partial_A=
d+\nu_{alg}+\psi_\t\partial_\t  +\psi_A\partial_A.$$

In this calculation we use the equality
$2\pi i \partial E_1/\partial\tau= E_3-E_1E_2$.
If we change generators $\t, A$ to $\talg=u\t, {\salg}=u^{-1}(B+e_2\t)$, the coefficients of the
differential form $\nu_{alg}$
become polynomials in $u^{-2}(E_2-e_2)=x$, $-2u^{-3}E_3=y$, $60u^{-4}e_4=g_2$ 
and $140u^{-6}e_6=g_3$, so we shell express
the forms $u(d\,\xi +\frac1{2\pi i}E_1d\,\tau)$ and $\frac{u^2d\,\tau}{2\pi i}$
in terms of $E_2-e_2$, $E_3$, $e_4$ and $e_6$.

Note that
$d\,\Delta=-12 \Delta (e_2\frac{d\,\tau}{2\pi i}+\frac{d\,u}u)$, so
$e_2\frac{d\,\tau}{2\pi i}+\frac{d\,u}u=-\frac1{12}\frac{d\,\Delta}{\Delta}$,
is an algebraic differential form, denote this form by $\kappa$.
We can treet the operator $d\, +j \kappa$ as the $\Bbb G_m$-equivariant 
connection on the trivial bundle on $\cal B$ eqipped by action $\lambda\to
\lambda^{-j}$ om $\Bbb G_m$, this explain
the coefficient of $\kappa$ in formulas bellow.

As $2\pi id\,e_4=(14e_6-4e_2e_4)d\,\tau$, 
$d\, g_2=6g_3\frac{u^2d\,\tau}{2\pi i}-4\kappa g_2$, hence
$\frac{u^2d\,\tau}{2\pi i}=\frac1{6}
\frac{(d\, +4e\kappa) e_4}{e_6}$
is algebraic.

As $2\pi i\partial e_2/\partial\tau=(5e_4-e_2^2) $ and
$2\pi i\partial E_2/\partial\tau=3((E_2-e_2)^2-5e_4)-E_2^2-2E_1E_3$ we have
$$  d\,x=yu(d\,\xi+\frac1{2\pi i}E_1d\,\tau)
+(2x^2-\frac13g_2)
\frac{u^2d\,\tau}{2\pi i}-2x\kappa ,
$$
so
$$u(d\,\xi +\frac1{2\pi i}E_1d\,\tau)=
 \frac{(d+2\kappa)x}y-
\frac{2x^2-\frac13g_2}{y}\frac{u^2d\,\tau}{2\pi i}$$
is $\Bbb Q$-algebraic.
Hence we can summarize that the differential forms
$$\frac{u^2d\,\tau}{2\pi i},\quad \left(e_2\frac{d\,\tau}{2\pi
i}+\frac{d\,u}u\right), \quad \mbox{and}\quad
u^{-1}(d\,\xi +\frac1{2\pi i}E_1d\,\tau)$$
can be expressed in terms of $E_2-e_2$, $E_3$, $e_4$, and $e_6$ and their
differentials with rational coefficients.

As we perform the change of generators $(\t, A)\to (\talg, {\salg})$
the differential term $d+\psi_\t\partial_\t + \psi_A\partial_A$
transforms.
The generator $\salg=u^{-1}(A+e_2\t)$ depends in $\tau$ directly, and both  
$\talg=u\t$ and $\salg$ depend in $u$, so the differentiation $d$
transforms to $d+d\,u/u\talg\partial_{\talg}+u^{-2}(de_2)\talg\partial_{\salg}-d\,u/u\salg\partial_{\salg}
$  , furthermore
$\psi_\t\partial_\t=-\frac{Ad\,\tau}{2\pi
i}\partial_{\t}$ transforms to
$$\left(u^{-1}e_2\talg -u{\salg}\right) \frac{d\,\tau}{2\pi
i}\left(u\partial_{\talg} +u^{-1}e_2\ \partial_{\salg}\right).$$
As $d\,e_2=(5e_4-e_2^2)\frac{d\,\tau}{2\pi i}$,
 we get that the term $d\,+ \psi_\bfa\partial_\bfa$ becames

$$d+  \left(\kappa\talg +\frac{u^2d\,\tau}{2\pi i}\salg\right)\partial_{\talg}
+\left( \frac1{12}g_2\frac{u^2d\,\tau}{2\pi i}\talg
-\kappa\salg\right)\partial_{\salg};$$
which is $\Bbb Q$-algebraic.

Finally, the summand $\psi_A\partial_A$ transforms to
$$\psi_{\salg}\partial_{\salg}=-\frac12
u\frac{u^{-2}XY}{u^{-1}X+u^{-1}Y}
$$
$$\times\left(\left(\wp(u^{-1}X)-\frac1{(u^{-1}X)^2}\right)
-\left(\wp(u^{-1}Y)-\frac1{(u^{-1}Y)^2}\right)
\right)\odb {\salg},{\salg}\cdb_{\talg} \frac{d\,\tau}{2\pi i}\partial_{\salg},$$
and the coefficient of terms
$[\ad_{\talg}^i{\salg},\ad_{\talg}^j{\salg}]\partial_{\salg}$
 in this expression can by calculated in terms of   the Taylor
 expansion at zero of $\wp(X)-X^2$. This coefficient
 is equal to $(-1)^{j-1}(i+j)u^{i+j+1}e_{i+j+1}\frac{u^2d\,\tau}{2\pi i}$, 
 so they are polynomials in $g_2$ and $g_3$ multiplied by algebraic form.
$\frac{u^2d\,\tau}{2\pi i}$.
 

So we  construct $\Bbb Q$ algebraic connections 
$({\cal R}_{alg}, \nabla_{{\cal R}alg})$ on {\cal B} and  
$({\frak P}_{alg}, \nabla_{{\frak P}alg})$ on
 ${\cal Q}^{aff}$ which are equal to the analytic ones after tensoring by $
 \Bbb C$. This algebraic connections are $\Bbb G_m$-equivariant.  

 Let $X\to S$ be a smooth algebraic family of elliptic curves defined over 
 $\Bbb Q$. Then
we have well defined  map of the family $X(\Bbb C)\to B(\Bbb C)$
of $\Bbb C$-points to $(\Bbb X)/SL_2(\Bbb Z)$, this map determines
the analytic connections ${\cal R}_S$ and ${\frak P}_{X/S}$.
We shall define an algebraic $\Bbb Q$ structure on them.  Denote  the generic 
point of $S$ by $\eta$. As the generic point
is  the spectrum of some field $K$, the elliptic curve $X_\eta$
over this point is
isomorphic to a cubic $y^2=4x^3-g_2 x -g_3$, this cubic is unique up to
 dilatations $g_2\to\lambda^4g_2,\quad g_3\to\lambda^6g_3,\quad
 x\to\lambda^2x,\quad y\to\lambda^3y$, $\lambda\in k$. 
 Fix some choice of $g_2$ and $g_3$, let $\tilde{S}$ be the open subscheme 
 of $S$ determined by inequalities $g_2\neq \infty$ , $g_3\neq \infty$ and $\Delta\neq 0$,
 put $\tilde{X}\to \tilde{S}$ be the induced family. Then we have the map
 $g=(g_2,g_3)$ from $\tilde{S}$ to $\cal B$ and $\tilde{X}$ is induced by $g$.
 
 The connections ${\cal R}_{\tilde{S}}$ and ${\frak P}_{\tilde{X}/\tilde{S}}$
 are equal to the pull-back of the correspondent connections on ${\cal
 Q}\to{\cal B}$, so the pull-back of ${\cal R}_{alg}$ and ${\frak P}_{alg}$
 determins the $\Bbb Q$-algebraic structure on them. Note that  
  $g^*{\cal R}_{alg}$ and $g^*{\frak P}_{alg}$ can be continued  as regular
 algebraic connections to $S$ and $X$ respectivly, as after tensoring by 
 $\Bbb C$ they becames regular analytic connections.
 
 These algebraic $\Bbb Q$-structures don't depend in the choice of $g_2$ and
 $g_3$ as they can be changed by dilateted one and  
 ${\cal R}_{ {\cal B}}$ and ${\frak P}_{{\cal
 Q}/{\cal B}}$ are $\Bbb G_m$-equivariant.


==> Andrey-2007-03-03/eis.tex <==
Let as recall the notations from WWW. chapters III and IV.

Consider a lattice generated by $\tau$ and $1$, $\Im(\tau)>0$. The point of
the space $\Bbb C$ we denote by $\xi$
$z=\exp(2\pi i \xi)$, $q=\exp(2\pi i \\tau)$

$\sum'$ denotes the summation over nonzero elements of a lattice.
$\sum'_e$ denotes some variant of regularization of the divergent sums,
known as {\em Eisenstein summation}.

Then $e_k(\tau)=\sum'_e(n\tau +m)^{-k}$, $E_k(\xi,\tau)=
\sum'_e(\xi+n\tau +m)^{-k}$; $e_k$ are modular functions for $k\ge 4$,
$E_k$ are elliptic functions for $k\ge 2$, moreover one can express the
Weierstrass elliptic functions and modular forms as
$\mp=E_2-e_2$, $\wp'=-2E_3$, $g_2=60e_4$ and $g_3=140e_6$.
It is knowm that $e_k$ are rational polynomials in $e_4$ and $e_6$ for
$k\ge 8$; $E_k$ are rational polynomials in $E_2-e_2$, $E_3$, $e_4$ and $e_6$ 
for $k\ge 4$, moerover the rings $\Bbb Q[e_k]$ and $\Bbb Q[E_k,e_k]$ are  
stable under differentiation
$(2\pi i)\partial_\tau$.

The basic theta-function is defined by the Jacobi product formula
$$\theta(\xi, \tau)=-iq^{1/8}(z^{1/2}-z{-1/2})\prod_{j=0}^\infty 
(1-zq^j)(1-z^{-1}q^j)(1-q^j).$$

Then $E_1=\partial_\xi\theta$.


==> Andrey-2007-03-03/geom.tex <==
\section{The Fundamental Hopf algebras for geometrical fiber functors.}

In this section we shall discuss the following question. Let $X\to
S, e$ be a families of elliptic curves. Let $\sigma$ be a section
of $U=X\setminus e(S)\to S$. Then the pull-back $\sigma^*$ is a
fibre functor $\sigma^*\colon\nilpconn(X/S; e)\to \conn (S)$. We
want to calculate the corresponding fundamental Hopf algebra in
the target category $\conn (S)$. We also consider the following
generalization of such pull-back (the tangential base point). Let
$z$ be a $1$-germ of fiberwise coordinate at the section $e$. Then
it defines a fibre functor by the rule: let  $\nabla$ be a flat
connection on $X$ with simple pole at $e$; denote by $K$ its
residue at $e$. Then the local connection $\nabla-Ad\,z/z$ has no
singularities and it is simple to check that
$e_z^*(\nabla):=e^*(\nabla-Ad\,z/z)$ is a flat connection on $S$.
Note that this functor depends on $1$-germ of $z$.

Some preparation. As we have mentioned, a continuation of the fiberwise functor ${\cal F}\colon
\mods{R}\to \nilpconn(X;e)$
  to the relative functor ${\cal F}_S\colon
\mods{{\cal R}_S} \to \nilpconn(X/S;e)$ is not unique. Indeed, let
$\mu$ be a ${\cal R}_S$-valued differential $1$-form which
satisfies to the Maurer-Cartan (MC) equation $\nabla_{\cal R}\mu
+\mu\wedge \mu=0$. Then we can define a new connection
$\nabla_{\cal R}^\mu=
 \nabla_{\cal R}+ad_{\mu}$ on the bundle ${\cal R}_S$. It is easy to check that
 MC equation yields flatness  of $\nabla_{\cal R}^\mu$. Denote by ${\cal R}^\mu$
 the connection ${\cal R}_S,\nabla_{\cal R}^\mu$. We can define the new
 connection
 $\nabla_{\frak P}^\mu=\nabla_{\cal R}^\mu +\nu-p^*\mu
 $ on ${\frak P}_{X/S}$, this connection is flat and corresponding
 object will be denote by ${\frak P}^\mu$. It determines  the functor
 ${\cal F}^\mu_S\colon\mods{{\cal R}_S^\mu} \to \nilpconn(X/S;e)$ in the same
 may as ${\frak P}_{X/S}$ determines ${\cal F}_S$.

 Note that the categories $\mods{{\cal R}_S}$ and $\mods{{\cal R}_S^\mu}$
 are equivalent, the corresponding functor $F_{0,\mu}$ sends ${\cal V},\nabla_{\cal V}$
 to ${\cal V},\nabla_{\cal V}+\mu$. Equivalently, this functor is define by the
 bimodule ${\cal P}_{0,\mu}\in \mods{{\cal R}_S^\mu}-{\cal R}_S$
 as bundle it is ${\cal R}_S$ and the connection $\nabla_{0,\mu}=\nabla_{\cal
 R}+\mu$.  Evidently,   ${\cal F}_S$ is isomorphic to ${\cal F}^\mu_S\circ
 F_{0,\mu}$,
 so ${\cal F}^\mu_S$ defines an equivalence of categories. We can treat
 ${\cal P}_{0,\mu}$ as the torsor of paths from $\omega_{DR}$ to the
 quasi-inverse  $\omega^\mu_{DR}$ of ${\cal F}^\mu_S$. More
 generically, the torsor of paths from $\omega^\mu_{DR}$ to $\omega^{\mu'}_{DR}$
is isomorphic to the bimodule ${\cal P}_{\mu,\mu'}\in \mods{{\cal
R}_S^{\mu'}}-{\cal R}_S^\mu$ as bundle it is ${\cal R}_S$ and the
connection $\nabla_{\mu,\mu'}$ is defined by the rule
$\nabla_{\mu,\mu'}r=\nabla_{\cal
 R}r+\mu'r-r\mu$.

 Now we can calculate the composition $\sigma^*\circ {\cal F}^\mu_S$
 By the very definition we get that it maps $({\cal V},
 \nabla_{\cal V})$ to $({\cal V}, \nabla_{\cal
 V}+\sigma^*(\nu)-\mu)$. So, for $\mu=\sigma^*(\nu$ we get that
 this composition is isomorphic to the forgetting functor
 from $\mods{{\cal R}}^\mu_S$ to $\conn(S)$. As ${\cal F}^\mu_S$
 is an equivalence of categories we can conclude that ${\cal R}_S^\mu$
 for $\mu=\sigma^*(\nu)$ is isomorphic to the fundamental Hopf algebra of fibre functor
 $\sigma^*$. In the same way one can show that for two sections $\sigma_1$ and $\sigma_2$
the bimodule ${\cal P}_{\mu_1,\mu_2}$, $\mu_i=\sigma_i(\nu)$ is
isomorphic to the torsor of paths from $\sigma_1$ to $\sigma_2$.

By applying the Reimann-Hilbert correspondence, we can conclude
that the parallel transport $\Phi$ with respect to the connection
${\frak P}_{X/S}$ along a $S$-family of paths from $\sigma_1$ to
$\sigma_2$ satisfies to the equation
$$\nabla \Phi +\sigma_1^*(\nu)\Phi-\Phi\sigma_2^*(\nu)=0.$$

The case of the tangential base point can be treated in the same
way.

Note that if $X/S$ be an algebraic family over $\Bbb Q$ and $\mu$
is $\Bbb Q$-algebraic ${\cal R}_{alg}$-valued $1$-form, then
${\cal R}^\mu$ and ${\frak P}^\mu$ can be equipped by algebraic
structure. Hence, for $\Bbb Q$ section $\sigma$ the fundamental
Hopf algebra is equipped by algebraic $\Bbb Q$-structure.


==> alg.tex <==
\section{Algebraic structure.} In this section we describe the algebraic $\Bbb Q$
structure on $\cal P$ and $R$ for an elliptic curve defined over
$\Bbb Q$.

We start from reminding of some standard  facts about algebraic
elliptic curves. Let $(X,O)$ be an elliptic curve defined over
some field $k$ of characteristic zero.
 Then  it can be represented as a plane cubic $y^2=4x^3-g_2 x -g_3$,
 $g_2, g_3\in k$  and the
 marked point $O$ lies at infinity. This form is unique up to
 dilatations $g_2\to\lambda^4g_2,\quad g_3\to\lambda^6g_3,\quad
 x\to\lambda^2x,\quad y\to\lambda^3y$, $\lambda\in k$.

  If $k$ is a subfield of $\Bbb C$, e.g.
$k=\Bbb Q$, one can represent the analytic curve $X(\Bbb C)$ as the
quotient of $\Bbb C$ by some lattice $L$. The
map  from $X(\Bbb C)$ to $\Bbb C/L$ is defined by integration
of the form
$\omega =d\,x/y$ from the marked point to the variable one
$p\to\int_O^p\omega$. The ambiguity in choosing of the path of integration
belongs to the topological first homology group $H_1(X(\Bbb C),\Bbb Z)$
which corresponds to the lattice $L$.
 Choose some basis $(u, v)$ in
such a way that $\Im (v/u)>0$, put $\tau=v/u$. Then
$g_2=60u^{-4}e_4(\tau),\quad g_3=140u^{-4}e_6(\tau)$, moreover
the map
$\xi\to (x(\xi)=u^{-2}(E_2(\xi,\tau)-e_2(\tau)),\quad y(\xi)=-2u^{-3}E_3(\xi,\tau))$
produces an analytic isomorphism between $X_{\tau}=\Bbb C/(\Bbb Z\tau +\Bbb Z)$
and  $X(\Bbb C)$ and $\omega=d\,x/y=ud\,\xi$. So, $u$ can be calulated as the
period (elliptic integral) of the algebraic form $\omega$ against a
topological
chain. If we choose another equation of $X$, twisted say, by $\lambda$,
then $\omega$ becomes $\lambda^{-1}\omega$ and $(u,v)\to (\lambda^{-1}u,
\lambda^{-1}v)$.


Some analytic preparations. Note that over the complement
$U_\tau$ to the marked point in $X_\tau$ the bundle $\cal P$
defined by multiplier $\exp(-2\pi i\t)$ is trivial and can be
trivialized by the left multiplication by
$g(\xi)=\exp(-E_1(\xi,\tau)\t)$, indeed,  sections of $\cal P$
are the quasiperiodic functions $f$ on $\Bbb C$:
$f(\xi+1)=f(\xi);\quad f(\xi+\tau)=\exp(-2\pi i\t)f(\xi)$; hence
$g(\xi)f$ are periodic, as $E_1(\xi+1,\tau)=E_1(\xi,\tau), \quad
E_1(\xi+\tau,\tau)= E_1(\xi,\tau)-2\pi i$.

The connection $\nabla=d-\ad_\t F(\xi,\ad_\t)Ad\,\xi$
transforms under the gauge transformation $s\to g(\xi)s$ to the operator
$$g(\xi)\nabla g^{-1}(\xi)=d-d\,g(\xi)g^{-1}(\xi)-
g(\xi)\ad_\t F(\xi,\ad_\t)Ag^{-1}d\,\xi$$
$$=d-E_2(\xi,\tau)\t d\,\xi -\exp(-E_1(\xi,\tau)\ad_\t )
 \exp\left(-\sum _{k=1}^{\infty}\frac{(-\ad_\t  )^k}k
(E_k(\xi,\tau  )-e_k(\tau))\right)Ad\,\xi$$
$$=
d-\left((E_2(\xi,\tau)-e_2(\tau))\t    +
 \exp\left(-\sum _{k=2}^{\infty}\frac{(-\ad_\t  )^k}k
(E_k(\xi,\tau  )-e_k(\tau))\right)(A+e_2(\tau)\t\right)d\,\xi.
$$

Consider new generators $\talg=u\t$ and ${\salg}=u^{-1}(A+e_2(\tau)\t)$ of the 
ring $R$. In terms of this generators
the transformed connection has the form:
$$d-\left(u^{-1}(E_2(\xi,\tau)-e_2(\tau))\talg    +
 \exp\left(-\sum _{k=2}^{\infty}\frac{(-\ad_{\talg } )^k}k
u^{-k}(E_k(\xi,\tau  )-e_k(\tau))\right){\salg}\right)ud\,\xi.
$$


As $e_{2k}(\tau)$, $k\ge 4$ are polynomial in $e_4(\tau)$ and
$e_6(\tau)$ with rational coefficients ,
$u^{-2k}e_{2k}(\tau)$  are polynomial in $60u^{-4}e_4(\tau)=g_2$ and
$140u^{-6}e_6(\tau)=g_3$ with rational coefficients.

As $E_k(\xi,\tau)$ are polynomial in $(E_2(\xi,\tau)-e_2(\tau)$,
$E_3(\xi,\tau)$, $e_4(\tau)$ and $e_6(\tau)$ with rational coefficients,
$u^{-k}E_k(\xi,\tau)$ are polynomial in $u^{-2}(E_2(\xi,\tau)-e_2(\tau)=x$,
$-2u^{-3}E_3(\xi,\tau)=y$, $g_2$ and $g_3$ with rational coefficients.

So, we see that for generators $\talg$ and ${\salg}$
the transformed connection $\nabla_{alg}$ is algebraic over $\Bbb
Q$; hence the ring $R_{alg}=\Bbb Q\ll \talg, {\salg}\gg$
is the algebraic $\Bbb Q$-structure on $R$.  Note that this
rational structure does not depends in the choice of the equation
of the elliptic curve, as a change of the equation multiplies $u$
by some {\it rational} number $\lambda^{-1}$.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%Relative case%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We shall realize analytic stacks $\Bbb H/SL_2(\Bbb Z)$ and $\Bbb X/SL_2(\Bbb Z)$
as stacks of $\Bbb C$-points of some algebraic stacks. All  mentioned bellow results are very classical and belongs to the 19{th}
century mathematics.

Consider the product $\Bbb H\times \Bbb C^*$, denote the coordinate on $\Bbb C^*$
by $u$. Define the action of $SL_2(\Bbb Z)$ by the following formula:
$$\left(\begin{array}{cc}
a&b\\
c&d
\end{array}\right):(\tau,u)\to\left(\frac{a\tau+b}{c\tau+b},
(c\tau+d)u\right).$$ In the coordinates $(v=u\tau,u)$ this action
is linear action on the column of $v$ and $u$. Then the map
$(\tau,u)\to (g_2=60u^{-4}e_4(\tau),\quad g_3=140u^{-4}e_6(\tau))$
is $SL_2(\Bbb Z)$-invariant and provides an isomorphism of the
quotient and  the complement ${\cal B}_{\Bbb C}$ of the curve
$\Delta:=g_2^3-27g_3^2=0$ in $\Bbb C^2$. As $ \Bbb H/SL_2(\Bbb Z)$
is the quotient of $ (\Bbb H\times\Bbb C^*)/SL_2(\Bbb Z)$ by $\Bbb
C^*$ acting on the second factor, this quotient stack  is equal to
$\Bbb C$-points of the quotient stack of ${\cal B}=\Bbb
A^2\setminus \{\Delta =0\}$ by the following action om $\Bbb G_m$:
$(g_2, g_3)\to(\lambda^{-4}g_2, \lambda^{-6}g_3)$. Evidently, this
algebraic stack is defined over $\Bbb Q$.

In the same way, we can consider the quotient $(\Bbb X\times\Bbb C^*)/SL_2(\Bbb Z)$ with
the same action of the group $SL_2(\Bbb Z)$ on the second factor.
Furthermore, the map $(\tau,\xi,u)\to  (g_2=60u^{-4}e_4(\tau),\quad g_3=140u^{-4}e_6(\tau)
x =u^{-2}(E_2(\xi,\tau)-e_2(\tau)),y=-2u^{-3}E_3(\xi,\tau),z=1)$ is an
isomorphism of this quotient with a complex projective cubic ${\cal Q}_{\Bbb C}
=\{y^2z=4x^3-g_2xz^2-g_3z^3\}$
over ${\cal B}_\Bbb C$. We get that $\Bbb X/SL_2(\Bbb Z)$ equals a stack of
$\Bbb
C$-points of the quotient of the cubic ${\cal Q}=\{y^2z=4x^3-g_2xz^2-g_3z^3\}$
over $\cal B$ by the action of $\Bbb G_m$ defined as the following:
$(g_2,g_3,x,y)\to (\lambda^{-4}g_2, \lambda^{-6}g_3 ,\lambda^{-2}x,
\lambda^{-3}y)$. The variety $\cal Q$ and action on it is defined over
$\Bbb Q$. The complement of the neutral section corresponds to the
affine curve ${\cal Q}^{aff}=\{y^2=4x^3-g_2x-g_3\}$.



Some analytic preparation.

As in the case of individual curve we apply the gauge
transformation of the left multiplication by $g(\xi,
\tau)=\exp(-E_1(\xi, \tau)\t)$. This transform the connection
$\nabla$ on $\frak P$ to
$$d-d\,g(\xi,\tau)g^{-1}(\xi,\tau)+g(\xi,\tau)\nu(\xi,\tau)g^{-1}(\xi,\tau)
-g(\xi,\tau)\psi_\t\partial_\t g^{-1}(\xi,\tau)-
g(\xi,\tau)\psi_A\partial_Ag^{-1}(\xi,\tau)$$
$$=d-(E_2 d\,\xi -\frac1{2\pi i}(E_3-E_1E_2)d\,\tau)\t
-\left(\exp\left(-\sum _{k=2}^{\infty}\frac{(-\ad_\t )^k}k
(E_k -e_k )\right) d\,\xi\right.
$$
$$
+\left(\left(-\frac{1}{\ad_\t}
+\sum _{k=1}^{\infty}
(-\ad_\t )^{k-1}
(E_k -e_k )
\right)
\exp\left(-\sum _{k=2}^{\infty}
\frac{(-\ad_\t )^k}k
(E_k -e_k )\right)\right.$$
$$\left.\left.+
\frac{\exp(-E_1\ad_\t)}{\ad_\t}\right)\frac{d\,\tau}{2\pi i}\right) A
+\left(\psi_\t\partial_\t -\frac1{2\pi
i}\frac{\exp(-E_1\ad_\t)-1}{-\ad_{\t}}
Ad\,\tau\right)+\psi_A\partial_A$$
$$=d-\left(E_2 \t
+\exp\left(-\sum _{k=2}^{\infty}\frac{(-\ad_\t )^k}k
(E_k -e_k )\right)A \right)(d\,\xi +\frac1{2\pi i}E_1d\,\tau)
+ E_3 \frac{\t d\,\tau}{2\pi i}
$$
$$
-\left(\left(-\frac{1}{\ad_\t}
+\sum _{k=2}^{\infty}
(-\ad_\t )^{k-1}
(E_k -e_k )
\right)
\exp\left(-\sum _{k=2}^{\infty}
\frac{(-\ad_\bfa )^k}k
(E_k -e_k )\right)+
\frac{1}{\ad_\t}\right)\frac{Ad\,\tau}{2\pi i} $$
$$
+\psi_\t\partial_\t  +\psi_A\partial_A=
d+\nu_{alg}+\psi_\t\partial_\t  +\psi_A\partial_A.$$

In this calculation we use the equality
$2\pi i \partial E_1/\partial\tau= E_3-E_1E_2$.
If we change generators $\t, A$ to $\talg=u\t, {\salg}=u^{-1}(B+e_2\t)$, the coefficients of the
differential form $\nu_{alg}$
become polynomials in $u^{-2}(E_2-e_2)=x$, $-2u^{-3}E_3=y$, $60u^{-4}e_4=g_2$ 
and $140u^{-6}e_6=g_3$, so we shell express
the forms $u(d\,\xi +\frac1{2\pi i}E_1d\,\tau)$ and $\frac{u^2d\,\tau}{2\pi i}$
in terms of $E_2-e_2$, $E_3$, $e_4$ and $e_6$.

Note that
$d\,\Delta=-12 \Delta (e_2\frac{d\,\tau}{2\pi i}+\frac{d\,u}u)$, so
$e_2\frac{d\,\tau}{2\pi i}+\frac{d\,u}u=-\frac1{12}\frac{d\,\Delta}{\Delta}$,
is an algebraic differential form, denote this form by $\kappa$.
We can treet the operator $d\, +j \kappa$ as the $\Bbb G_m$-equivariant 
connection on the trivial bundle on $\cal B$ eqipped by action $\lambda\to
\lambda^{-j}$ om $\Bbb G_m$, this explain
the coefficient of $\kappa$ in formulas bellow.

As $2\pi id\,e_4=(14e_6-4e_2e_4)d\,\tau$, 
$d\, g_2=6g_3\frac{u^2d\,\tau}{2\pi i}-4\kappa g_2$, hence
$\frac{u^2d\,\tau}{2\pi i}=\frac1{6}
\frac{(d\, +4e\kappa) e_4}{e_6}$
is algebraic.

As $2\pi i\partial e_2/\partial\tau=(5e_4-e_2^2) $ and
$2\pi i\partial E_2/\partial\tau=3((E_2-e_2)^2-5e_4)-E_2^2-2E_1E_3$ we have
$$  d\,x=yu(d\,\xi+\frac1{2\pi i}E_1d\,\tau)
+(2x^2-\frac13g_2)
\frac{u^2d\,\tau}{2\pi i}-2x\kappa ,
$$
so
$$u(d\,\xi +\frac1{2\pi i}E_1d\,\tau)=
 \frac{(d+2\kappa)x}y-
\frac{2x^2-\frac13g_2}{y}\frac{u^2d\,\tau}{2\pi i}$$
is $\Bbb Q$-algebraic.
Hence we can summarize that the differential forms
$$\frac{u^2d\,\tau}{2\pi i},\quad \left(e_2\frac{d\,\tau}{2\pi
i}+\frac{d\,u}u\right), \quad \mbox{and}\quad
u^{-1}(d\,\xi +\frac1{2\pi i}E_1d\,\tau)$$
can be expressed in terms of $E_2-e_2$, $E_3$, $e_4$, and $e_6$ and their
differentials with rational coefficients.

As we perform the change of generators $(\t, A)\to (\talg, {\salg})$
the differential term $d+\psi_\t\partial_\t + \psi_A\partial_A$
transforms.
The generator $\salg=u^{-1}(A+e_2\t)$ depends in $\tau$ directly, and both  
$\talg=u\t$ and $\salg$ depend in $u$, so the differentiation $d$
transforms to $d+d\,u/u\talg\partial_{\talg}+u^{-2}(de_2)\talg\partial_{\salg}-d\,u/u\salg\partial_{\salg}
$  , furthermore
$\psi_\t\partial_\t=-\frac{Ad\,\tau}{2\pi
i}\partial_{\t}$ transforms to
$$\left(u^{-1}e_2\talg -u{\salg}\right) \frac{d\,\tau}{2\pi
i}\left(u\partial_{\talg} +u^{-1}e_2\ \partial_{\salg}\right).$$
As $d\,e_2=(5e_4-e_2^2)\frac{d\,\tau}{2\pi i}$,
 we get that the term $d\,+ \psi_\bfa\partial_\bfa$ becames

$$d+  \left(\kappa\talg +\frac{u^2d\,\tau}{2\pi i}\salg\right)\partial_{\talg}
+\left( \frac1{12}g_2\frac{u^2d\,\tau}{2\pi i}\talg
-\kappa\salg\right)\partial_{\salg};$$
which is $\Bbb Q$-algebraic.

Finally, the summand $\psi_A\partial_A$ transforms to
$$\psi_{\salg}\partial_{\salg}=-\frac12
u\frac{u^{-2}XY}{u^{-1}X+u^{-1}Y}
$$
$$\times\left(\left(\wp(u^{-1}X)-\frac1{(u^{-1}X)^2}\right)
-\left(\wp(u^{-1}Y)-\frac1{(u^{-1}Y)^2}\right)
\right)\odb {\salg},{\salg}\cdb_{\talg} \frac{d\,\tau}{2\pi i}\partial_{\salg},$$
and the coefficient of terms
$[\ad_{\talg}^i{\salg},\ad_{\talg}^j{\salg}]\partial_{\salg}$
 in this expression can by calculated in terms of   the Taylor
 expansion at zero of $\wp(X)-X^2$. This coefficient
 is equal to $(-1)^{j-1}(i+j)u^{i+j+1}e_{i+j+1}\frac{u^2d\,\tau}{2\pi i}$, 
 so they are polynomials in $g_2$ and $g_3$ multiplied by algebraic form.
$\frac{u^2d\,\tau}{2\pi i}$.
 

So we  construct $\Bbb Q$ algebraic connections 
$({\cal R}_{alg}, \nabla_{{\cal R}alg})$ on {\cal B} and  
$({\frak P}_{alg}, \nabla_{{\frak P}alg})$ on
 ${\cal Q}^{aff}$ which are equal to the analytic ones after tensoring by $
 \Bbb C$. This algebraic connections are $\Bbb G_m$-equivariant.  

 Let $X\to S$ be a smooth algebraic family of elliptic curves defined over 
 $\Bbb Q$. Then
we have well defined  map of the family $X(\Bbb C)\to B(\Bbb C)$
of $\Bbb C$-points to $(\Bbb X)/SL_2(\Bbb Z)$, this map determines
the analytic connections ${\cal R}_S$ and ${\frak P}_{X/S}$.
We shall define an algebraic $\Bbb Q$ structure on them.  Denote  the generic 
point of $S$ by $\eta$. As the generic point
is  the spectrum of some field $K$, the elliptic curve $X_\eta$
over this point is
isomorphic to a cubic $y^2=4x^3-g_2 x -g_3$, this cubic is unique up to
 dilatations $g_2\to\lambda^4g_2,\quad g_3\to\lambda^6g_3,\quad
 x\to\lambda^2x,\quad y\to\lambda^3y$, $\lambda\in k$. 
 Fix some choice of $g_2$ and $g_3$, let $\tilde{S}$ be the open subscheme 
 of $S$ determined by inequalities $g_2\neq \infty$ , $g_3\neq \infty$ and $\Delta\neq 0$,
 put $\tilde{X}\to \tilde{S}$ be the induced family. Then we have the map
 $g=(g_2,g_3)$ from $\tilde{S}$ to $\cal B$ and $\tilde{X}$ is induced by $g$.
 
 The connections ${\cal R}_{\tilde{S}}$ and ${\frak P}_{\tilde{X}/\tilde{S}}$
 are equal to the pull-back of the correspondent connections on ${\cal
 Q}\to{\cal B}$, so the pull-back of ${\cal R}_{alg}$ and ${\frak P}_{alg}$
 determins the $\Bbb Q$-algebraic structure on them. Note that  
  $g^*{\cal R}_{alg}$ and $g^*{\frak P}_{alg}$ can be continued  as regular
 algebraic connections to $S$ and $X$ respectivly, as after tensoring by 
 $\Bbb C$ they becames regular analytic connections.
 
 These algebraic $\Bbb Q$-structures don't depend in the choice of $g_2$ and
 $g_3$ as they can be changed by dilateted one and  
 ${\cal R}_{ {\cal B}}$ and ${\frak P}_{{\cal
 Q}/{\cal B}}$ are $\Bbb G_m$-equivariant.


==> carac.tex <==
\usepackage{mathrsfs}

\def \AM{{\mathbb{A}}}
\def \BM{{\mathbb{B}}}
\def \CM{{\mathbb{C}}}
\def \DM{{\mathbb{D}}}
\def \EM{{\mathbb{E}}}
\def \FM{{\mathbb{F}}}
\def \GM{{\mathbb{G}}}
\def \HM{{\mathbb{H}}}
\def \IM{{\mathbb{I}}}
\def \JM{{\mathbb{J}}}
\def \KM{{\mathbb{K}}}
\def \LM{{\mathbb{L}}}
\def \Mm{{\mathbb{M}}}
\def \NM{{\mathbb{N}}}
\def \OM{{\mathbb{O}}}
\def \PM{{\mathbb{P}}}
\def \QM{{\mathbb{Q}}}
\def \RM{{\mathbb{R}}}
\def \SM{{\mathbb{S}}}
\def \TM{{\mathbb{T}}}
\def \UM{{\mathbb{U}}}
\def \VM{{\mathbb{V}}}
\def \WM{{\mathbb{W}}}
\def \XM{{\mathbb{X}}}
\def \YM{{\mathbb{Y}}}
\def \ZM{{\mathbb{Z}}}

\def \AC{{\mathcal A}}
\def \BC{{\mathcal B}}
\def \CC{{\mathcal C}}
\def \DC{{\mathcal D}}
\def \EC{{\mathcal E}}
\def \FC{{\mathcal F}}
\def \GC{{\mathcal G}}
\def \HC{{\mathcal H}}
\def \IC{{\mathcal I}}
\def \JC{{\mathcal J}}
\def \KC{{\mathcal K}}
\def \LC{{\mathcal L}}
\def \MC{{\mathcal M}}
\def \NC{{\mathcal N}}
\def \OC{{\mathcal O}}
\def \PC{{\mathcal P}}
\def \QC{{\mathcal Q}}
\def \RC{{\mathcal R}}
\def \SC{{\mathcal S}}
\def \TC{{\mathcal T}}
\def \UC{{\mathcal U}}
\def \VC{{\mathcal V}}
\def \WC{{\mathcal W}}
\def \XC{{\mathcal X}}
\def \YC{{\mathcal Y}}
\def \ZC{{\mathcal Z}}

\def \AG{{\mathfrak A}}
\def \BG{{\mathfrak B}}
\def \CG{{\mathfrak C}}
\def \DG{{\mathfrak D}}
\def \EG{{\mathfrak E}}
\def \FG{{\mathfrak F}}
\def \GG{{\mathfrak G}}
\def \HG{{\mathfrak H}}
\def \IG{{\mathfrak I}}
\def \JG{{\mathfrak J}}
\def \KG{{\mathfrak K}}
\def \LG{{\mathfrak L}}
\def \MG{{\mathfrak M}}
\def \NG{{\mathfrak N}}
\def \OG{{\mathfrak O}}
\def \PG{{\mathfrak P}}
\def \QG{{\mathfrak Q}}
\def \RG{{\mathfrak R}}
\def \SG{{\mathfrak S}}
\def \TG{{\mathfrak T}}
\def \UG{{\mathfrak U}}
\def \VG{{\mathfrak V}}
\def \WG{{\mathfrak W}}
\def \XG{{\mathfrak X}}
\def \YG{{\mathfrak Y}}
\def \ZG{{\mathfrak Z}}

\def \aG{{\mathfrak a}}
\def \bG{{\mathfrak b}}
\def \cG{{\mathfrak c}}
\def \dG{{\mathfrak d}}
\def \eG{{\mathfrak e}}
\def \fG{{\mathfrak f}}
\def \gG{{\mathfrak g}}
\def \hG{{\mathfrak h}}
\def \iG{{\mathfrak i}}
\def \jG{{\mathfrak j}}
\def \kG{{\mathfrak k}}
\def \lG{{\mathfrak l}}
\def \mG{{\mathfrak m}}
\def \nG{{\mathfrak n}}
\def \oG{{\mathfrak o}}
\def \pG{{\mathfrak p}}
\def \qG{{\mathfrak q}}
\def \rG{{\mathfrak r}}
\def \sG{{\mathfrak s}}
\def \tG{{\mathfrak t}}
\def \uG{{\mathfrak u}}
\def \vG{{\mathfrak v}}
\def \wG{{\mathfrak w}}
\def \xG{{\mathfrak x}}
\def \yG{{\mathfrak y}}
\def \zG{{\mathfrak z}}

\def \ACC{{\mathscr A}}
\def \BCC{{\mathscr B}}
\def \CCC{{\mathscr C}}
\def \DCC{{\mathscr D}}
\def \ECC{{\mathscr E}}
\def \FCC{{\mathscr F}}
\def \GCC{{\mathscr G}}
\def \HCC{{\mathscr H}}
\def \ICC{{\mathscr I}}
\def \JCC{{\mathscr J}}
\def \KCC{{\mathscr K}}
\def \LCC{{\mathscr L}}
\def \MCC{{\mathscr M}}
\def \NCC{{\mathscr N}}
\def \OCC{{\mathscr O}}
\def \PCC{{\mathscr P}}
\def \QCC{{\mathscr Q}}
\def \RCC{{\mathscr R}}
\def \SCC{{\mathscr S}}
\def \TCC{{\mathscr T}}
\def \UCC{{\mathscr U}}
\def \VCC{{\mathscr V}}
\def \WCC{{\mathscr W}}
\def \XCC{{\mathscr X}}
\def \YCC{{\mathscr Y}}
\def \ZCC{{\mathscr Z}}


\def\aB{\mathbf{a}}
\def\bB{\mathbf{b}}
\def\cB{\mathbf{c}}
\def\dB{\mathbf{d}}
\def\eB{\mathbf{e}}
\def\fB{\mathbf{f}}
\def\gB{\mathbf{g}}
\def\hB{\mathbf{h}}
\def\iB{\mathbf{i}}
\def\jB{\mathbf{j}}
\def\kB{\mathbf{k}}
\def\lB{\mathbf{l}}
\def\mB{\mathbf{m}}
\def\nB{\mathbf{n}}
\def\oB{\mathbf{o}}
\def\pB{\mathbf{p}}
\def\qB{\mathbf{q}}
\def\rB{\mathbf{r}}
\def\sB{\mathbf{s}}
\def\tB{\mathbf{t}}
\def\uB{\mathbf{u}}
\def\vB{\mathbf{v}}
\def\wB{\mathbf{w}}
\def\xB{\mathbf{x}}
\def\yB{\mathbf{y}}
\def\zB{\mathbf{z}}
\def\AB{\mathbf{A}}
\def\BB{\mathbf{B}}
\def\CB{\mathbf{C}}
\def\DB{\mathbf{D}}
\def\EB{\mathbf{E}}
\def\FB{\mathbf{F}}
\def\GB{\mathbf{G}}
\def\HB{\mathbf{H}}
\def\IB{\mathbf{I}}
\def\JB{\mathbf{J}}
\def\KB{\mathbf{K}}
\def\LB{\mathbf{L}}
\def\MB{\mathbf{M}}
\def\NB{\mathbf{N}}
\def\OB{\mathbf{O}}
\def\PB{\mathbf{P}}
\def\QB{\mathbf{Q}}
\def\RB{\mathbf{R}}
\def\SB{\mathbf{S}}
\def\TB{\mathbf{T}}
\def\UB{\mathbf{U}}
\def\VB{\mathbf{V}}
\def\WB{\mathbf{W}}
\def\XB{\mathbf{X}}
\def\YB{\mathbf{Y}}
\def\ZB{\mathbf{Z}}

